Providing Long-Term Participation Incentive in Participatory Sensing

Providing an adequate long-term participation incentive is important for a participatory sensing system to maintain enough number of active users (sensors), so as to collect a sufficient number of data samples and support a desired level of service quality. In this work, we consider the sensor selection problem in a general time-dependent and location-aware participatory sensing system, taking the long-term user participation incentive into explicit consideration. We study the problem systematically under different information scenarios, regarding both future information and current information (realization). In particular, we propose a Lyapunov-based VCG auction policy for the on-line sensor selection, which converges asymptotically to the optimal off-line benchmark performance, even with no future information and under (current) information asymmetry. Extensive numerical results show that our proposed policy outperforms the state-of-art policies in the literature, in terms of both user participation (e.g., reducing the user dropping probability by 25% to 90%) and social performance (e.g., increasing the social welfare by 15% to 80%).

==> section-old.tex <==
%!TEX root = main_participarory_sensing.tex
%SourceDoc main_participarory_sensing.tex


\section{Literature Review}\label{sec:literature}



\subsection{System Model and Problem Formulation}


Let $\N \eq \{1,...,N\}$ denote the set of mobile users that the SP employs for data sensing. 
The SP requests data from mobile users periodically, with a period ranging from minutes to hours depending on different types of applications/tasks. 
We consider the sensing operations in a time interval consisting of $T$ sensing periods.
At each sensing period $t\in \{1,...,T\}$, the SP requires at least $K$ (where $K\leq N$) mobile users' sensing data to ensure the availability/reliability of the obtained data.\footnote{\rev{\small Extension: Later we may consider the ``spatial reuse'' among mobile users. For example, mobile users are randomly distributed within a certain area, and the SP requires at least $K$ spatially-separated mobile users' data.}} 
In such a context, one of the important problems is to choose the proper set of mobile users as data sources at each sensing period.
%When a mobile user is chosen as data source at a particular sensing period, it performs the sensing activity and transmits the sensing data to the SP.

\emph{Sensing cost}. 
When a mobile user is chosen as data source at a particular sensing period, it performs the sensing process and transmits the sensing data to the SP. 
This sensing activity will incur additional operational cost (called \emph{sensing cost}) on the mobile user due to, for example, the energy consumption, transmission bandwidth occupancy, and etc. 
Let $c_n^{(t)}$ denote the sensing cost of mobile user $n$ at sensing period $t$. 
We consider a general model where a mobile user may have different sensing costs at different sensing periods, and different mobile users may have different sensing costs at the same sensing period.
For writing convenience, let $\bc_n \eq \{c_n^{(1)}, ..., c_n^{(T)}\}$ denote the sensing cost vector of mobile user $n$ at all sensing periods, and $\bc^{(t)} \eq \{c_1^{(t)}, ..., c_N^{(t)}\}$ denote the sensing cost vector of all mobile users at sensing period $t$.

\emph{Dropping threshold}. When a mobile user is chosen as data source at a sensing period, the SP needs to pay certain monetary compensation to the user.
This compensation is not only used to compensate the potential sensing cost incurred on the user, but may also provide positive revenue for the user so as to incentivize the user to perform the sensing activity. 
Thus, with such compensations, mobile users are interested in being data sources and sensing data for the SP. 
However, if a mobile user is rarely chosen as data source, it will gradually lose the interest and decide not to participate in the sensing system in the future (in this case we will say the user drops). 
%Whenever a mobile user drops, it will never participate in the future sensing tasks. 
For analytic convenience, we consider such a scenario: Each mobile user will drop if the probability of being chosen as data source is smaller than a certain threshold (called \emph{dropping threshold}). 
Let $\dpr_n$ denote the dropping threshold of mobile user $n$, and $\bdpr \eq \{\dpr_1,...,\dpr_N\}$ denote the dropping threshold vector of all mobile users. 


Based on the above, the key problem in such a sensing system is to determine (i) the set of data sources at each sensing period, and (ii) the corresponding payments (compensations) to the data sources.
The  {objective} is to \emph{minimize the SP's total payments to mobile users, subject to the SP's sensing requirement and
the mobile user's participatory constraint}. 
%The SP's \emph{payoff} is defined as the difference between the revenue from the applications/tasks and the payments to the data sources.
The SP's sensing requirement guarantees the availability/reliability of the obtained data at each sensing period, i.e., the number of data sources is no smaller than $K$.
The mobile user's \emph{participatory constraint} guarantees that a mobile user $n$ will not drop out of the system, i.e., the probability of being chosen as data source is no smaller than its dropping threshold $\dpr_n$. 

We will study the \emph{SP's payment minimization} problem under different information scenarios: (i) complete information, (ii) incomplete symmetric information, and (iii) incomplete asymmetric information.\footnote{\rev{\small The SP's payoff maximization problem is totally equivalent to the SP's payment minimization problem, if we assume that the SP achieves a fixed revenue from the obtained data (i.e., the SP's achieved revenue is independent of the number of data sources as long as the sensing requirement is satisfied). 
However, if we assume that the SP's revenue increases with the number of data sources, these two problems will be a bit different, but similar analytic method can be applied.}}
In this model, the information mainly includes the sensing costs of mobile users. 
Under complete information, the SP knows the exact sensing costs of all mobile users at all sensing periods in advance. 
Under incomplete information, however, the SP does not know the exact sensing costs of mobile users at the future sensing periods, but only certain stochastic distributions about such sensing costs.
Moreover, under incomplete symmetric information, the SP is able to observe the exact sensing costs of mobile users at the current sensing period, 
while under incomplete asymmetric information, the SP cannot observe the exact sensing costs of mobile users at the current sensing period.

It is easy to see that under complete information or incomplete symmetric information, to minimize the total payment, the SP will pay a mobile user (who is chosen as data source) such a payment that is exactly same as the user's sensing cost (i.e., the minimum payment that the user will accept). 
Under asymmetric incomplete information, however, the SP needs to provide certain incentive mechanism to ensure mobile users truthfully reveal their sensing costs. 
To achieve this goal, the payment to a mobile user may be higher than the user's sensing cost (which is usually referred to as \emph{information rent} in economics).

\subsection{Complete Information -- Benchmark}	

Under complete information, the SP knows the exact sensing costs of all mobile users at all sensing periods in advance. Thus, the SP is able to determine the optimal data source selection and the corresponding payment in an off-line manner.

Let $b_n^{(t)} \in \{0,1\}$ denote whether a mobile user $n$ is chosen as data source at sensing period $t$.
Then, the payment to mobile user $n$ at sensing period $t$ is $\pi_n^{(t)} = b_n^{(t)} \cdot c_n^{(t)}$. 
The SP's payment minimization problem is
\begin{equation}\label{opt-comp}
\begin{aligned}
\min_{\{b_n^{(t)}, \forall n,\forall t\}} &\quad \sum_{n=1}^N \sum_{t=1}^T b_n^{(t)} \cdot c_n^{(t)} 
\\
\mbox{s.t.} & \quad \mbox{(a) } b_n^{(t)} \in \{0,1\},\quad \forall n\in\{1,...,N\},\ t\in\{1,...,T\},
\\
& \quad \mbox{(b) }  \sum_{n=1}^N b_n^{(t)} \geq K, \quad \forall t\in\{1,...,T\},
\\
& \quad \mbox{(c) }  \frac{1}{T} \cdot\sum_{t=1}^T b_n^{(t)} \geq \dpr_n, \quad \forall n\in\{1,...,N\}.
\end{aligned}
\end{equation}
The second constraint (b) is the SP's sensing requirement, and the third constraint (c) is the mobile user's participatory constraint.
It is easy to see that the above problem is an integer programming, and thus can be solved by classic KKT analysis. 

\subsection{Incomplete Symmetric Information}	

Under incomplete symmetric information, the SP knows the exact sensing costs of all mobile users at the current sensing period, but not those at the future sensing periods. 
Thus, the optimal data source selection and the corresponding payment cannot be determined in an off-line manner.
In this section, we will first show that the problem can be formulated as a convex programming problem, which minimizes the SP's expected payment based on the stochastic distribution of mobile user's sensing cost.
Solving this problem requires the explicit knowledge about the distribution information.  
Then we will provide an on-line scheduling policy that achieves the expected payment minimization solution without the above distribution information.

\subsubsection{Convex Programming Problem Formulation}
For convenience, we consider such a scenario where each user's sensing cost is independently and identically distributed (iid) at different sensing periods. 
Moreover, we assume that different mobile users' sensing costs are independent with each other, but may follow different distributions.
Let $f_n(c)$ denote the probability distribution function (pdf) of mobile user $n$'s sensing cost. 
Then, the pdf of the sensing cost vector $\bc = \{c_1,...,c_N\}$ of all mobile users can be written as $g(\bc) \eq f_1(c_1)\cdot...\cdot f_N(c_N)$.\footnote{\rev{\small Here we omit the superscript $^{(t)}$ as we are not talking about the sensing cost at a particular sensing period.}}

Let $b_n(\bc) \in \{0,1\}$ denote whether to choose mobile user $n$ as data source under the sensing cost vector $\bc$. Then the probability of choosing mobile user $n$ as data source is 
$$
q_n = \int_{\bc\in\BC}  b_n(\bc)\cdot g(\bc) \dd \bc,
$$
where $\BC$ is the set of all possible sensing cost vector $\bc$.
The expected payment to mobile user $n$ when it is chosen as data source is
$$
\pi_n = \int_{\bc\in\BC}  b_n(\bc)\cdot c_n \cdot g(\bc) \dd \bc.
$$
The SP's expected payment minimization problem is
\begin{equation}\label{eq:opt-incomp}
\begin{aligned}
\min_{\{b_n(\bc), \forall n,\forall \bc \}} &\quad  \Pi \eq \sum_{n=1}^N \int_{\bc\in\BC}  b_n(\bc)\cdot c_n \cdot g(\bc) \dd \bc 
\\
\mbox{s.t.} & \quad \mbox{(a) } b_n(\bc) \in \{0, 1\},\quad
 \forall \bc\in\BC,\ \forall n\in\{1,...,N\},
\\
& \quad \mbox{(b) }  \sum_{n=1}^N b_n(\bc) \geq K, \quad \forall \bc\in\BC,
\\
& \quad \mbox{(c) }  \int_{\bc\in\BC}  b_n(\bc)\cdot g(\bc) \dd \bc \geq \dpr_n, \quad \forall n\in\{1,...,N\}.
\end{aligned}
\end{equation}
Obviously, the above problem is an integer (convex) programming with infinite decision variables. We can solve  this problem by the KKT analysis. 
However, solving the above problem requires the explicit knowledge about the distribution information, i.e., $g(\bc)$, which is difficult to be obtained in practice. 
This motivates us to study an on-line scheduling policy that does not rely on the distribution information. 


\subsubsection{Dual-decomposition
 Based On-line Scheduling Policy}
Now we will provide an on-line scheduling policy that achieves the expected payment minimization solution. This scheduling policy requires only the current network information and the past scheduling history. Namely, it does not need any information about the distribution of the mobile user's sensing cost. 

The on-line scheduling policy is based on the dual decomposition. 
Specifically, introduce a Lagrange multiplier (also called shadow price) $\lambda_n$ for each constraint (c) in problem (\ref{eq:opt-incomp}), i.e., $\int_{\bc\in\BC}  b_n(\bc)\cdot g(\bc) \dd \bc \geq \dpr_n$.
Then, the Lagrangian for the optimization problem (\ref{eq:opt-incomp}) is 
$$
L(\boldsymbol{b}(\cdot), \boldsymbol{\lambda}) = 
\sum_{n=1}^N \int_{\bc\in\BC}  \big(b_n(\bc)\cdot c_n  - b_n(\bc)\cdot \lambda_n  \big) \cdot g(\bc) \dd \bc  + \sum_{n=1}^N  Q_n \cdot \lambda_n,
$$
where $\boldsymbol{b}(\cdot) = \{b_1(\bc), b_2(\bc),...,b_N(\bc)\}_{\forall \bc }$ denotes the vector consisting of all scheduling strategies, and $\boldsymbol{\lambda} = \{\lambda_1,\lambda_2, ...,\lambda_N\}$ denotes the vector consisting of all shadow prices.

By the duality principle, the Lagrangian dual function is defined as the minimum value of the above Lagrangian over $\boldsymbol{b}(\cdot)$, i.e., 
$$
D(\boldsymbol{\lambda}) = \inf_{\{b_n(\bc), \forall n,\forall \bc \}} 
L(\boldsymbol{b}(\cdot), \boldsymbol{\lambda}),\quad \mbox{s.t. constraints (a) and (b) in (\ref{eq:opt-incomp}).}
$$

Suppose strong duality holds. Then, we further have:
$$
 D(\boldsymbol{\lambda}^*)
 \eq
 \max_{\boldsymbol{\lambda} \geq 0} D(\boldsymbol{\lambda})
 =
   \max_{\boldsymbol{b}(\cdot)} \Pi(\boldsymbol{b}(\cdot))
    \eq
 \Pi(\boldsymbol{b}^*(\cdot)).
$$

The on-line scheduling policy consists of two steps.
First, it continuously updates the shadow prices $\lambda_n$ and other necessary information (such as the probability $q_n$ of choosing each mobile user $n$). Such information essentially captures the past scheduling history. 
Second, it optimally selects a set of mobile users at each sensing period based on the current network information and the shadow prices (and possibly other necessary information mentioned above).
For convenience, let $\lambda_n^{(t)}$ denote the shadow price (associated with the user $n$'s participatory constraint) at the sensing period $t$, and  $q_n^{(t)} = \frac{1}{t} \cdot\sum_{s=1}^t b_n^{(s)} $ denote the probability of choosing mobile user $n$ as data source at the first $t$ sensing periods.

The basic idea of the on-line scheduling policy is following. 
%The basic idea of the on-line scheduling policy is based on the dual decomposition. 
%First, introduce a shadow price $\lambda_n$, and define a virtual cost $\vc_n = c_n - \lambda_n$ for each mobile user $n$. 
First, define a virtual cost 
$$\vc_n^{(t)} = c_n^{(t)} - \lambda_n^* $$ 
for each mobile user $n$. 
Second, at each sensing period $t$, the SP either (i) chooses $K$ mobile users with the minimal virtual cost as data sources if the $(K+1)$th smallest virtual cost is larger than zero, or (ii) otherwise,  chooses all mobile users with the negative virtual cost.
Third, at each sensing period $t$, update the shadow prices in the following way:
$$
\lambda_n = [\lambda_n - \Delta\cdot ( q_n^{(t)} - Q_n)]^+, \quad \forall n\in \N,
$$
where the stepsize $\Delta$ is a small positive number.


\subsubsection{Lyapunov-Based On-line Scheduling Policy}
Now we will provide a different on-line scheduling policy which is based on the Lyapunov approach for stochastic optimization problem. 
Similarly, this scheduling policy requires only the current network information and the past scheduling history. 
Namely, it does not need any information about the distribution of the mobile user's sensing cost. 

To fit the Lyapunov formulation, we assume a long enough time interval, e.g., $T \rightarrow\infty$. 
Moreover, we introduce a new decision variable $a_n^{(t)} \in \{0,1\}$ to denote whether a mobile user $n$ is \emph{not} chosen as data source at sensing period $t$. That is, $b_n^{(t)} \in \{0,1\} = 1- a_n^{(t)} \in \{0,1\}$.
Then, the SP's payment minimization problem given in (\ref{opt-comp}) can be rewritten as the following expected payment minimization problem
\begin{equation}\label{opt-lya}
\begin{aligned}
\min_{\{a_n^{(t)}, \forall n,\forall t\}} &\quad \sum_{n=1}^N \sum_{t=1}^T (1-a_n^{(t)}) \cdot c_n^{(t)} 
\\
\mbox{s.t.} & \quad \mbox{(a) } a_n^{(t)} \in \{0,1\},\quad \forall n\in\{1,...,N\},\ t\in\{1,...,T\},
\\
& \quad \mbox{(b) }  \sum_{n=1}^N (1-a_n^{(t)}) \geq K, \quad \forall t\in\{1,...,T\},
\\
& \quad \mbox{(c) } \lim_{T\rightarrow \infty} \frac{1}{T} \cdot\sum_{t=1}^T (1-a_n^{(t)}) \geq \dpr_n, \quad \forall n\in\{1,...,N\}.
\end{aligned}
\end{equation}
The limitation operation in the last constraint is used to meet the time-average constraint of the Lyapunov formulation.   
With a simple transformation, we can transform the above problem into the following problem
\begin{equation}\label{opt-lya}
\begin{aligned}
\max_{\{a_n^{(t)}, \forall n,\forall t\}} &\quad \sum_{n=1}^N \sum_{t=1}^T a_n^{(t)} \cdot c_n^{(t)} 
\\
\mbox{s.t.} & \quad \mbox{(a) } a_n^{(t)} \in \{0,1\},\quad \forall n\in\{1,...,N\},\ t\in\{1,...,T\},
\\
& \quad \mbox{(b) }  \sum_{n=1}^N a_n^{(t)} \leq N- K, \quad \forall t\in\{1,...,T\},
\\
& \quad \mbox{(c) } \lim_{T\rightarrow \infty} \frac{1}{T} \cdot\sum_{t=1}^T a_n^{(t)} \leq 1 - \dpr_n, \quad \forall n\in\{1,...,N\}.
\end{aligned}
\end{equation}
Obviously, this is an stochastic optimization with time-average constraint. Thus, we can use the Lyapunov approach to solve the problem in an online manner without the prior knowledge about the stochastic distribution information. The detailed process is as follows.

First, we introduce a \emph{virtual queue} for every user $n$, denoted by $G_n$. For convenience, let $G_n^{(t)}$ denote the size of the virtual queue in the sensing period $t$. 
Then, in every sensing period $t$, the SP solves the following single-period optimization problem: 
\begin{equation}\label{opt-lya-drift}
\begin{aligned}
\min_{\{a_n^{(t)}, \forall n \}} &\quad 
\sum_{n=1}^N  a_n^{(t)} \cdot G_n^{(t)} - 
V \cdot \sum_{n=1}^N a_n^{(t)} \cdot c_n^{(t)} 
\\
\mbox{s.t.} & \quad \mbox{(a) } a_n^{(t)} \in \{0,1\},\quad \forall n\in\{1,...,N\},
\\
& \quad \mbox{(b) }  \sum_{n=1}^N a_n^{(t)} \leq N- K,
\end{aligned}
\end{equation} 
where $V$ is a parameter used to tradeoff the virtual queue length (reflecting the converging time) and the performance gap  between the online scheduling and the offline benchmark.
It is easy to see that the optimal solution of (\ref{opt-lya-drift}) is to (i) \emph{exclude} the first $N-K$ mobile users with the smallest and negative $(G_n^{(t)} - V\cdot c_n^{(t)})$ as data sources (if the $(N-K+1)$th smallest $(G_n^{(t)} - V\cdot c_n^{(t)})$ is smaller than zero), or (ii) otherwise, \emph{exclude} all of $N'$ (where $N' \leq N-K$) mobile users with the negative $(G_n^{(t)} - V\cdot c_n^{(t)})$ as data sources (if the $(N-K+1)$th smallest $(G_n^{(t)} - V\cdot c_n^{(t)})$ is larger than zero). 
After getting the optimal solution of (\ref{opt-lya-drift}), i.e., $a_n^{(t)*}, n=1,...,N$, we can immediately obtain the following scheduling for sensing period $t$: $b_n^{(t)*} = 1- a_n^{(t)*}, n=1,...,N$.
Finally, the virtual queue of each mobile user $n$ is updated according to the following way:
$$
G_n^{(t+1)} = \left[ G_n^{(t)} - (1-Q_n) \right]^+ + a_n^{(t)},
$$
where $[x]^+ = \max\{x, 0\}$.

Formally, we summarize the Lyapunov-Based online scheduling policy in Algorithm 1. 


\begin{algorithm}[h]
\label{algo:rule}
\small
\caption{Lyapunov-Based Online Scheduling Policy}
\DontPrintSemicolon
Initialize the virtual queue of every user $n$: $G_n^{(1)} = 0, \ \forall n=1,...,N $; \;
\For{each sensing period $t = 1,...,T$}
{
Every user $n$ reports its instantaneous sensing cost: $c_n^{(t)}, \forall n = 1,...,N$; 
\\
The SP solves the single-period optimization problem (\ref{opt-lya-drift}): $a_n^{(t)}, \ \forall n=1,...,N$;
\\
The SP chooses the users as data sources: $b_n^{(t)} = 1 - a_n^{(t)},\ \forall n=1,...,N$;
\\
Update the virtual queue of every user $n$: $G_n^{(t+1)} = \left[ G_n^{(t)} - (1-Q_n) \right]^+ + a_n^{(t)}, \ \forall n=1,...,N $. \;
}
\end{algorithm}


\begin{theorem}
Algorithm 1 converges to the optimal solution of problem (\ref{eq:opt-incomp}).
\end{theorem}

\subsubsection{Performance Evaluation}
Now we provide simulations to illustrate the performance of the above two online scheduling approaches.

\begin{table}[h]
\small\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$T_q$ (Dual) & $V$ (Lyapunov) & Offline Benchmark & Dual  (stable) & Dual (actual) & Lyapunov (stable) & Lyapunov (actual) \\
\hline
 1 & 10 & 0.9428 & 0.9432 & 0.9290  & 1.0559 & 1.0481
 \\
\hline
 10 &  20 &   0.9428&    0.9429 &   0.9285 &   0.9935 &   0.9860
 \\
\hline
 20 &  50 &      0.9428   & 0.9459  &  0.9293  &  0.9649 &   0.9462
 \\ 
\hline 
50 &  100 &   0.9428   & 0.9417  &  0.9291   & 0.9554  &  0.9216
\\
\hline
 100 &  200 &       0.9428&    0.9448 &   0.9327&    0.9512  &  0.8879
 \\
\hline
\end{tabular}
\end{table}

\subsection{Incomplete Asymmetric Information}
It is notable that in the previous incomplete symmetric information scenario, the SP knows the exact sensing costs of all mobile users at the current sensing period (but not those at the future sensing periods). In practice, however, the SP may not know the current sensing costs of mobile users, as the sensing costs are private information of mobile users, and are known only to their respective owner.	
Therefore, when applying either online scheduling policy derived in the above section, a proper mechanism that effectively eliciting the users' sensing costs is necessary. 

Let us take the Lyapunov-based online scheduling policy as an illustration. We will show how to design an auction to credibly elicit mobile users' sensing costs, and meanwhile 
achieve the optimal online scheduling. 
Notice that an auction includes an allocation rule (winner determination) and a payment rule. Next we will study the allocation rule and the payment rule systematically. 

\emph{Allocation Rule.} To achieve the optimal online scheduling, the allocation rule must solve the single-period optimization problem (\ref{opt-lya-drift}).
With simple transformations, we have the following allocation problem for the auction:
\begin{equation}\label{opt-lya-drift-xx}
\begin{aligned}
\max_{\{a_n^{(t)}, \forall n \}} &\quad 
\sum_{n=1}^N  a_n^{(t)} \cdot (c_n^{(t)} - g_n^{(t)} ) 
\\
\mbox{s.t.} & \quad \mbox{(a) } a_n^{(t)} \in \{0,1\},\quad \forall n\in\{1,...,N\},
\\
& \quad \mbox{(b) }  \sum_{n=1}^N a_n^{(t)} \leq N- K,
\end{aligned}
\end{equation} 
where $g_n^{(t)} = \frac{G_n^{(t)}}{V}$. 
Note that $c_n^{(t)}$ is the private information of mobile user $n$ and not known by the SP, while $g_n^{(t)}$ is maintained by the SP and is the private information of the SP. 
For convenience, we denote $(c_n^{(t)} - g_n^{(t)} )$ as the \emph{shifted cost} of user $n$.

It is easy to see that the allocation rule given by problem (\ref{opt-lya-drift-xx}) is to \emph{(i) select the $N-K$ users with the largest and positive shifted cost as winner, or (ii) select all users with the positive shifted cost as winner if there are less than $N-K$ users with the positive shifted cost.}

From the allocation problem (\ref{opt-lya-drift-xx}), we can see that the proposed auction differs from the traditional auction in the following aspects. 
\begin{itemize}
\item
First, in a traditional auction, the allocation rule is usually used to optimize the sum of user costs or valuations. 
In our proposed auction, the allocation rule is used to optimize the sum of the \emph{shifted} costs, where each user $n$'s cost $c_n^{(t)}$ is shifted by a factor $g_n^{(t)}$. This will affect the design of the payment rule. 

\item 
Second, in a traditional auction, a winner is usually assigned an item or selected to perform certain task. Accordingly, the winners can gain certain benefit and meanwhile be charged by certain money, or suffer certain cost and meanwhile be paid by certain money. The losers gain/suffer nothing, and be charged/paid by nothing. 
In the our auction, however, a winner of the above allocation rule is \emph{not} selected to perform the sensing task, while a loser is actually selected to perform the sensing task. Accordingly, the losers will suffer the sensing cost, and are expected to be paid by certain money.
\end{itemize}
 
\emph{Payment Rule.} Now we provide the payment rule such that all mobile users are willing to truthfully reveal their private information.  
Specifically, the payment rule is following: \emph{(i) the payment to each winner $n$ (i.e., $a_n^{(t)} = 1$) is $p_n^{\textsc{win}} = 0$, as a winner will not be selected to perform the sensing task, and (ii) the payment to each loser $n $ (i.e., $a_n^{(t)} = 0$) is $p_n^{\textsc{loss}} =  g_n^{(t)} + \underline{c} $, where $\underline{c} $ is the minimum shifted cost of all winners.}

\begin{theorem}
The auction with the above allocation rule and payment rule is truthful.  
\end{theorem}

\begin{proof}
We first prove that each mobile user $n$ has no incentive to bid a sensing cost $c_n'$  lower than its real sensing cost $c_n$, i.e., $c_n' \leq c_n$. There are several cases:
\begin{enumerate}
\item
Win at $c_n$ and $c_n'$. The payment to user $n$ is zero under both the truthful bid $c_n$ and non-truthful bid $c_n'$. Thus, the user's surplus is zero under both bids. 
\item
Loss at $c_n$ and $c_n'$. The payment to user $n$ is $g_n + \underline{c} $ under both the truthful bid $c_n$ and non-truthful bid $c_n'$. Thus, the user's surplus is $g_n + \underline{c} - c_n$ under both bids.  
\item 
Win at $c_n$ but loss at $c_n'$. 
When biding truthfully, user $n $ wins, and the payment to user $n$ is zero, and the user's surplus is also zero. 

Suppose user $n$ is \emph{not} the last winner (with the smallest shifted cost), i.e., $c_n - g_n > \underline{c}$.
When biding $c_n'$, user $n$ losses, and the payment to user $n$ is $g_n + \underline{c}$, and the user's surplus is $g_n + \underline{c} - c_n < 0$. 

Suppose user $n$ is the last winner, i.e., $c_n - g_n = \underline{c}$. Denote $\underline{c}^{\dag}$ as the shifted cost of the first loser, and obviously $\underline{c}^{\dag} < \underline{c}$.
When biding $c_n'$, user $n$ losses and the first loser wins, and the payment to user $n$ is $g_n + \underline{c}^{\dag}$, and the user's surplus is $g_n + \underline{c}^{\dag} - c_n = \underline{c}'- \underline{c} < 0$.
\end{enumerate}

We next prove that each mobile user $n$ has no incentive to bid a sensing cost $c_n'$ larger than its real sensing cost $c_n$, i.e., $c_n' \geq c_n$. There are several cases:
\begin{enumerate}
\item
Win at $c_n$ and $c_n'$. The payment to user $n$ is zero under both the truthful bid $c_n$ and non-truthful bid $c_n'$. Thus, the user's surplus is zero under both bids. 
\item 
Loss at $c_n$ and $c_n'$. The payment to user $n$ is $g_n + \underline{c} $ under both the truthful bid $c_n$ and non-truthful bid $c_n'$. Thus, the user's surplus is $g_n + \underline{c} - c_n$ under both bids.  
\item 
Loss at $c_n$ but win at $c_n'$. 
When biding truthfully, user $n $ losses, and the payment to user $n$ is $g_n + \underline{c} $, and the user's surplus is $g_n + \underline{c} - c_n \geq 0$. 
When biding $c_n'$, user $n$ wins, and the payment to user $n$ is zero, and the user's surplus is also zero. 
\end{enumerate}

\end{proof}

\textbf{Remaining problems in the auction design: }

1. The above auction is designed for the sensing cost minimization, not for the SP's revenue maximization. The latter is more challenging, as we need to design an optimal reservation price for the SP, which may be mathematically intractable. (I wonder if we can use the objective of sensing cost minimization?)

2. There is a key assumption: mobile users are myopic, in the sense that in a particular sensing period, they only focus on the 
payoff at the current sensing period, but not consider the potential impacts of the current strategies on the future payoff. 

\rev{\emph{Remark 1:} 
Based on the previous meeting, we feel that the second assumption (myopic assumption for mobile users) is acceptable.}

\rev{\emph{Remark 2:} 
As for the first issue, it might be challenging and even mathematically intractable to study the revenue maximization auction design. The reasons are as follows. First, a revenue maximization auction requires to solve a complicated optimization problem (to obtain the best reservation price for the auctioneer), which is challenging even for a simplest second-price auction with homogeneous bidders. In our case, the mobile users may not be homogeneous, and the auction design is much complicated than a second-price auction. Thus, in my feeling, it is hard (even impossible) to obtain the close-form best reservation price or a good approximation. Second, the calculation of the best reservation price requires the stochastic distribution information of all bidders' cost information. However, this distribution information is not known by the SP in our model (this is the key motivation for our online scheduling policy).

Moreover, the key motivation for the sensing cost minimization (which is equivalent to the social welfare maximization) is the following one. We can image the SP as a government organization (e.g., Weather Bureau or Ministry of Transportation), whose objective is to collect certain data for the public usage.}


\rev{
\subsection{Model Extension}

To capture the features of a real sensing system, we need to consider the following potential extensions in the model. 

\subsubsection{Network Topology Extension}
Instead of considering the number of scheduled users only, the SP needs to consider the conflict relationship among users. For example, the nearby users should not be scheduled at the same time, since their sensing data are highly reduplicative. 

Key Idea: We  can use a conflict graph $\I = \{I_{ij}\}_{i=1,...,N;j=1,...,N}$ to denote the conflict relationship among mobile users, where $I_{ij}\in\{0,1\}$ denotes whether mobile users $i$ and $j$ are conflict with each other.  
Then, instead of finding $K$ arbitrary mobile users in each sensing period, we need to find \emph{a subset of mobile users with at least $K$ independent users.}


\subsubsection{Sensing Quality Differentiation}
The SP may have  different evaluations for the sensing data from different mobile users, for example, due to the different sensing efforts of users, or different locations of users. 

Key Idea: We can use an additional parameter $v_n^{(t)}$ to denote the value (quality) of mobile user $n$'s sensing data at sensing period $t$. 
Then, instead of considering the sensing cost $c_n^{(t)}$ only (i.e., minimizing the total sensing cost) in the scheduling decision, we need to consider both the sensing value and the sensing cost in the scheduling decision (e.g., maximizing the difference between the total value and total cost).

\subsubsection{Elastic Sensing Requirement}
Instead of requesting a fixed $K$ sensing data at each period, the SP has an elastic sensing requirement, where $K$ is no longer fixed but a decision variable. Accordingly, the benefit from the sensing data is a generic concavely increasing function of the number of scheduled users (i.e., $K$) as well as the SP's evaluations for the scheduled users' data. 

Solution: 
Let $U(\bb^{(t)})$ denote the benefit of the SP (called \emph{utility})  under the scheduling decision $\bb^{(t)} = \{b_1^{(t)}, ..., b_N^{(t)}\}$ at the sensing period $t$. 
Then, the SP's objective becomes $U(\bb^{(t)}) - C(\bb^{(t)})$, where $C(\bb^{(t)})$ is the total sensing cost of all scheduled users. 
}

\subsection{A New Model}

\subsubsection{Limitation of the above model extensions}
However, we find that the conflict graph cannot capture the \emph{partial conflict relationship} among mobile users, which is very important in a real sensing system. 
For example, in a real system, two mobile users' sensing data may not be  fully reduplicative, but partially reduplicative. 
A natural idea is to use a weighted conflict graph, where the conflict relationship among every two users $m$ and $n$ is associated with a weight $\rho_{mn}$ which reflects the conflict level among them. 
Then, the total value from two users (say $m$ and $n$) can be simply defined as $(v_m+v_n)\cdot \rho_{mn}$. 
However, it is still hard to define the total value from a set of  more than 2 users. 

\subsubsection{A new model}
To this end, we propose a new model, which can not only capture the above three features, but can also capture the partial conflict relationship among mobile users. 
As shown in Figure \ref{fig:model}, we consider a total sensing area $\AR$, which is divided into many small grids $\AR_i, i=1,...,I$. A grid is the minimum sensing unit/area, e.g., a square with $10$m$\times 10$m. Each grid $\AR_i$ is associated with a weight $w_i$, which reflects the different importances of the grids.  For example, a grid in the downtown area may be more important than a grid in the suburban area, and thus has a larger weight. 

Mobile users may  have different sensing ranges, depending on their sensing efforts and other factors such as the terrains and device capabilities. Let $d_{n,i}^{(t)}\in\{0,1\}$ denote whether the grid $i$ is within mobile user $n$'s sensing range in the period $t$. The value of a mobile user $n$'s sensing data is defined as the aggregate weight of its covered sensing area, i.e., 
$$
v_n^{(t)} = \sum_{i=1}^I d_{n,i}^{(t)} \cdot w_i.
$$
Notice that mobile users move randomly across sensing periods, and thus the sensing area of each user changes accordingly. That is, $d_{n,i}^{(t)}$ changes randomly in different periods. 



Accordingly, the total value of a set of mobile users' sensing data is defined as the aggregate weight of the total sensing area of these users. 
Notice that different mobile users' senseng areas may be overlapped, e.g., those of MU 3 and MU 4 in Figure \ref{fig:model}. This essentially captures the partial conflict relationship among mobile users. 
Take MU 3 and MU 4 in Figure \ref{fig:model} as an illustration, where MU 3 covers 20 grids (assuming each with a unit weight), and MU 4 covers 9 grid (assuming each with a unit weight). 
Then, (i) when scheduling MU 3 only, the value of MU 3's sensing data is $v_3 = 20$, (ii) when scheduling MU 4 only,  the value of MU 4's sensing data is $v_4 = 9$, and (iii) when scheduling MU 3 and MU 4 concurrently, the value of their sensing data is $v_{3,4} = 20 + 9 - 3 = 26$, since there are 3 grids covered by both users' sensing ranges (hence can only be counted once). 

It is easy to show that this model captures the following two features: (partial) conflict relationship among users and sensing quality differentiation. 
Besides, by assuming that the SP allows different number of sensing data in each period, and 
tries to maximize the difference between the total sensing value (utility) and the total sensing cost, this model captures the feature of elastic sensing requirement for the SP. 

\subsubsection{Complete Information -- Benchmark}

With this new model, the SP's optimization problem  under the complete information is the following:
\begin{equation}\label{opt-comp-new}
\begin{aligned}
\max_{\{b_n^{(t)}, \forall n,\forall t\}} &\quad \sum_{t=1}^T U(\bb^{(t)}) - C(\bb^{(t)}) 
\\
\mbox{s.t.} & \quad \mbox{(a) } b_n^{(t)} \in \{0,1\},\quad \forall n\in\{1,...,N\},\ t\in\{1,...,T\},
%\\
%& \quad \mbox{(b) }  \sum_{n=1}^N b_n^{(t)} \geq K, \quad \forall t\in\{1,...,T\},
\\
& \quad \mbox{(b) }  \frac{1}{T} \cdot\sum_{t=1}^T b_n^{(t)} \geq \dpr_n, \quad \forall n\in\{1,...,N\},
\\
& \quad \mbox{(c) }  U(\bb^{(t)})  \triangleq \sum_{i=1}^I d_i^{(t)} \cdot w_i, \quad d_i^{(t)} = \textbf{1}_{\sum_{n=1}^N  b_n^{(t)}\cdot d_{n,i}^{(t)} \geq 1},
\\
& \quad \mbox{(d) } C(\bb^{(t)})  \triangleq \sum_{n=1}^N b_n^{(t)} \cdot c_n^{(t)},
\end{aligned}
\end{equation}
where $d_i^{(t)} = \textbf{1}_{\sum_{n=1}^N b_n^{(t)}\cdot  d_{n,i}^{(t)} \geq 1}$ denotes that $d_i^{(t)} = 1$ if $\sum_{n=1}^N d_{n,i}^{(t)} \geq 1$, and $d_i^{(t)} = 0$ if $\sum_{n=1}^N b_n^{(t)}\cdot  d_{n,i}^{(t)} =0$, which indicates whether the grid $\AR_i$ is sensed by at least one user. 



==> section2-literature-xx.tex <==
%!TEX root = sum_reference.tex
%SourceDoc sum_reference.tex

 

\section{Literature Review}\label{sec:literature}



\subsection{J. Burke (2006) -- \comm{The first paper}}

\ctra{
[e1] J. Burke, D. Estrin, M. Hansen, A. Parker, N. Ramanathan, S. Reddy,
and M. B. Srivastava, ``Participatory sensing,'' in In: Workshop on
World-Sensor-Web (WSW06): Mobile Device Centric Sensor Networks
and Applications, 2006, pp. 117-134.
}

\ab

This paper introduces the concept of participatory sensing, which
tasks everyday mobile devices, such as cellular phones, to form
interactive, participatory sensor networks that enable public and
professional users to gather, analyze and share local knowledge.
An initial architecture to enhance data credibility, quality, privacy
and ÔshareabilityÕ in such networks is described, as well as a
campaign application model that encompasses participation at
personal, social and urban scales. Example applications are
outlined in four areas: urban planning, public health, cultural
identity and creative expression, and natural resource
management.


\bg

Two billion people carry mobile phones. These ubiquitous
devices are increasingly capable of capturing, classifying and
transmitting image, acoustic, location and other data, interactively
or autonomously. Given the right architecture, they could act as
sensor nodes and location-aware data collection instruments. The
idea of a wireless sensor network is not new; we are already able
to integrate sensing, computation and connectivity in low-power
devices and embed networks of them in the physical world to
collect data. Through physical proximity to what they study,
multiscale operation and adaptive, autonomous observation,
embedded sensor networks allow the observation of previously
unobservable phenomena. From research and deployment, we
know something about what distributed sensing can be used for in
the sciences, industry and the military. We know much less about
its function and utility in the public sphere when the components
are owned and operated by everyday users. As sensors, networkconnected
mobile handsets will be embedded near the ultimate
elusive subjects: people and their built environments. Instead of
being in the hands of a central observer, these sensors are alwayson
and under their ownersÕ control. Leveraging them effectively
and conscientiously will require models that prioritize user
participation in sensing.

Participatory sensing will task deployed mobile devices to
form interactive, participatory sensor networks that enable public
and professional users to gather, analyze and share local
knowledge. Microphones and imagers on-board the mobile
handsets can record environmental data now, while in the future
other sensors will be integrated or connect wirelessly. Cell tower
localization, GPS and other technologies can provide location and
time-synchronization data. Wireless radios and onboard
processing enable human interaction with both local data
processing and remote servers. With these capabilities in mind,
new network architecture is described below that enhances data
credibility, quality, privacy and ÔshareabilityÕ, encouraging
participation at personal, social and urban scales.

 


\newpage

\subsection{Buster O. Holzbauer (2014) -- \comm{Book}}

\ctra{
{[R2]
Buster O. Holzbauer, 
Boleslaw K. Szymanski, and 
Eyuphan Bulut, 
``Incentivizing
Participatory Sensing via
Auction Mechanisms'',
Chapter in \emph{Opportunistic Mobile Social Networks}, 
Taylor and Francis, CRC Press, 2014. }
}

\ab

With the increasing availability of smart phones and other mobile devices with sensing
capabilities, a class of problems known as participatory sensing is becoming
increasingly popular. Participatory sensing refers to a sensing system in which humans
voluntarily participate in the system, actively contributing to sensing, either
by passively carrying devices or actively engaging in sensing. With respect to opportunistic
networks, humans provide mobility and decision-making difficult to implement
in dedicated sensor networks. Participatory sensing is also a more scalable
solution since the costs are far lower than the costs associated with deploying a dedicated
larger or computationally intensive sensor network. However, by involving
humans, many issues must be addressed in designing a participatory sensing system.
In this chapter we discuss several issues in participatory sensing system design,
then introduce several papers on existing systems and study lessons that can be applied
towards designing a new system. Finally, we conclude by presenting our own
participatory sensing system and results from its simulations.1

\textbf{1.1 Introduction}

Over the past decade, our ability to gather information about our world has drastically
improved. Technology has allowed for cheaper sensors, better communication,
hardware that can be powered longer, and increasingly mobile sensor networks [1].
This has led to a type of sensor network applications often referred to as participatory
sensing. Specifically, participatory sensing refers to a sensing system in which
humans are carriers for sensing platforms known as `nodes' and voluntarily participate
in the system. Various definitions with varying specifics exist in literature, but
the general consensus is that the problem involves humans directly contributing to
sensing, either by passively carrying devices or actively engaging in sensing.


As mentioned previously, participatory sensing can be viewed as the problem
of using voluntarily contributions from humans and their devices to collect measurements
about a particular phenomenon.More discussion on how a system can leverage
human involvement follows in Section 1.3.


\textbf{1.3 Issues In Participatory Sensing}

Participatory sensing is not without its challenges. Since it is still a type of sensor network,
problems relating to hardware, communication, and application design found
in traditional sensor networks still apply. Mobility is achieved through human movement
[6], but integrating humans into the system introduces several new types of
challenges as well. Before examining a paper on one of these challenges, we outline
some of the key issues and their impact on designing participatory sensing systems.

\textbf{1.3.1 Data}

The purpose of a participatory sensing system is to perform some variety of sensing
task. One of the most obvious design decisions is determining what measurements
are required to achieve the system?s goal, and what hardware is required to support
these measurements. Beyond the basic type of measurements, additional requirements
may be needed such as resolution of data, how often samples are provided,
geographic coverage, etc.


\textbf{1.3.2 Coordination}

An important decision, independent of the types of measurements taken, is who takes
samples and how often. Assuming that privacy is not an issue, there are still several
factors to consider. A simple sensor network deployment design is to have static
sensors that sense and report on a fixed schedule. Without incurring communication
overhead or adding a central controller, such a system cannot react to dynamic
changes or events that cannot be perceived without a global view. If the system is
synchronous, and run by one or more central controllers which dictate which nodes
take measurements and which types of samples to take, these issues can be avoided.
However, this ?client-server? model adds communication overhead, and depending
on the network conditions, can result in significant lag. Either the controller risks
running on an outdated view of the sensors, or sensors may spend time idling while
states are updated and while waiting for instructions from the controller.

Alternatively, decisions could be made by the human operators. To continue with
the aforementioned wildlife detection example, in a synchronous system the controller
might decide to request samples when nodes were known to be close to local
areas of interest, or areas where no information was recorded. Without such a controller,
the nodes might resort to simply taking an image periodically and submitting
a measurement. When considering resource usage, it might be better if users took a
picture when they spotted wildlife or were at a location known to require addition
sampling. Such a user-driven approach is one alternative to having a central coordinator.
Upon examination, the idea of users knowing which locations need additional
data came up. This ties into the challenge in Section 1.3.1, since seeing something
like a report of number of measurements by location is yet another query that might
not be anticipated by a designer who only considered the system?s end-goal. Such
reporting also brings up software engineering challenges in APIs and usability.

A third option is to use a peer-to-peer, or ad hoc, network. In this case there
is little to no structure, and events or queries drive the behavior of the network. A
discussion of ad-hoc techniques is outside the scope of this chapter. While in traditional
sensor networks work has been done on peer-to-peer setups [7], applying the
paradigm of participatory sensing to such networks is an open problem [8].

\textbf{1.3.3 Privacy And Security}

By involving humans in the sensing process, the data that comes out of the system
may reflect information about the participants. In general, this information is not
part of the goals of the sensing task, but is an issue nonetheless. For example, many
sensing tasks involve spatio-temporal context (a time and a place). If the identity
of the user is not adequately protected, then access to reports could reveal exactly
where someone was at a particular time. This constitutes a breach of privacy, and is
undesirable [8].

\textbf{1.3.4 Human Concerns}

In participatory sensing, the device which humans use to sense is often their cellular
device [8, 11]. This may be a feature phone or a smartphone, possibly with additional
sensors interfacing through technologies such as Bluetooth. In all of these cases,
the user has everyday uses for their devices, such as phone calls, messaging, and
a wide variety of apps. These uses require energy, as does running a participatory
sensing system [12]. Thus, supporting the participatory sensing task has a tangible
cost. Furthermore, this cost may not be considered a renewable resource depending
on the timescale, since there is no guarantee about when a user can charge their
device next.

Communication also imposes upon the user. Bandwidth used for participatory
sensing may cause performance degradation in other activities the user would normally
do on their phones. In addition, the users may have a limited amount of data
they are allowed to transmit and receive based on service provider restrictions.

If the sensing task is not passive, then users spend time and effort to contribute
to the it. Users may have a feeling that their time has worth, and justifying the use of
their time towards participatory sensing should be something designers are prepared
to do. In the case of subjective and qualitative metadata added by users, additional
resources may have to be spent to verify user input and manage users.

\textbf{1.3.5 Participants}

The salient feature of participatory sensing is the voluntary participation of users.
Without users, the system cannot survive. Furthermore, humans can act in a variety
of ways that do not benefit the system, such as never contributing, falsifying results,
or providing information that does not satisfy requirements. While we do not discuss
issues in reviewing data or recruitment of users in-depth, research exists in literature
on the topic [13].


Another issue is that since user participation is voluntary, they can stop participating
at any time for any reason. Whether motivation is intrinsic (such as users participating
in a sensing campaign that will better their community) or extrinsic (such
as the system providing compensation for user participation), the system designers
should be aware of what is needed to provide and reinforce motivation [11]. Additionally,
system designers must be aware that participants can start or stop participating
at any time. In Section 1.4 we cover terms and develop ideas about incentive to
support the idea of extrinsic motivation to encourage participation.


\textbf{1.4 Applying Market Mechanisms}

Earlier in the chapter, it was established that persistent participation is essential to
participatory sensing, and that this required potential users to be motivated to use
the system. In Section 1.5, a scheme for participatory privacy regulation will be discussed.
One of the advantages of the approach described in that paper is that by
having users be involved in design, research, and regulation, they are intrinsically
motivated to continue participating. Unfortunately, this kind of involvement is not
always a realizable option. Even in cases where users are involved, incentive that is
extrinsic to the sensing application can help reinforce participation. When users do
not have any personal reason to join a system, or when they avoid a system because of
perceived inconvenience incurred through participation, incentive is a useful tool. To
discuss incentives, we refer to economic and market theory, which is a well studied
subject [14].


In economics, a market is a system with one or more goods. These goods, which
are produced by sellers, have a price associated with them. Buyers purchase goods
from seller in exchange for currency. In this chapter we will consider the currency
to be ?incentive? and do not specify whether it is a monetary or otherwise tangible
reward, or some sort of intangible reward such as points for ranking on a virtual
leaderboard. One way to model participatory sensing with a central controller is to
view it as a buyer of goods which are produced when participants perform sensing
tasks. This makes participants the seller, meaning they place a price on the imaginary
good produced by performing a sensing task. This price may be affected by factors
about the human behind it, such as perceived sensitivity or valuation of their time and
resources. Much like in markets with tangible goods, multiple producers, and supply
exceeding demand, sellers (participants) are forced to compete with each other to try
and sell their goods to a buyer. If participation is sufficient, this supply and demand
relationship can be met and competition affects prices. Otherwise, the only limiting
factor is budget of buyers (sensing applications).


Deciding how to set prices under competition is not a trivial problem, however
before addressing this issue we examine another problem. How sellers and buyers
interact must be defined to have any idea what sorts of strategies a buyer or seller
might take to try andmaximize their utility. Utility for a seller is the price paid less the
cost of producing the good. For a buyer, the utility is their valuation of the good they
wish to buy less the price they pay. Since buyers and sellers in a participatory sensing
campaign have an interest in the same types of goods, we can apply the concept
of an auction. In an auction, an auctioneer requests bids, and provides a good in
exchange for payment from a winner selected by the auctioneer. In a reverse auction,
the auctioneer still collects bids and selects a winner. However, the auctioneer gives
the winner a payment and receives a good in exchange. While reverse auctions are
not the only way to leverage incentive, they are the way our approach (discussed
at the end of Section 1.6) manages incentive to address participation, inspired by
Lee and Hoh?s work described next. The auction model considers buyers and sellers
interacting directly, however other successful incentive mechanisms have been used,
such as recursive incentive [15].


\ctra{
[x] Holzbauer, Buster O., Boleslaw K. Szymanski, and Eyuphan Bulut. "Socially-aware market mechanism for participatory sensing." In Proceedings of the first ACM international workshop on Mission-oriented wireless sensor networking, pp. 9-14. ACM, 2012.
}

By using personal mobile devices, participatory sensing pro-
vides an alternative to deploying dedicated mobile nodes to
perform data acquisition tasks in areas where human car-
riers are already present. However, this application comes
with some unique challenges. In this paper, we study the
challenges resulting from social concerns of participants in
a participatory sensing application and propose a socially
aware auction mechanism to address them. Through simu-
lations, we compare the proposed mechanism to several ex-
isting mechanisms. The results demonstrate that, with the
right configuration, our proposed mechanism can decrease
the cost for the data sinks and decrease the privacy loss and
battery usage of participants while preserving their partici-
pation.

Participatory sensing relies on participants contributing
observed data to build a data collection [1] [2]. It can also be
considered as a potentially commercializable or voluntary-
based type of a distributed sensor or mobile network.
There are many examples of participatory sensing applica-
tions in real-world [3] [4] [5]. We specifically focus on the set
of applications where there is a sensing campaign with the
objective of maintaining a set of sufficiently recent sensor
readings (such as vehicle emissions) from adequately cov-
ered area. Since mobility is an energy-intensive activity, we
rely on human mobility to move the sensors. Smartphones
with sensing capabilities are examples of devices that are
routinely carried by people. Thus, in this paper we consider
the sensor platform to be personal phones and mobility to
be restricted to human mobility.



Human-centric sensing invokes several challenges includ-
ing the mitigation of social concerns. One such challenge
is balancing power usage between normal activities such as
phone calls, and sensor readings. Another one is how to over-
come recruitment constraints such as budget restrictions or
human constraints such as motivation, availability, and pri-
vacy. Since applications that we consider in this paper re-
quire data about spatio-temporal coordinates of collection,
privacy is particularly important.


In this paper, we propose to use a reverse auction mecha-
nism to address both the retention of participants and their
social concerns arising from participation (e.g. Figure 1) at
the same time. Participation rewards requires that the fre-
quency of sensing for a participant is not too low while social
concerns require the frequency of sensing is not too high.

\textbf{2.2 Previous Auction Mechanisms}

Next, we will give the details of some auction mechanisms
previously proposed in literature.
First Price Auctions: A classic auction is the first price
sealed bid auction. All participants that are competing for
incentive in a given auction submit bids simultaneously to
provide one of the N required sensor readings. The auc-
tioneer (data sink), which in our example problem is a cell
tower, waits until all bids are received and then select the
N cheapest bids received as winners. This mechanism is
very easy for the auctioneer to run. However, from a par-
ticipant?s standpoint this type of reverse auction is difficult
to understand. Since winners pay what they bid, the bid
cannot reflect their true valuation so the first price reverse
auction is not incentive compatible. The bidding strategy
in a first price auction is dependent on a given participant?s
perception of all other participants? strategies. Making a
decision about what amount to bid is non-trivial and may
deter accurate bidding and participation.

Reverse Auction based Dynamic Price incentive
mechanism with Virtual Participation Credit (RADP-
VPC): RADP-VPC is a modification of the first price auc-
tion that is designed with reverse auctions in mind [8]. For
every consecutive round in which participant loses, the corresponding bid is decreased by constant. The auctioneer
ignores this virtual participation credit when awarding in-
centive, so the participant?s odds of winning are improved
without decreasing payout. The auction is run in all other
aspects like a first price auction. To promote rejoining the
auction by dropped out bidder, the mechanism notifies them
of the highest winning bid in the current round.

Participation Incentive Generalized Vickrey Auc-
tion (PI-GVA): An alternative to the first price auction is
the Generalized Vickrey Auction, which is incentive compat-
ible. The Participation Incentive GVA mechanism computes
for each participant a score that encapsulates the expected
and actual number of times a participant has won, as well as
the corresponding bids [9]. PI-GVA has a parameter ? which
determines the weight of the average bidding term. The auc-
tioneer uses the scores in computing prices for selecting win-
ners. PI-GVA as originally described is a forward auction,
to make it a reverse auction bids are negated and the small-
est scores are used. Despite the complexity compared to the
previous two mechanisms, PI-GVA is easy for participants
to understand if they realize it is incentive-compatible. PI-
GVA also has the desirable property of being effective even
in recurring auctions. This means that the mechanism re-
tains sufficiently many participants to maintain competition
even as participants learn information as the recurrent auc-
tion progresses.

\ct{
[1] Mobile Millennium http://traffic.berkeley.edu.

[2] Nokia Simple Context
https://alpha.nokoscope.com/eb2.

[3] MIT Media Lab: The Owl Project
http://owlproject.media.mit.edu.

[4] Krause, A., Horvitz, E., Kansal, A., and Zhao, F.
Toward community sensing, in IPSN, 2008.

[5] Hoh, B., Gruteser, M., Herring, R., Ban, J., Work, D.,
Herrera, J.C., Bayen, A. M., Annavaram, M., and
JACOBSON, Q. Virtual trip lines for distributed
privacy-preserving traffic monitoring, MobiSys 2008,
Breckenridge, CO.

[6] Srivastava, M., Abdelzaher, T., and Szymanski, B.
2012. Human-centric Sensing. In Transactions of
Royal Society, Series A, 370:176-197.

[7] Reddy, S., Estrin, D., Hansen, M., and Srivastava, M.
2010. Examining Micro-Payments for Participatory
Sensing Data Collections. In International Conference
on Ubiquitous Computing, Denmark, Sept. 2010.

[8] Lee, J., and Hoh, B. Sell Your Experiences: A Market
Mechanism based Incentive for Participatory Sensing.
IEEE PerCom, Mannheim, Germany, March 2010,
60-68.

[9] Lee, J.-S., and Szymanski, B. 2009. A Participation
Incentive Market Mechanism for Allocating
Heterogeneous Network Services. In IEEE Globecom,
Hawaii, Dec. 2009, 1-6.

[10] Danezis, G., Lewis, S., and Anderson, R. How Much is
Location Privacy Worth?, in WEIS ?05:Proceedings of
the Fourth Workshop on the Economics of
Information Security. 2005.
}



\newpage

\subsection{J.-S. Lee (2010) -- \comm{Long-term Participation Incentive}}


\ctra{
[R2.10]
Lee, Juong-Sik, and Baik Hoh. "Dynamic pricing incentive for participatory sensing." Pervasive and Mobile Computing 6, no. 6 (2010): 693-708.}

\ctra{The following paper is similar: 
[R1.8] 
Lee, Juong-Sik, and Baik Hoh. "Sell your experiences: a market mechanism based incentive for participatory sensing." In Pervasive Computing and Communications (PerCom), 2010 IEEE International Conference on, pp. 60-68. IEEE, 2010.
}

\ab

User participation is one of the most important elements in participatory sensing
application for providing adequate level of service quality. However, incentive mechanism
and its economic model for user participation have been less addressed so far in this
research domain. This paper studies the economic model of user participation incentive in
participatory sensing applications. To stimulate user participation, we design and evaluate
a novel reverse auction based dynamic pricing incentive mechanism where users can
sell their sensing data to a service provider with usersÕ claimed bid prices. The proposed
incentive mechanism focuses on minimizing and stabilizing the incentive cost while
maintaining adequate level of participants by preventing users from dropping out of
participatory sensing applications. Compared with random selection based fixed pricing
incentive mechanism, the proposed mechanism not only reduces the incentive cost for
retaining the same number of participants but also improves the fairness of incentive
distribution and social welfare.

\bg

There has been a growing body of studies on sensor networks; however commercialization of sensor network
technologies has never been successfully deployed (or introduced) in the real world due to the expensive installation cost
for sufficient number of sensors. Considering the issue, several groups [1,2] have recently proposed to incorporate human
carrying smart phones in a sensing data collecting loop. Such a novel approach is shortly called ÔParticipatory SensingÕ. In
participatory sensing, a large number of users carrying smart phones contribute to monitoring the environments with their
sensing measurements (e.g., Mobile Millennium [3], Nokia Simple Context [4], Urban Atmosphere [5]). Smart phones carried
by users transmit the sensing data to service providers, thereby replacing dedicated infrastructure and sensors. 2 

However,
currently existing deployments have suffered from insufficient participants because participants who voluntarily submit
their sensing data found no interest to remain actively in the system without being rewarded. From the viewpoints of service
providers that collect and utilize user sensing data, a well designed incentive mechanism increases user participation for
the service and helps address privacy concerns that arise in the data collection step. A participant may drop out of the
collecting loop unless his Return on Investment (ROI) in participatory sensing application is greater than their expectations.
The expected ROI is dependent on true valuation of userÕs investment that includes all efforts for collecting data such as
battery power consumption, device resources, and privacy. However, such a true valuation dynamically changes among
individuals, different types of sensing data, and userÕs contexts (e.g., spatial-temporal situations). In such environments,
we observed that fixed price incentive mechanisms cannot adapt to dynamic distributions of userÕs true valuations and
lead users to dropping out of participatory sensing applications. Additionally, it is hard to infer optimal incentive price for
user sensing data in the fixed price incentive mechanism. 

In this study, we address the problem of designing an incentive
mechanism that removes the burden of accurate pricing for user sensing data, adapts itself to dynamic change of userÕs
true valuation, and minimizes the user drop out with minimal cost spent. Motivated by several inherent advantages of the
dynamic pricing scheme such as its dynamic adaptation to market environments [6], we introduce a Reverse Auction based
Dynamic Price (RADP) incentive mechanism in which users sell their sensing data to the service provider with their claimed
bids, and a service provider selects multiple users and purchases their sensing data. The selected users receive their bid prices
as a reward for their sensing data. A reverse auction for participatory sensing application is a recurring one since a service
provider recurrently and continuously requires usersÕ sensing data. In such a recurring reverse auction, we observe that
the users with higher true valuations become starved frequently for being winners who sell their sensing data. Therefore
the users with higher true valuations lose their interest in continuous participation and drop out of the reverse auction.
The dropped out participants weaken price competitions, thereby they cause incentive cost explosion because remaining
participants constantly win and, as a result, increase their bid prices for selling their sensing data for the future auction
rounds to maximize their expected profits. To overcome the challenge, we let the service provider give a virtual credit to
the participants who lost in the previous reverse auction as a reward for their participation only. The virtual participant
credit (VPC) can only be used for lowering bid price and the bid price after the deduction increases the wining probability
of the user in future auction rounds. With this mechanism, the bidders who have higher true valuations can be winners
by continuous participation and they can still remain active in the reverse auction. Such participation incentives maintain
enough active bidders (i.e., desired level of participatory sensing service quality) and stabilizes the incentive cost by keeping
the price competitions. We envision that the presented incentive mechanism effectively fits to commercial participatory
sensing applications that will be popular soon upon many requests of environmental sensing. For its successful deployment
in the real world, we have many issues to be resolved, but the incentive mechanism explored in this study plays an essential
role as a cornerstone in achieving high level service quality in participatory sensing applications.
\textbf{This paper is extended from our previous work [R2.10].}

\bg

\textbf{Applications:}
Traditional sensor networks require application-specific sensors deployed over a large area to monitor the environment
such as air quality or automotive traffic jam. However, its performance is heavily dependent on the number of sensors. If
sensor networks fail to lower the sensor cost, they cannot provide enough sensors to cover a wide area. As smart phones
are getting prevalent in mobile industry, they are expected to replace application-specific sensors. Wireless connectivity,
GPS-based localization capability, and OS can provide a platform for general-purpose sensors. Furthermore, smart phones
carried by users add mobility to static sensors, covering a dynamic range. Each user transmits what he or she senses through
the phone to nearby wireless access points (e.g., cellular base stations or WLAN access points). The infrastructure service
provider aggregates sensing measurements from a large number of users through access networks, and then delivers raw
data or statistics to application service providers. Examples of participatory sensing applications can be categorized into two
groups, environment monitoring (e.g., traffic [8-12], air pollution [5], and noise [13]) and personal monitoring (e.g., phone
data [4], user activity [14], and context [15]). In environment monitoring, the predefined number of user sensing data is
required for a given geographic region at a given time in order to guarantee desired level of service quality. This paper
focuses on environment monitoring participatory sensing applications in which a service provider collects the predefined
number of user sensing data that includes geographical and temporal features.

\textbf{Motivations:}
User participation is the most important element in participatory sensing application since application services (e.g.,
environmental sensing services) are truly dependent on usersÕ sensing data. Additionally, user participation includes sensing
and transmitting the measurements to a service provider. During the participation, a user consumes his own private resource
such as battery and computation power of his device. Also, he may expose himself to potential location privacy threats
by sharing his sensing data tagged with location. Hence, without loss of generality, each user has Ôtrue valuationÕ of the
sensing data that denotes minimum price that the user wants to receive for their consumed resource and privacy. By
monetizing and quantifying the true value, an incentive mechanism helps us to increase participation in the service and
address privacy concerns that arise in the data collection step. Designing incentive mechanisms requires knowing what
value the user place on their sensing data and what factors this value depends on. Prior work [16] is limited to addressing
the valuation of user data simply with a fixed price, and it does not differentiate different times of day, locations or various
situations of a user. Moreover, userÕs true valuation differs among individuals and over different types of data, changes
dynamically based on contexts (e.g., spatial-temporal situations), and depends on the perceived usefulness of the returned
service/application (e.g., many users ignore privacy while using Web based email system, which is notorious for collecting
user data). In such environments, without proper incentive or reward for user sensing data, we easily expect that users (with
high true valuation) drop out of participatory sensing application, and it becomes very difficult to maintain an adequate level
of participants that are required for guaranteeing desired service quality. To the best of our knowledge, it is a challenging
question to design a user participation incentive mechanism that removes the burden of accurate pricing for user sensing
data and adapts the price to dynamic change of userÕs true valuation. It has never been addressed in the research domain of
sensor networks. At the same time, minimizing the total cost of incentives while maintaining the required service quality
gives us another challenge. Responding to these challenges, we propose a reverse auction based dynamic pricing incentive
mechanism in which users can sell their sensing data to a service provider with their claimed bids and the price for user
sensing data is determined not by a service provider but by users.


\textbf{Challenges in Reserve Auction:}
Two types of market mechanisms can be applied to the participatory sensing applications from the pricing perspective
for rewarding user sensing data: Random Selection based Fixed Pricing (RSFP) incentive mechanism and Reverse Auction
based Dynamic Pricing (RADP) incentive mechanism. In RSFP incentive mechanism, a service provider selects predefined
number of users randomly and purchases their sensing data with a fixed price. Hence the selected users receive the fixed
price equally. On the other hand, in RADP incentive mechanism, users bid for selling their sensing data, a service provider
selects predefined number of lower bid price users, and the selected users receive their bid prices for their sensing data as
a reward. Hence, the selling price in this mechanism dynamically changes based on bid prices of users. Compared to RSFP
incentive mechanism, RADP incentive mechanism provides several inherent benefits from auction mechanism. Since users
decide their own prices for selling their sensing data, RADP incentive mechanism simplifies pricing decision of incentive
cost from the service providerÕs point of view and users play more active roles in incentive negotiation from the user point
of view. The user may enjoy and entertain the competition between other users in RADP incentive mechanism as if they are
playing a game. Additionally RADP incentive mechanism can adapt to dynamically changed data collection environments
(e.g., geographic imbalance of collecting user sensing data) because when the number of participants decreases, the price
increases to recruit more participants.



\ct{
[1] Nokia Sensor Planet Project. http://www.sensorplanet.org.

[2] F. Zhao, Sensornet 2.0: the new frontier, in: RTSSÕ06: Proceedings of the 27th IEEE International Real-Time Systems Symposium, IEEE, Washington,
DC, USA, 2006.

[3] Mobile Millennium. http://traffic.berkeley.edu.

[4] Nokia Simple Context. https://alpha.nokoscope.com/eb2.

[5] Intel Urban Atmosphere. http://www.urban-atmospheres.net/.

[6] M. Bichler, The Future of e-Markets: Multidimensional Market Mechanism, Cambridge University Press, 2001.

[7] J. Lee, B. Hoh, Sell your experiences: market mechanism based incentive for participatory sensing, in: IEEE International Conference on Pervasive
Computing and Communications, PERCOM 2010, Mannheim, Germany, 2010.

[8] B. Hoh, M. Gruteser, Computer ecology: responding to mobile worms with location-based quarantine boundaries, in: International Workshop on
Research Challenges in Security and Privacy for Mobile and Wireless Networks, 2006.

[9] B. Hull, V. Bychkovsky, Y. Zhang, K. Chen, M. Goraczko, A.K. Miu, E. Shih, H. Balakrishnan, S. Madden, CarTel: a distributed mobile sensor computing
system, in: 4th ACM SenSys, Boulder, CO, November 2006.

[10] A. Krause, E. Horvitz, A. Kansal, F. Zhao, Toward community sensing, in: ACM/IEEE International Conference on Information Processing in Sensor
Networks, IPSN, April 2008.

[11] T. Abdelzaher, Y. Anokwa, P. Boda, J. Burke, D. Estrin, L. Guibas, A. Kansal, S. Madden, J. Reich, Mobiscopes for human spaces, IEEE Pervasive ComputingÑ
Mobile and Ubiquitous Systems 6 (2) (2007).

[12] B. Hoh, M. Gruteser, R. Herring, J. Ban, D. Work, J.C. Herrera, A.M. Bayen, M. An-navaram, Q. Jacobson, Virtual trip lines for distributed privacy-preserving
traffic monitoring, in: MobiSys 2008, Breckenridge, CO.

[13] M. Allen, L. Girod, R. Newton, S. Madden, D.T. Blumstein, D. Estrin, Voxnet: an interactive, rapidly deployable acoustic monitoring platform, in: IPSNÕ08:
Proceedings of the 2008 International Conference on Information Processing in Sensor Networks, IPSN 2008, IEEE Computer Society, Washington, DC,
USA, 2008, pp. 371-382.

[14] MIT Media Lab: The Owl Project. http://owlproject.media.mit.edu.

[15] UCLA Center for Embedded Networked Sensing. http://research.cens.ucla.edu.

[16] G. Danezis, S. Lewis, R. Anderson,Howmuch is location privacy worth? WEISÕ05: Proceedings of the Fourth Workshop on the Economics of Information
Security, Harvard University 2005.}



\newpage

\subsection{Oscar Wang (INFOCOM 2013) -- \comm{Reputation and Trust}}

\ctra{
[x]
Oscar Wang, Xinlei, Wei Cheng, Prasant Mohapatra, and Tarek Abdelzaher. "ARTSense: anonymous reputation and trust in participatory sensing." In INFOCOM, 2013 Proceedings IEEE, pp. 2517-2525. IEEE, 2013.}

\ab

With the proliferation of sensor-embedded mobile
computing devices, participatory sensing is becoming popular
to collect information from and outsource tasks to participating
users. These applications deal with a lot of personal information,
e.g., usersÕ identities and locations at a specific time. Therefore,
we need to pay a deeper attention to privacy and anonymity.
However, from a data consumerÕs point of view, we want
to know the source of the sensing data, i.e., the identity of
the sender, in order to evaluate how much the data can be
trusted. ÒAnonymityÓ and ÒtrustÓ are two conflicting objectives in
participatory sensing networks, and there are no existing research
efforts which investigated the possibility of achieving both of
them at the same time. In this paper, we propose ARTSense,
a framework to solve the problem of Òtrust without identityÓ
in participatory sensing networks. Our solution consists of a
privacy-preserving provenance model, a data trust assessment
scheme and an anonymous reputation management protocol. We
have shown that ARTSense achieves the anonymity and security
requirements. Validations are done to show that we can capture
the trust of information and reputation of participants accurately.


\bg

In recent years, we have seen the massive prevalence of
mobile computing devices such as smartphones and tablet
computers. These devices usually come with multiple embedded
sensors, such as camera, microphone, GPS, accelerometer,
digital compass and gyroscope. Because of these advancements,
the participatory sensing model is becoming popular.
Participants use their personal mobile devices to gather data
about nearby environment and make them available for largescale
applications. Two examples of participatory sensing
applications are Gigwalk [1] developed by a startup company
and mCrowd [2] developed by University of Massachusetts
Amherst. They provide a marketplace for sensing tasks that
can be performed from smartphones. A requester of data can
create tasks that uses the general public to capture geo-tagged
images, videos, audio snippets, or fill out surveys. Participants
who have installed the client apps on their smartphones can
submit their data and get rewarded. For example, Microsoft
Bing has been collecting photos using Gigwalk for panoramic
3-D photosynthesis of businesses and restaurants in Bing Map.

\textbf{Privacy:}
Sharing sensed data tagged with spatio-temporal information
could reveal a lot of personal information, such as a userÕs
identity, personal activities, political views, health status, etc.
[3], which poses threats to the participating users. Therefore,
participatory sensing requires a deeper attention to privacy
and anonymity, and a mechanism to preserve usersÕ location 
privacy and anonymity is mandatory. Another dimension of
data security in participatory sensing is the reliability of
the sensed data. In participatory sensing applications, data
originates from sensors controlled by other people, and any
participant with an appropriately configured device can easily
submit falsified data, hence data trustworthiness becomes more
crucial than the traditional wireless sensor networks. There is
an inherent conflict between trust and privacy. If a participatory
sensing system provides full anonymity to the participants, it
is difficult to guarantee the trustworthiness of submitted data.
Finding a solution that achieves both trust and anonymity is a
major challenge in such systems [4].

There have been plenty of research efforts that have investigated
privacy techniques for anonymous data collection in
location based services (LBS) and particularly in participatory
sensing systems. However, how to assess the trustworthiness of
the anonymously collected data has not been considered. Other
pieces of work which studied trust models did not consider the
privacy requirements. In this paper, we are trying to solve the
problem of Òtrust without identityÓ in participatory sensing
networks. To the best of our knowledge, our work is the first
attempt for a trust and reputation framework while maintaining
the desired anonymity in the context of participatory sensing.

\ct{[1] ÒGigwalk.Ó http://www.gigwalk.com.

[2] ÒmCrowd.Ó http://crowd.cs.umass.edu/.

[3] I. Krontiris, F. Freiling, and T. Dimitriou, ÒLocation privacy in urban
sensing networks: research challenges and directions,Ó IEEE Wireless
Communications, vol. 17, no. 5, pp. 30-35, 2010.

[4] A. Kapadia, D. Kotz, and N. Triandopoulos, ÒOpportunistic sensing:
Security challenges for the new paradigm,Ó in IEEE International
Communication Systems and Networks and Workshops., 2009.
}




\newpage

\subsection{K. Iordanis (INFOCOM 2013) -- \comm{Optimal Reserve Auction}}


\ctra{
[R1.10]
Koutsopoulos, Iordanis. "Optimal incentive-driven design of participatory sensing systems." In INFOCOM, 2013 Proceedings IEEE, pp. 1402-1410. IEEE, 2013.
}

\ab

Participatory sensing has emerged as a novel
paradigm for data collection and collective knowledge formation
about a state or condition of interest, sometimes linked to a
geographic area. In this paper, we address the problem of incentive
mechanism design for data contributors for participatory sensing
applications. The service provider receives service queries in an
area from service requesters and initiates an auction for user
participation. Upon request, each user reports its perceived cost
per unit of amount of participation, which essentially maps
to a requested amount of compensation for participation. The
participation cost quantifies the dissatisfaction caused to user due
to participation. This cost is considered to be private information
for each device, as it strongly depends on various factors inherent
to it, such as the energy cost for sensing, data processing and transmission
to the closest point of wireless access, the residual battery
level, the number of concurrent jobs at the device processor, the
required bandwidth to transmit data and the related charges of
the mobile network operator, or even the user discomfort due
to manual effort to submit data. Hence, participants have strong
motive to misreport their cost, i.e. declare a higher cost that the
actual one, so as to obtain higher payment.

We seek a mechanism for user participation level determination
and payment allocation which is most viable for the provider, that
is, it minimizes the total cost of compensating participants, while
delivering a certain quality of experience to service requesters. We
cast the problem in the context of optimal reverse auction design,
and we show how the different quality of submitted information
by participants can be tracked by the service provider and used
in the participation level and payment selection procedures. We
derive a mechanism that optimally solves the problem above, and
at the same time it is individually rational (i.e., it motivates users to
participate) and incentive-compatible (i.e. it motivates truthful cost
reporting by participants). Finally, a representative participatory
sensing case study involving parameter estimation is presented,
which exemplifies the incentive mechanism above.

\bg

In recent years, participatory (or community) sensing has
rapidly proliferated as a paradigm for multi-modal data collection
and dissemination [1], [2]. The large penetration of
smartphones with various embedded sensors (e.g. camera, microphone,
accelerometer, light, GPS) have greatly automatized
the information generation process, which now mostly occurs
without human intervention. On the other hand, in cases where
human intervention is needed, the ease with which information
like text, image or video can be created and uploaded, has
made the human factor almost transparent in the whole chain
of information generation, transport and consumption. Participatory
sensing has also revolutionized the field of wireless
sensor networks, since it eliminates the need for deploying a
specific purpose sensor network. It has also created a novel
viewpoint in information gathering and exploitation, which is
known as collective awareness, or collective intelligence. That
is, information can be easily collected through user contribution,
and after appropriate processing and aggregation, it can
aid in forming collective knowledge about a specific state or
condition of interest, sometimes linked to a geographic area.
Collective knowledge is of value to the community at large, and,
depending on the application, it can be directly or indirectly
influential to data contributors as well.

In participatory sensing, a specific-purpose application is
launched by an application service provider. Applications that
rely on participatory sensing are abundant and diverse, and
they range from air pollution or electromagnetic field (EMF)
radiation monitoring, up to road traffic condition reporting,
prediction and tracking of disease outbreaks, or urban parking
space management. The common objective in all applications
is to represent an underlying phenomenon, process or state as
accurately as possible and deliver it to interested users. Thus,
in air pollution and EMF radiation monitoring, the target is a
dynamic city map of air pollution or EMF radiation levels; in
parking space management, the goal is to construct a map with
free parking spot locations, and so on.


There exist participants to the service, who act as information
providers. These entities submit measurement data, usually
through mobile devices, or they simply provide input, whatever
that might be, based on their own experience at their location.
Data are submitted through the wireless operator infrastructure
or WiFi access points and are forwarded to the application
service provider. There also exist subscribers to the service,
namely information consumers. These place queries related to
the service (e.g. about the air pollution level or free parking
spots) in their vicinity and require to be served. The service
provider aggregates data samples of providers and forwards
the result to querying entities for some price, thereby generating
revenue. However, service availability and provisioning
at certain quality depends crucially on participation levels of
providers and on the quality of provided information. Information
providers voluntarily contribute data subject to various
costs, such as mobile device battery energy cost for sensing,
data processing and transmission, charges by the mobile operator
for the bandwidth needed for transmitting data, processing
power cost, or discomfort due to manual effort to submit data.
It is therefore very important for the survivability of the service
to have appropriate incentive mechanisms to motivate users to
participate in data collection.


Incentive mechanisms can be actual payments or credits.
Payments need to be large enough to cover participation costs
and create motives for participation but also low enough, so that
the application service is maintained without much expenditure
by the service provider. The participation cost is private information
for users, and users are strongly motivated to misreport
the actual cost so as to receive higher compensation. The design
of incentive mechanisms for participatory sensing applications
that are economically viable for the application provider, yet
they encourage truthful cost reporting for users and guarantee
a given quality of service, is the problem we address in this
paper, by using the optimal auction design framework [18].

\re

Participatory sensing applications can be classified into three
categories: environment-centered, infrastructure and facility related,
and socially or community centered. In the first class,
the OpenSense [3] participatory sensing infrastructure performs
real-time air quality monitoring and comprises heterogeneous
sensors and a management middleware. In the second category,
an example is GreenGPS [4], which uses a vehicle interface
to measure and transmit fuel consumption and location data. It
then constructs fuel-efficient routes to destinations for querying
users. CrowdPark [5] facilitates parking reservation through
user submitted information about when parking resources will
be available, and uses this information to help other users locate
parking spots. In the same spirit but using a different approach,
ParkNet [6] application detects available parking spots using
ultrasonic sensing devices installed on cars, combined with
smart phones. Finally, in a representative system of the third
category, LiveCompare participants use their phone cameras to
take a picture of the price tag of a product of interest [7]. In
exchange for submitting a price data point, the user receives
pricing information for the product at nearby grocery stores.
Finally, in DietSense [8], individuals take pictures of what they
eat and share it within a community to compare eating habits,
e.g. in a community of diabetics.


In [9], the authors address the problem of sensor selection
out of a set of available ones, such that value of derived
measurement data is maximized, subject to sensor resource
usage constraints. The value of information is defined as the
expected weighted reduction in prediction uncertainty of the
underlying process at unobserved locations, where the weight is
the query demand load at various locations, and the expectation
is taken over the probability distribution induced on possible
available sensor locations by the selected ones.

The problem of incentive provisioning to users for contributing
data is a central one in participatory sensing [10].
In some cases, participation incentives are intrinsic to the
application: for example in LiveCompare, users obtain the
service, namely product prices in nearby stores, only if they
participate by submitting prices themselves. If participants
do not obtain a direct benefit from participation, appropriate
incentive mechanisms need to be designed. In the CrowdPark
system, compensation comes through subsequent gains from
re-selling the parking spot, which exceed the refund received
if they deny the spot on purpose. The work in [11] guides
credit allocation to participants by using the feedback of quality
of provisioned information (QoI) and credit satisfaction from
information requesters and participants respectively. In [12],
the authors consider users as data contributors and requesters
at the same time, and they formulate convex optimization
problems that allocate credit quota to users to maximize utility
functions that denote social welfare or fairness. User utility is
a concave function of normalized allocated credit, normalized
over user demand and contribution cost. In [13], the authors
consider a reputation-based scheme in the context of a crowdsourcing
website. The scheme builds upon a reputation metric
that rewards or penalizes users, depending on whether their
strategy is aligned to or deviates from a social norm. The
scheme is then incorporated into a repeated game model that
captures interactions of users who contribute to and request
information from the website.

In Bayesian games [14], information about player characteristics
(e.g. payoffs) is incomplete or uncertain. Uncertainty is
captured by a random variable, the user type, whose realization
is known only to that user. Mechanism design is the branch of
game theory that seeks to influence the outcome of a Bayesian
game towards a certain objective. Auctions are an important
class of mechanism design and study rules for allocation
of a divisible or indivisible good to interested buyers and
subsequent pricing [15], under the regime of unknown private
buyer valuations. The Vickrey Clark Groves (VCG) auction
[16], [17] for divisible goods is efficient, in the sense that
it maximizes social welfare of the allocation while ensuring
truthful declaration of the private utility function. On the other
hand, an optimal auction maximizes the expected revenue of
the seller while ensuring that truth-telling is an equilibrium of
the Bayesian game among users. The seminal work in optimal
auctions for an indivisible good is [18].

Along that spirit, the recent work in [19] considers the
selection of the subset of users to collect measurements from
for maximizing system utility minus sum of payments. The
authors exploit sub-modularity of the objective above to show
that a greedy algorithm in user selection and payment solves
the problem, while the mechanism is truthful and has positive
objective function value. In [20], a reverse auction is proposed,
in which users submit their offers, and the provider selects some
of them and compensates them based on their offers. A virtual
credit is also included just for participating in the auction,
provided that the participant reduces its offer in subsequent
rounds, so that the set of winning users changes at different
times. This discourages increasing offers by winning users and
is shown to reduce compensation cost. Reverse auctions have
also been considered for designing incentive mechanisms for
3G traffic offloading [21], where users are compensated based
on the bids they submit about the delay they wish to experience
while offloading, versus price reduction.

Our work is different from the mechanism in [18] in that
we consider an optimal reverse auction with multiple winners.
The provider needs to fulfil a given quality of service constraint
by ?buying? different participation levels from different users.
Differently from [20] and [11], in addition to the above, the
constraint of providing a guaranteed quality of service and
the consideration of quality of contributed data are novel and
are taken into account in the allocation process. Moreover,
we explicitly compute the payment and participation level for
each user. Compared to [19], our method explicitly minimizes
compensation cost, and it takes into account the computed
quality of submitted information. Furthermore, it adheres to
a participation level allocation approach rather than a user
selection one, and thus it allows for more flexibility.


\ct{
[1] R.K. Ganti, F. Ye, H. Lei, ?Mobile Crowdsensing: Current state and future
challenges?, IEEE Comm. Mag., vol.49, no.11, pp.32-39, Nov. 2011.

[2] J. Goldman, K. Shilton, J. Burke, D. Estrin, M. Hansen, N. Ramanathan,
S. Reddy, V. Samanta, M. Srivastava, ?Participatory Sensing: A citizenpowered
approach to illuminating the patterns that shape our world?, White
Paper, Center for Embedded Networked Sensing, UCLA, 2008.

[3] OpenSense Project: http://www.nano-tera.ch/projects/401.php, 2010.

[4] R.K. Ganti, N. Pham, H. Ahmadi, S. Nangia, and T.F. Abdelzaher,
?GreenGPS: A Participatory sensing fuel-efficient maps application?, in
Proc. ACM MobiSys, 2010.

[5] T. Yan, B. Hoh, D. Ganesan, K. Tracton, T.Iwuchukwu, J.-S. Lee,
?CrowdPark: A Crowdsourcing-based Parking Reservation System for
Mobile Phones?, University of Massachusetts at Amherst Tech. Report,
http://lass.cs.umass.edu/ yan/pubs/yan11CrowdPark.pdf

[6] S. Mathur, T. Jin, N. Kasturirangan, J. Chandrashekharan, W. Xue, M.
Gruteser, and W. Trappe, ?Parknet: Drive-by sensing of road-side parking
statistics,?, in Proc. of ACM MobiSys, 2010, pp. 123136.

[7] L. Deng and L.P.Cox, ?LiveCompare: Grocery Bargain Hunting through
Participatory Sensing?, in Proc. ACM HotMobile, 2009.

[8] S. Reddy, A. Parker, J. Hyman, J. Burke, D. Estrin and M. Hansen, ?Image
browsing, processing, and clustering for participatory sensing: Lessons
from a dietsense prototype?, in Proc. 4th Workshop on Embedded Net.
Sensors (EmNets), 2007.

[9] A. Krause, E. Horvitz, A. Kansal and F. Zhao, ?Toward community
sensing?, in Proc. ACM/IEEE Int. Conf. on Inform. Proc. in Sensor
Networks (IPSN), 2008.

[10] S. Reddy, D. Estrin, M. Hansen, and M. Srivastava, ?Examining micropayments
for participatory sensing data collections?, in Proc. ACM Int.
Conf. on Ubiquitous computing (Ubicomp), 2010.

[11] C. H. Liu, P. Hui, C. Bisdikian, J. W. W. Branch, and B. Yang, ?Efficient
network management for context-Aware participatory sensing?, in Proc.
IEEE SECON, 2011.

[12] T. Luo and C.-K. Tham, ?Fairness and social welfare in incentivizing
participatory sensing?, in Proc. IEEE SECON, 2012.

[13] Y. Zhang and M. van der Schaar, ?Reputation-based incentive protocols
in crowdsourcing applications?, in Proc. IEEE INFOCOM, 2012.

[14] R. Gibbons, Game Theory for Applied Economists, Princeton University
Press, 1992.

[15] V. Krishna, Auction Theory, Academic Press, 2002.

[16] W. Vickrey, ?Counterspeculation, Auctions and Competitive Sealed Tenders?,
Journal of Finance, vol. 16, pp. 8-37, 1961.

[17] T. Groves, ?Incentives in Teams?, Econometrica, vol. 41, pp. 617-631,
1973.

[18] R, Myerson, ?Optimal auction design?, Math. of Oper. Research, vol.6,
pp.58-73, 1981.

[19] D. Yang, G. Xue, X. Fang and J. Tang, ?Crowdsourcing to Smartphones:
Incentive mechanism design for mobile phone sensing?, in Proc. ACM
MobiCom, 2012.

[20] J.-S. Lee and B. Hoh, ?Dynamic pricing incentive for participatory
sensing?, Elsevier Pervasive and Mobile Computing, vol.6, no.6, pp. 693-
708, Dec. 2010.

[21] X. Zhuo, W. Gao, G. Cao and Y. Dai, ?Win-Coupon: An incentive
framework for 3G traffic offloading?, in Proc. IEEE Int. Conf. on Net.
Protocols (ICNP), 2011.

[22] I. Koutsopoulos and M. Halkidi, ?Lifetime maximization in wireless
sensor networks with an estimation mission?, in Proc. IEEE GLOBECOM,
2009.

[23] S. Shakkottai and R. Srikant, Network Optimization and Control, Foundations
and Trends in Networking, NoW Publishers, 2007.

[24] S. Yang and B. Hajek,?VCG-Kelly mechanisms for allocation of divisible
goods: Adapting VCG mechanisms to one-dimensional signals?, IEEE J.
Selected Areas of Communications, vol. 25, no.6, pp. 1237-1243, 2007.

}









\newpage



\subsection{Tie Luo (INFOCOM 2014) -- \comm{All-pay Auciton}}

\ctra{
[R1]
Luo, Tie, Hwee-Pink Tan, and Lirong Xia. "Profit-maximizing incentive for participatory sensing." In IEEE INFOCOM. 2014.
}

\ab

We design an incentive mechanism based on all-pay
auctions for participatory sensing. The organizer (principal) aims
to attract a high amount of contribution from participating users
(agents) while at the same time lowering his payout, which we formulate
as a profit-maximization problem. We use a contributiondependent
prize function in an environment that is specifically
tailored to participatory sensing, namely incomplete information
(with information asymmetry), risk-averse agents, and stochastic
population. We derive the optimal prize function that induces
the maximum profit for the principal, while satisfying strict
individual rationality (i.e., strictly have incentive to participate at
equilibrium) for both risk-neutral and weakly risk-averse agents.
The thus induced profit is demonstrated to be higher than the
maximum profit induced by constant (yet optimized) prize. We
also show that our results are readily extensible to cases of riskneutral
agents and deterministic populations.

\bg

The global proliferation of smartphones has spurred the
recent emergence of participatory sensing paradigm, in which
the public crowd rather than professionals undertake various
sensing activities with inbuilt sensors on their smartphones.
This paradigm relieves the need for deploying and maintaining
costly wireless sensor networks, yet can achieve pervasive
spatiotemporal coverage, making it appealing enough to have
spawned a large number of projects such as PEIR [1], ParkNet
[2] and Ear-phone [3], to name a few.

The crowdsourcing nature and lacking of intrinsic motivation
in many participatory sensing applications, however, render
incentive the foremost challenge to the viability of participatory
sensing. Although a variety of incentives in similar contexts
have been discussed, including micro-payment [4], reputation
[5], and fun [6], we deem auction [7] to be an excellent
candidate for designing incentive mechanisms, as it solves the
challenging issue of pricing participantsÕ effort, endogenously
(rather than by an external authority) by leveraging the market
power under a game setting. Indeed, we are not alone in holding
this opinion; some prior studies [8]-[10] were carried out in
this regard. The common central theme of these studies is to
determine a sound wage for participants using reverse auctions,
with certain objectives such as retaining auction losers [8],
minimizing cost and ensuring truthful bidding [9], [10].

Along a different spirit, [20] proposes a market-based incentive
scheme using a demand-and-supply model: participants
are not only data suppliers but also service consumers who
demand information service provisioned from processing the
contributed data. Therefore, instead of offering monetary incentive,
the service provider allocates consumable service to
participants in accordance with their data contribution levels, in
such a way that ensures fairness and maximizes social welfare.

\ct{
[1] M. Mun, S. Reddy, K. Shilton, N. Yau, J. Burke, D. Estrin, M. Hansen,
E. Howard, R. West, and P. Boda, ``PEIR, the personal environmental
impact report, as a platform for participatory sensing systems research,''
in ACM MobiSys, 2009, pp. 55-68.

[2] S. Mathur, T. Jin, N. Kasturirangan, J. Chandrasekaran, W. Xue,
M. Gruteser, and W. Trappe, ``ParkNet: drive-by sensing of road-side
parking statistics,'' in ACM MobiSys, 2010, pp. 123-136.

[3] R. Rana, C. T. Chou, S. Kanhere, N. Bulusu, and W. Hu, ``Ear-phone:
An end-to-end participatory urban noise mapping system,'' in ACM/IEEE
IPSN, 2010.


[4] S. Reddy, D. Estrin, M. Hansen, and M. Srivastava, ``Examining micropayments
for participatory sensing data collections,'' in UbiComp, 2010.

[5] Y. Zhang and M. van der Schaar, ``Reputation-based incentive protocols
in crowdsourcing applications,'' in IEEE INFOCOM, 2012.

[6] K. Han, E. A. Graham, D. Vassallo, and D. Estrin, ``Enhancing motivation
in a mobile participatory sensing project through gaming,'' in IEEE
SocialCom, 2011.


[7] V. Krishna, Auction theory, 2nd ed. Academic Press, 2009.

[8] J.-S. Lee and B. Hoh, ``Sell your experiences: A market mechanism based
incentive for participatory sensing,'' in IEEE PerCom, 2010.

[9] D. Yang, G. Xue, X. Fang, and J. Tang, ``Crowdsourcing to smartphones:
Incentive mechanism design for mobile phone sensing,'' in ACM Mobi-
Com, 2012.

[10] I. Koutsopoulos, ``Optimal incentive-driven design of participatory sensing
systems,'' in IEEE INFOCOM, 2013.

[20] T. Luo and C.-K. Tham, ``Fairness and social welfare in incentivizing
participatory sensing,'' in IEEE SECON, June 2012, pp. 425-433.
}


\ctra{
[R1.x]
Wu, Fang-Jing, and Tie Luo. "A Generic Participatory Sensing Framework for Multi-modal Datasets." In Symposium on Participatory Sensing and Crowdsourcing of ISSNIP, vol. 21, p. 24. 2014.
}

\ab

Participatory sensing has become a promising data
collection approach to crowdsourcing data from multi-modal data
sources. This paper proposes a generic participatory sensing
framework that consists of a set of well-defined modules in
support of diverse use cases. This framework incorporates a
concept of Òhuman-as-a-sensorÓ into participatory sensing and
allows the public crowd to contribute human observations as well
as sensor measurements from their mobile devices.We specifically
address two issues: incentive and extensibility, where the former
refers to motivating participants to contribute high-quality data
while the latter refers to accommodating heterogeneous and
uncertain data sources. To address the incentive issue, we design
an incentive engine to attract high-quality contributed data
independent of data modalities. This engine works together with a
novel social network that we introduce into participatory sensing,
where participants are linked together and interact with each
other based on data quality and quantity they have contributed.
To address the extensibility issue, the proposed framework
embodies application-agnostic design and provides an interface to
external datasets. To demonstrate and verify this framework, we
have developed a prototype mobile application called imReporter,
which crowdsources hybrid (image-text) reports from participants
in an urban city, and incorporates an external dataset from a
public data mall. A pilot study was also carried out with 15
participants for 3 consecutive weeks, and the result confirms that
our proposed framework fulfills its design goals. 

\bg


Modern mobile devices with a variety of built-in sensors
have enabled the confluence of ubiquitous computing,
networking technologies, distributed decision making, and
wireless sensor networks. Emerging on this trend is participatory
sensing, which crowdsources sensory measurements
from mobile devices owned by public crowd, and has become
a promising approach to large-scale and multi-modal data
collection [1][2][3][4][5][6].

In this paper, we propose a generic participatory sensing
(gPS) framework which consists of multiple functional
modules that are independent of specific applications and
can accommodate multi-modal data sources. This framework
incorporates a concept of Òhuman-as-a-sensorÓ into the participatory
sensing paradigm to collect human observations, in
addition to sensor measurements, from mobile devices owned
by the public crowd. Fig. 1 gives the overview of such a
gPS system, which we describe below using an example
use case in transportation. The organizers launch a city-wide
data collection campaign of transportation activities for urban
planing. Each participant carries a mobile device to report
measurements from the built-in accelerometer, gyroscope, and
GPS sensor, which can be used to deduce his travel mode
(e.g., by car or foot) and travel speed, as well as to report
images using the built-in camera, which may serve as witness
of traffic accidents. A participant can also annotate the images
and write text-based feedback on city transportation systems.
These reports are then sent to a back-end application server or a cloud via WiFi/3G/4G connections. In addition to these
crowdsourced dynamic traffic information, some relatively
static video streams which are captured at road junctions and
stored in a public data mall, can also be fed into the back-end
cloud. The campaign organizers, who may also be end-users,
can then extract useful information from the combination of
dynamic crowdsourced content and static database to figure out
the actual traffic situations and make more informed decisions.

In participatory sensing, two critical challenges arise: incentive
[8][9] and extensibility. The former refers to motivating
the public crowd to contribute data from their mobile devices,
while the latter refers to providing an elastic framework for
diverse and uncertain data sources. To address the incentive issue,
our proposed gPS framework embeds an incentive engine
working together with an endorsement social network, which
exploits mutual influence among participants by allowing them
to interact with each other based on the quality and quantity
of their contributed data. To address the extensibility issue, the
gPS framework features application-agnostic design in support
of diverse use cases and multi-modal datasets, and allows for
interfacing with external datasets as well.

\re

Smartphone-based sensing technologies combined with
data analytics has steered data collection towards a new
sensing paradigm, participatory sensing [10].

\ct{
[1] ``Waze: Free GPS navigation with turn by turn,'' https://www.waze.com/.

[2] ``Steptacular project,'' http://scsn.stanford.edu/index.php.

[3] H. K. Le, J. Pasternack, H. Ahmadi, M. Gupta, Y. Sun, T. Abdelzaher,
and D. R. J. Han, ``Apollo: Towards factfinding in participatory sensing.''
in IEEE IntÕl Symp. Information Processing in Sensor Networks, 2011,
pp. 129-130.

[4] ``NoiseTube,'' http://www.noisetube.net/.

[5] ``CleanLah,'' http://appshopper.com/productivity/cleanlah.

[6] ``MyENV,'' https://itunes.apple.com/sg/app/myenv/id444435182.

[7] ``Data Mall - MyTransport.SG,'' http://www.mytransport.sg/content
/mytransport/home.html.

[8] T. Luo and C.-K. Tham, ``Fairness and social welfare in incentivizing
participatory sensing,'' in IEEE SECON, 2012.

[9] T. Luo, H.-P. Tan, and L. Xia, ``Profit-maximizing incentive for participatory
sensing,'' in IEEE INFOCOM, 2014, to appear.

[10] J. Burke, D. Estrin, M. Hansen, A. Parker, N. Ramanathan, S. Reddy,
and M. B. Srivastava, ``Participatory sensing,'' in In: Workshop on
World-Sensor-Web (WSW06): Mobile Device Centric Sensor Networks
and Applications, 2006, pp. 117-134.
}

\ctra{
[R1.x]
Luo, Tie, Salil S. Kanhere, and Hwee-Pink Tan. "SEW-ing a Simple Endorsement Web to Incentivize Trustworthy Participatory Sensing.", IEEE SECON 2014}


\ab

Two crucial issues to the success of participatory
sensing are (a) how to incentivize the large crowd of mobile
users to participate and (b) how to ensure the sensing data to be
trustworthy. While they are traditionally being studied separately
in the literature, this paper proposes a Simple Endorsement Web
(SEW) to address both issues in a synergistic manner. The key idea
is (a) introducing a social concept called nepotism into participatory
sensing, by linking mobile users into a social Òweb of participantsÓ
with endorsement relations, and (b) overlaying this network with
investment-like economic implications. The social and economic
layers are interleaved to provision and enhance incentives and
trustworthiness. We elaborate the social implications of SEW,
and analyze the economic implications under a Stackelberg game
framework. We derive the optimal design parameter that maximizes
the utility of the sensing campaign organizer, while ensuring
participants to strictly have incentive to participate. We also design
algorithms for participants to optimally ÒsewÓ SEW, namely to
manipulate the endorsement links of SEW such that their economic
benefits are maximized and social constrains are satisfied. Finally,
we provide two numerical examples for an intuitive understanding.


\bg

The booming smartphone industry has stimulated participatory
sensing as a new sensing paradigm which primarily
harnesses the sensors on handheld mobile devices to perform
sensing tasks that were traditionally done by wireless sensor
networks or that were not even possible. It features pervasiveness,
large scale and low cost, and has hence found a wide
range of applications in transportation [1], [2], environment [3],
lifestyle [4], healthcare [5], and so on.

However, whether participatory sensing will be viable critically
depends on two key issues: incentive and trustworthiness.
The former refers to providing motivation for the public crowd
to participate in the sensing campaigns and the latter refers
to ensuring participants to contribute good quality sensing
data; in essence, both issues arise from the fact that data is
crowdsourced from the general public. While there is a sizable
body of prior work [6]-[14] dedicated to addressing these two
issues (usually separately), a common feature of these studies
is that participants are treated individuallyÑthere is no explicit
interaction among participants.

In this paper, we take a new, social-economic approach by
(a) exploiting the incumbent social relationships among mobile
users and (b) overlaying investment-like economic relationships
over the social linkages, to provision and enhance both incentive
and trustworthiness in a synergistic manner. Precisely, we propose
a Simple Endorsement Web (SEW), a web of participants
in which participants endorse one another, out of two sources
of motivation: economically, they aim to maximize their own
economic benefit by (optimally) selecting whom to endorse and
whom to be endorsed by; socially, they are driven by nepotism
which is a notion that we first incorporate into crowdsourcing
(which subsumes participatory sensing) and is elaborated below.

\re

Incentive design has been extensively studied in economics
and recently attracted substantial attention from the participatory
sensing research community. Lee and Hoh [6] proposed a
dynamic-pricing based incentive scheme using reverse auctions,
in which participants bid their desired prices to sell their sensing
data to the campaign organizer. Yang et al. [7] studied two
incentive models: a platform-centric model where the platform
allocates a total reward to users in proportion to their planned
sensing times, and a user-centric model where each user declares
a set of tasks to complete together with his desired payment,
after which the platform will select a set of users to perform the
tasks and pay them with no lower than their declared payments.
Koutsopoulos [9] designed an auction in which users declare
their unit costs and the service provider (organizer) determines
usersÕ participation levels (e.g., data sampling rates) as well
as their payments in order to minimize total payment subject
to a given quality of service. Luo and Tham [8] proposed
a market-based incentive scheme using a demand-and-supply
model, in which participants are not only data suppliers but
also service consumers who demand information service provisioned
from processing the contributed data. Luo et al. [10]
designed an incentive mechanism based on all-pay auctions
with a contribution-dependent prize; the model is tailored to
accommodate realistic participatory sensing contexts such as
uncertain population size, unknown user types, and risk aversion
of users. All these prior studies treat participants individually,
whereas SEW links them together to take advantage of the
mutual influence among users.

To address the trustworthiness issue in participatory sensing,
Wang et al. [13] took a maximum likelihood estimation (MLE)
approach to discover truth from multiple observations. It assumes
that most users will submit multiple different reports
for the same object and some users will repeat the same
report multiple times, neither of which is assumed by SEW.
Also, it deals with binary reports only whereas SEW handles
general cases. [14] proposed a trust framework to find candidate
participants for sensing tasks, by evaluating the suitability of
candidates using information published on social media, such as
expertise and education background, which is clearly different
from this work. [11] and [12] made an attempt to tackle the
issue by using Trusted Platform Module (TPM) which involves
hardware modification; in addition, the trustworthiness thereof
refers to protecting data integrity against malicious users, which
is not the quality of data in the general sense.

\ct{
[1] A. Thiagarajan, J. Biagioni, T. Gerlich, and J. Eriksson, ``Cooperative
transit tracking using smart-phones,'' in ACM SenSys, 2010, pp. 85-98.

[2] J. K.-S. Lau, C.-K. Tham, and T. Luo, ``Participatory cyber physical system
in public transport application,'' in Proc. CCSA, IEEE/ACM UCC, 2011.

[3] R. K. Rana, C. T. Chou, S. S. Kanhere, N. Bulusu, and W. Hu, ``Ear-phone:
an end-to-end participatory urban noise mapping system,'' in ACM/IEEE
IPSN, 2010, pp. 105-116.

[4] L. Deng and L. P. Cox, ``Live compare: grocery bargain hunting through
participatory sensing,'' in ACM HotMobile, 2009, pp. 1-6.

[5] B. Longstaff, S. Reddy, and D. Estrin, ``Improving activity classification
for health applications on mobile devices using active and semi-supervised
learning,'' in PervasiveHealth, 2010.

[6] J.-S. Lee and B. Hoh, ``Sell your experiences: A market mechanism based
incentive for participatory sensing,'' in IEEE PerCom, 2010.

[7] D. Yang, G. Xue, X. Fang, and J. Tang, ``Crowdsourcing to smartphones:
Incentive mechanism design for mobile phone sensing,'' in ACM Mobi-
Com, 2012.

[8] T. Luo and C.-K. Tham, ``Fairness and social welfare in incentivizing
participatory sensing,'' in IEEE SECON, June 2012, pp. 425-433.

[9] I. Koutsopoulos, ``Optimal incentive-driven design of participatory sensing
systems,'' in IEEE INFOCOM, 2013.

[10] T. Luo, H.-P. Tan, and L. Xia, ``Profit-maximizing incentive for participatory
sensing,'' in IEEE INFOCOM, 2014.

[11] A. Dua, N. Bulusu, W.-C. Feng, and W. Hu, ``Towards trustworthy
participatory sensing,'' in 4th USENIX HotSec, 2009.

[12] P. Gilbert, L. P. Cox, J. Jung, and D. Wetherall, ``Toward trustworthy
mobile sensing,'' in ACM HotMobile, 2010.

[13] D. Wang, L. Kaplan, H. Le, and T. Abdelzaher, ``On truth discovery in social
sensing: A maximum likelihood estimation approach,'' in ACM/IEEE
IPSN, 2012.

[14] H. Amintoosi and S. S. Kanhere, ``A trust framework for social participatory
sensing systems,'' in MobiQuitous, December 2012.
}


\ctra{
[R1.x]
Tham, Chen-Khong, and Tie Luo. "Quality of contributed service and market equilibrium for participatory sensing." In Distributed Computing in Sensor Systems (DCOSS), 2013 IEEE International Conference on, pp. 133-140. IEEE, 2013.
}

\ab 

User-contributed or crowd-sourced information is
becoming increasingly common. In this paper, we consider the
specific case of participatory sensing whereby people contribute
information captured by sensors, typically those on a smartphone,
and share the information with others. We propose a new metric
called Quality of Contributed Service (QCS) which characterizes
the information quality and timeliness of a specific real-time
sensed quantity achieved in a participatory manner. Participatory
sensing has the problem that contributions are sporadic and infrequent.
To overcome this, we formulate a market-based framework
for participatory sensing with plausible models of the market
participants comprising data contributors, service consumers
and a service provider. We analyze the market equilibrium and
obtain closed form expressions for the resulting QCS at market
equilibrium. Next, we examine the effects of realistic behaviors of
the market participants and the nature of the market equilibrium
that emerges through extensive simulations. Our results show
that, starting from purely random behavior, the market and its
participants can converge to the market equilibrium with good
QCS within a short period of time.

\bg

User-contributed or crowd-sourced information is becoming
increasingly common. Together with the rise of social
media, they are increasingly being relied on as alternative
sources of information that supplement, or in some instances
even replace, traditional information channels. One specific
aspect of user-contributed or crowd-sourced information is
participatory sensing whereby people contribute information
captured by sensors, typically those on a smartphone, and
share the information with other users or a service provider.
The vast penetration of smartphones with a variety of builtin
sensors such as GPS, accelerometer and camera amongst
the population creates the potential of dense high-quality
participatory sensing and makes it an appealing alternative to
deployed sensors for large-scale data collection [1], [2].

There are several examples of smartphone applications that
harness user-contributed data. Waze [3]... WeatherLah [4]... ContriSense:Bus [2] ...


Participatory sensing has the potential to achieve a greater
sensing reach and coverage compared to the case of deployed
sensors, especially when there are many data contributors.
However, under normal circumstances, there are very few
user contributions to the WeatherLah, Mana Rapid Transit
and most other crowd-sourced or participatory applications.
Thus, one serious weakness of participatory sensing is that
user contributions are sporadic and infrequent, largely due to
usersÕ indifference and the cost to them in terms of mobile
data charges, battery life and inconvenience. Even when and
where there is data being contributed, the quality of the
contributed data in terms of accuracy, resolution, frequency
and timeliness may vary greatly as different contributors have
different sensors, smartphone models and mobile data plans.

In [6], we explored several ways to incentivize participatory
sensing and studied the fairness and social welfare characteristics
of several algorithms to apportion the service quota
of compelling services to a user based on the userÕs level of contribution and demand for services


\ct{
[2] J. K.-S. Lau, C.-K. Tham, and T. Luo, ``Participatory cyber physical system
in public transport application,'' in Proceedings of CCSA, IEEE/ACM
UCC, 2011.

[3] ``Waze - outsmarting traffic, together,'' 2012. [Online]. Available:
http://www.waze.com/

[4] Buuuk, ``WeatherLah iPhone application,'' 2012. [Online]. Available:
http://itunes.apple.com/us/app/weatherlah/id411646329?mt=8

[5] ----, ``Mana Rapid Transit iPhone application,'' 2012.
[Online]. Available: http://itunes.apple.com/sg/app/mana-rapid-transit/
id501961346?mt=8

[6] T. Luo and C.-K. Tham, ``Fairness and social welfare in incentivizing
participatory sensing,'' in IEEE Conference on Sensor, Mesh and Ad Hoc
Communications and Networks (IEEE SECON 2012), Jun 2012.
}


\ctra{
[R1.20]
Luo, Tie, and Chen-Khong Tham. "Fairness and social welfare in incentivizing participatory sensing." In Sensor, Mesh and Ad Hoc Communications and Networks (SECON), 2012 9th Annual IEEE Communications Society Conference on, pp. 425-433. IEEE, 2012.}


\ab 

Participatory sensing has emerged recently as a
promising approach to large-scale data collection. However, without
incentives for users to regularly contribute good quality data,
this method is unlikely to be viable in the long run. In this paper,
we link incentive to usersÕ demand for consuming compelling
services, as an approach complementary to conventional credit or
reputation based approaches. With this demand-based principle,
we design two incentive schemes, Incentive with Demand Fairness
(IDF) and Iterative Tank Filling (ITF), for maximizing fairness
and social welfare, respectively. Our study shows that the IDF
scheme is max-min fair and can score close to 1 on the JainÕs
fairness index, while the ITF scheme maximizes social welfare
and achieves a unique Nash equilibrium which is also Pareto and
globally optimal.We adopted a game theoretic approach to derive
the optimal service demands. Furthermore, to address practical
considerations, we use a stochastic programming technique to
handle uncertainty that is often encountered in real life situations.

\bg

With the vast penetration of smartphones with a variety of
built-in sensors such as GPS, accelerometers and cameras,
participatory sensing has emerged recently as a promising
approach to large-scale data collection. Compared to the case
of deployed sensors, participatory sensing removes the cost of
installing and maintaining sensors and their inter-connection,
while achieving much broader geographical coverage. The
challenge of prolonging network lifetime in traditional sensor
networks is no longer an issue in participatory sensing as the
node battery is now taken care of by participating users themselves.
Hence, participatory sensing is considered a promising
new sensing paradigm and has attracted extensive attention
and research efforts [1]-[3].

However, the success of participatory sensing strongly relies
on user participation to provide a sufficient and continuous
influx of user contributions. So far, most participatory sensing
studies, such as those mentioned above, focus on the sensing
tasks per se, while the participating users are recruited on a
voluntary or remunerated basis, which is not sustainable in the
long run in real-life scenarios.


This brings forth the important issue of incentive, which acts
as a driving force for participatory sensing. In this paper, we
adopt a demand-based principle to design incentive schemes,
by leveraging on the duality of a userÕs role: each user is a data
contributor as well as a service consumer. We propose a participatory
sensing framework consisting of data contributors
and service consumers with a service provider that processes
the contributed data and packages them into useful services
that are consumed by service consumers. As an example, let
us consider the case of traffic monitoring [3] (see Fig. 1). A
smartphone user, when traveling on a bus or car, can act as a
contributor of traffic data (e.g., GPS traces, bus crowd levels,
etc.) to a service provider via a network connection (e.g.,
WiFi, GPRS, 3G, etc.). The service provider then aggregates
and processes the data from all contributors and, thereby,
provides a real-time traffic information service (e.g., browsing
or querying on road jams, bus crowdedness, estimated time to
reach destination etc.) for users to consume. Other applications
include air pollution or noise level monitoring and flood or
fire alerts, in which the required data are obtained from usersÕ
handset sensor readings or are entered by the users.

In all such cases, \textbf{a user plays a dual role as a contributor
as well as a consumer}. Thus, we can exploit usersÕ demand to
consume useful and compelling services to design incentive
schemes.

\ct{
[1] M. Mun, S. Reddy, K. Shilton, N. Yau, J. Burke, D. Estrin, M. Hansen,
E. Howard, R. West, and P. Boda, ``PEIR, the personal environmental
impact report, as a platform for participatory sensing systems research,''
in ACM MobiSys, 2009, pp. 55-68.

[2] P. Dutta, P. M. Aoki, N. Kumar, A. Mainwaring, C. Myers, W. Willett,
and A. Woodruff, ``Common sense: participatory urban sensing using a
network of handheld air quality monitors,'' in ACM SenSys, 2009.

[3] J. K.-S. Lau, C.-K. Tham, and T. Luo, ``Participatory cyber physical system
in public transport application,'' in Proceedings of CCSA, IEEE/ACM
UCC, 2011.
}

\re

To the best of our knowledge, there are two studies that
specifically address incentive for participatory sensing. Lee
and Hoh [8] proposed a dynamic pricing mechanism that
allows users to sell their sensing data to a service provider. In
order to keep the service providerÕs cost low while retaining
an adequate number of participants, they proposed an auction
mechanism to keep the bid price competitive while using
``virtual participation credits'' to retain participants. Our work
does not use monetary incentive but leverages the dual role
a user plays, thereby motivating users with their intrinsic
demand for service. Furthermore, the techniques we use to
tackle this problem are all different from those used by Lee
and Hoh. The other work was a pilot study conducted in
UCLA by Reddy et al. [9] which looked into the effect of
micro-payments in participatory sensing. The study found that
monetary incentive is beneficial if combined with altruism and
competitiveness, and participants were very concerned with
fairness (which was left not addressed). In this paper, we not
only use a different incentive scheme, but we also place great
emphasis on and address the issue of fairness.

\ct{
{[8] J.-S. Lee and B. Hoh, ``Dynamic pricing incentive for participatory
sensing,'' Pervasive and Mobile Computing, vol. 6, pp. 693-708, 2010.}

{[9] S. Reddy, D. Estrin, M. Hansen, and M. Srivastava, ``Examining micropayments
for participatory sensing data collections,'' in UbiComp, 2010.}
}



\newpage







\subsection{Yanming Zhu (INFOCOM 2014) -- \comm{Social Welfare, Profit}}

\ctra{
{[R3.x]
Liu, Tong, and Yanmin Zhu. "Social welfare maximization in participatory smartphone sensing." In Wireless Algorithms, Systems, and Applications, pp. 351-365. Springer Berlin Heidelberg, 2013.}
}

\ab

Participatory smartphone sensing has lately become more
and more popular as a new paradigm for performing large-scale sensing,
in which each smartphone contributes its sensed data for a collaborative
sensing application. Most existing studies assume that smartphone
users are strictly strategic and completely rational, which can achieve
only sub-optimal system performance. Few existing studies can maximize
a system-wide objective which takes both the platform and smartphone
users into account. This paper focuses on the crucial problem
of maximizing the system-wide performance or social welfare for a participatory
smartphone sensing system. There are two great challenges.
First, the social welfaremaximization can not be realized on the platform
side because the cost of each user is private and unknown to the platform
in reality. Second, the participatory sensing system is a large-scale
real-time system due to the huge number of smartphone users who are
geo-distributed in the whole world. We propose a novel price-based decomposition
framework, in which the platform provides a unit price for
the sensing time spent by each user and the users return the sensing
time via maximizing the monetary reward. This pricing framework is
an effective incentive mechanism as users are motivated to participate
for monetary rewards from the platform. The original problem is equivalently
converted into an optimal pricing problem, and a distributed
solution via a step-size-free price-updating algorithm is proposed. More
importantly, the distributed algorithm ensures that the cost privacy of
each user is not compromised. Experimental results show that our novel
distributed algorithm can achieve the maximum social welfare of the
participatory smartphone system.

\bg

Because of the fast progress of wireless communication technology, such as the
third-generation mobile telecommunications (3G), the proliferation of smartphones
has been witnessed in the past few years. Smartphones are increasingly
equipped with a set of cheap but useful sensors such as accelerometer, camera,
and GPS, which can collect a lot of diverse useful information of our daily life.
Participatory sensing [1] has lately become more and more popular as a new
paradigm for performing large-scale sensing, in which each node contributes
its sensed data for a collaborative sensing application. Smartphones are usually
distributed over the globe and can stay connected over the Internet. This leads to
the construction of participatory smartphone sensing [2] [3]. A lot of appealing
applications can be realized, such as noise mapping and environment quality
monitoring, which are almost impossible in the past. Smartphones essentially
constitute a large-scale system of mobile sensors, instead of traditional static
sensors. A participatory smartphone sensing system consists of a sensing platform
and many smartphone users, which connect with the platform via cellular data
channels. In such a system of participatory smartphone sensing, the platform
first advertises a task of smartphone sensing, and smartphone users registered
with the system can participate in such a task by sending the sensed data to the
platform.


Because of the potential advantage of participatory smartphone sensing, a
great deal of research has devoted to developing various applications [4] [5] [6],
systems [7] [8] and technologies [9]. These existing studies simply assume that
all users are bounded to be cooperative and follow design instructions. In the
real-world, however, smartphones consume resources such as power and time.
Therefore, incentive mechanisms are needed to stimulate them to participate
distributed sensing. As a general incentive mechanism, users get monetary reward
for providing sensed data.
Many existing studies [10] [11] [12] [13] [14] employ auction algorithms to provide
incentive to users. These existing studies usually assume that smartphone
users are strictly strategic and completely rational. ...


This paper focuses on maximizing the system-wide performance or social welfare
for a participatory smartphone sensing system.
To overcome the difficulties, we propose a novel price-based decomposition
framework, where alternatively the platform provides a unit price for the sensing
time spent by each user and the users return the selection of sensing time
via maximizing the monetary reward minus the cost. This pricing framework
is a kind of an incentive mechanism as users are motivated to participate in
the participatory sensing for getting monetary rewards from the platform.

\ct{
1. Burke, J., Estrin, D., Hansen, M., et al.: Participatory sensing (2006)

2. Lane, N.D., Miluzzo, E., Lu, H., et al.: A survey of mobile phone sensing. IEEE
Communications Magazine 48(9), 140-150 (2010)

3. Chatzimilioudis, G., Konstantinidis, A., Laoudias, C., et al.: Crowdsourcing with
smartphones (2012)

4. Mun, M., Reddy, S., Shilton, K., et al.: Peir, the personal environmental impact
report, as a platform for participatory sensing systems research. In: Proc. ACM
MobiSys, pp. 55-68 (2009)

5. Stevens, M., DÕHondt, E.: Crowdsourcing of pollution data using smartphones. In:
Proc. Workshop on Ubiquitous Crowdsourcing (2010)

6. Kanhere, S.S.: Participatory sensing: Crowdsourcing data from mobile smartphones
in urban spaces. In: Hota, C., Srimani, P.K. (eds.) ICDCIT 2013. LNCS, vol. 7753,
pp. 19-26. Springer, Heidelberg (2013)

7. Yan, T., Marzilli, M., Holmes, R., et al.: mcrowd: a platform for mobile crowdsourcing.
In: Proc. ACM SenSys, pp. 347-348 (2009)

8. Sheng, X., Xiao, X., Tang, J., Xue, G.: Sensing as a service: a cloud computing
system for mobile phone sensing. In: Proc. IEEE Sensors, pp. 1-4 (2012)

9. Boulos, M.N.K., Resch, B., Crowley, D.N., et al.: Crowdsourcing, citizen sensing
and sensor web technologies for public and environmental health surveillance and
crisis management: trends, ogc standards and application examples. Health Geographics
10(1), 67 (2011)
}


\re

Participatory smartphone sensing has attracted a lot of researches. Several systems
and applications have been developed, such as mCloud [7] which is an
iPhone-based mobile crowdsourcing platform, S2aaS [8] to provide sensing services
for could users, PIER [4] for reporting personal environmental impact and
NoiseTube [5] for measuring and mapping the urban noise pollution. However,
most of these systems and applications focus on the system design by assuming
there are numerous smartphones voluntarily participating in the system. Actually,
smartphone users are motivated to participate by some money or service
reward because of resources consuming for sensed data, such as power and time.

Several recent works have focused on designing incentive mechanisms to motivate
smartphone users for participatory sensing. Most of these works apply
auction algorithms. A novel reverse auction based on dynamic price is proposed
in [10] [11], where users sell their sensed data to the platform by claiming bid
prices, and the platform selects a subset of these users and purchases at their
bid prices. Their work shows that using dynamic price can reduce the incentive
cost compared with fixed price. Luis G. Jaimes et al. [12] propose a greedy algorithm
based on the recurrent reverse auction incentive mechanism, which aims
to maximize the covered area under a budget constraint. Two system models
are considered in [13]: the platform-centric model and the user-centric model.
For the platform-centric model, an incentive mechanism based on Stackelberg
game is designed to maximize the utility of the platform. For the user-centric
model, an auction-based incentive mechanism is designed, under individuals rational
assumption. Koutsopoulos et al. [14] aim to minimize the total costs of
compensating users via proposing an optimal reverse auction mechanism. This
work illustrates the significance of the assumptions that the costs of users are
their privacy, and users are strategic to maximize their own utilities.

\ct{
10. Lee, J.S., Hoh, B.: Sell your experiences: a market mechanism based incentive for
participatory sensing. In: Proc. IEEE PerCom, pp. 60-68 (2010)
11. Lee, J.S., Hoh, B.: Dynamic pricing incentive for participatory sensing. Pervasive
and Mobile Computing 6(6), 693-708 (2010)

12. Jaimes, L.G., Vergara-Laurens, I., Labrador, M.A.: A location-based incentive
mechanism for participatory sensing systems with budget constraints. In: Proc.
IEEE PerCom, pp. 103-108 (2012)

13. Yang, D., Xue, G.,, X.F., et al.: Crowdsourcing to smartphones: incentive mechanism
design for mobile phone sensing. In: Proc. ACM MobiCom, pp. 173-184
(2012)

14. Koutsopoulos, I.: Optimal incentive-driven design of participatory sensing systems.
In: Proc. IEEE Infocom (2013)
}


\ctra{
[R3]
Han, Yang, Yanmin Zhu, Tong Liu, and Jiadi Yu. "Profit-Maximizing Stochastic Control for Participatory Sensing Platforms." 2014 (unpublished?)} -- 

\ab

In this paper, we consider the crucial problem
of maximizing the profit of a participatory sensing platform
which receives sensing requests from various subscribers and
completes the requests by leveraging sensing time of participating
smartphones. The profit of the platform equals the total charges
of sensing request minus the payments to smartphones. It is of
great challenge to the maximal profit for the platform, because
of stochastic arrivals of sensing requests, dynamic participation
of smartphones, and high complexity in allocating requests to
smartphones. In response to the challenges, we propose an
optimal online control framework which can efficiently utilize the
limited sensing time on each smartphone. Based on the stochastic
Lyapunov optimization techniques combined with the idea of
weight perturbation, our control framework makes online control
decisions including sensing requests admission and dispatching
control, sensing time purchasing control and sensing time allocation
control, without requiring any knowledge of the future
patterns. Rigorous mathematical analysis and comprehensive
simulation results show that our control framework can achieve
a time averaged profit that is arbitrarily close to the optimum,
while still maintaining strong system stability.

\bg

In recent years, participatory sensing has become a popular
paradigm for large-scale data collection [1][2]. The vast presentation
of smartphones with a rich set of built-in sensors (e.g.
accelerometer, humidity sensor, GPS, microphone and camera)
has greatly automatized the data generation process. Smartphones
can contribute their sensory data and collaboratively
provide large-scale sensing services, almost without human
intervention. It has also revolutionized the field of wireless
sensor networks, since it removes the cost of installing and
maintaining sensors, while obtaining much larger geographical
coverage. So far, there have been a number of participatory
sensing deployments, such as noise mapping [3], enviromental
monitoring [4][5][6], and civil infrastructure monitoring [7][8].

A typical participatory sensing system consists of a platform
deployed in the cloud and a number of smartphones with
various embedded sensors, as illustrated in Fig. 1. Smartphones
are connected to the platform via wireless networks.
The platform can provide sensing services to its subscribers by
processing their sensing requests (e.g. environmental and GPS
data collection requests). Sensing requests from subscribers
arrive at the platform dynamically. The platform pays the
users of smartphones for utilizing their devices and dispatches
sensing requests to smartphones for processing. At last it
aggregates sensory data of smartphones and forwards the
results to subscribers. In this way, the platform processes
sensing requests from subscribers and charges them for that
service. In other words, the platform can generate revenue
(utility) by processing sensing requests. In this paper, we
consider different types of heterogeneous sensing requests.
They may differ from each other in required sensors and can
generate different utility.




We can find that smpartphones play a significantly important
role in such a participatory sensing system since that the
service availability of the platform crucially depends on participation
of smartphones. However, the users of smartphones,
named participants, will suffer some cost during contribution
to the platform, such as battery energy cost, data processing
and transmission cost and their normal use of smartphones
may be affected when processing sensing requests. So that
participants would not allow the platform to utilize their
devices without limitation.

Therefore we consider the platform pays the participants
to motivate their participation in sensing requests processing,
according to their sensing time which means the time consumption
for processing sensing requests. To let the participants
have the initiative, we consider that they can sell sensing
time to the platform for requests processing. After purchasing
some sensing time, the platform then can utilize participants
for processing sensing requests. But it cannot utilize more than
the available sensing time that has been purchased. Note that
when and how much time to sell completely depends on the
participantsÕ willingness. For example, a participant may not
be willing to sell much sensing time when he or she is busy on
smartphone but may be willing to sell more sensing time when
he or she doesnÕt use smartphone frequently. The amount of
sensing time that participant is willing to sell represents how
willing the participant wants to participate in the system and
is totally dynamic and unpredictable.

The objective of the platform is to maximize the profit,
which equals to the revenue minus payment, subject to the
constraints that the average system backlog is finite (system
stability), and the sensing time-availability constraint is met,
i.e., the sensing time consumed on each smartphone is no more
than the time that is available, at all time. To achieve the
goal, four important control decisions need to be made in the
participatory sensing system: (1) how many requests of each
type to be admitted at any given time; (2) how to dispatch
the admitted sensing requests to a number of smartphones;
(3) how to allocate limited available sensing time to each type
of sensing requests for processing, on each smartphone; and
(4) how much sensing time to purchase when participants are
willing to sell some.



\textbf{Lyapunov:}
To tackle these challenges, we take advantage of Lyapunov
optimization technique developed in [9] to design a novel
optimal online control framework which can independently
and simultaneously make all the four control decisions in
the participatory sensing system. We utilize the basic Lyapunov
optimization technique together with the idea of weight
perturbation, e.g., [10] and [11]. The idea is to construct
the algorithm based on a quadratic Lyapunov function, but
carefully perturb the weights used for decision making, so
as to push the available sensing time volume towards certain
nonzero values on each smartphone to avoid underflow. Based
on this idea, our control framework can achieve a timeaveraged
profit which is arbitrarily close to the optimum,
while still remain strong stability. Specifically, our control
framework is able to achieve a time-averaged profit that is
within O(1/V ) of the optimum for any V > 0, and guarantees
that the system backlog is deterministically bounded by O(V ).



\ct{
[1] R. Ganti, F. Ye, and H. Lei, ``Mobile crowdsensing: current state and
future challenges,'' Communications Magazine, IEEE, vol. 49, no. 11,
pp. 32-39, 2011.

[2] N. D. Lane, E. Miluzzo, H. Lu, D. Peebles, T. Choudhury, and
A. T. Campbell, ``A survey of mobile phone sensing,'' Comm.
Mag., vol. 48, no. 9, pp. 140-150, Sep. 2010. [Online]. Available:
http://dx.doi.org/10.1109/MCOM.2010.5560598

[3] I. Schweizer, R. B¬artl, A. Schulz, F. Probst, and M. M¬uhl¬auser,
``Noisemap-real-time participatory noise maps,'' in Proc. 2nd Intl Workshop
on Sensing Applications on Mobile Phones (PhoneSense11), 2011,
pp. 1-5.

[4] M. Paxton and S. Benford, ``Experiences of participatory sensing in the
wild,'' in Proceedings of the 11th international conference on Ubiquitous
computing. ACM, 2009, pp. 265-274.

[5] D. Mendez, A. J. Perez, M. A. Labrador, and J. J. Marron, ``P-sense: A
participatory sensing system for air pollution monitoring and control,''
in Pervasive Computing and Communications Workshops (PERCOM
Workshops), 2011 IEEE International Conference on. IEEE, 2011,
pp. 344-347.

[6] D. Hasenfratz, O. Saukh, S. Sturzenegger, and L. Thiele, ``Participatory
air pollution monitoring using smartphones,'' in Proc. 1st Intl Workshop
on Mobile Sensing: From Smartphones and Wearables to Big Data,
2012.

[7] J. Eriksson, L. Girod, B. Hull, R. Newton, S. Madden, and H. Balakrishnan,
``The pothole patrol: using a mobile sensor network for road
surface monitoring,'' in Proceedings of the 6th international conference
on Mobile systems, applications, and services. ACM, 2008, pp. 29-39.

[8] A. Thiagarajan, L. Ravindranath, K. LaCurts, S. Madden, H. Balakrishnan,
S. Toledo, and J. Eriksson, ``Vtrack: accurate, energy-aware road
traffic delay estimation using mobile phones,'' in Proceedings of the
7th ACM Conference on Embedded Networked Sensor Systems. ACM,
2009, pp. 85-98.
}


\re

Little existing work has studied the problem of maximizing
the profit of the participatory sensing platforms subject to the
constraints of system stability and sensing time availability.
Most of the existing studies, such as [12] and [13], simply
assume the sensing requests are known and within the systemÕs
capacity, which is not practical. They donÕt need to consider
the problem of system stability and require sufficient statistical
knowledge of the sensing requests and the control decisions in
their work are made in an offline manner. Though there exist
online control solutions, e.g. [14], they work heavily relied
on a prediction-based approach. Their feasibility depends on
the accuracy of the prediction of future patterns, which is
usually nonstationary and almost unpredictable in the context
of participatory sensing. In comparison, our work proposes an
optimal online control framework which doesnÕt require any
priori knowledge of the future.


\ct{
[12] J.-S. Lee and B. Hoh, ``Sell your experiences: a market mechanism
based incentive for participatory sensing,'' in Pervasive Computing and
Communications (PerCom), 2010 IEEE International Conference on.
IEEE, 2010, pp. 60-68.

[13] I. Koutsopoulos, ``Optimal incentive-driven design of participatory sensing
systems,'' in INFOCOM, 2013 Proceedings IEEE, 2013, pp. 1402-
1410.

[14] H. Liu, S. Hu, W. Zheng, Z. Xie, S. Wang, P. Hui, and T. Abdelzaher,
``Efficient 3g budget utilization in mobile participatory sensing applications,''
in INFOCOM, 2013 Proceedings IEEE, 2013, pp. 1411-1419.
}


\ctra{
[R3.x]
Qingwen Zhao, Yanmin Zhu, \emph{et al.},
``Fair Energy-efficient Sensing Task Allocation in
Participatory Sensing with Smartphones,'' IEEE INFOCOM 2014.
}

\ab

With the proliferation of smartphones, participatory
sensing using smartphones provides unprecedented opportunities
for collecting enormous sensing data. There are two crucial
requirements in participatory sensing, fair task allocation and
energy efficiency, which are particularly challenging given high
combinatorial complexity, tradeoff between energy efficiency and
fairness, and dynamic and unpredictable task arrivals. In this paper,
we present a novel fair energy-efficient allocation framework
whose objective is characterized by min-max aggregate sensing
time. We rigorously prove that optimizing the min-max aggregate
sensing time is NP hard even when the tasks are assumed as a
priori. We consider two allocation models: offline allocation and
online allocation. For the offline allocation model, we design an
efficient approximation algorithm with the approximation ratio
of 2-1/m, where m is the number of member smartphones in
the system. For the online allocation model, we propose a greedy
online algorithm which achieves a competitive ratio of at most
m. The results demonstrate that the approximation algorithm
reduces over 81\% total sensing time, the greedy online algorithm
reduces more than 73\% total sensing time, and both algorithms
achieve over 3x better min-max fairness.

\bg


With the proliferation of mobile devices, participatory sensing
with smartphones becomes a new and important paradigm
for collecting and sharing data with the general public. A
lot of collaborative, crowdsourcing based applications spring
up. Example applications of participatory sensing include
intelligent transportation [1] [2] [3], localization [4] [5] [6],
environmental monitoring [7] [8], and crowding counting [9].

The typical architecture of a participatory sensing system
is illustrated in Fig. 1. The system is comprised of a central
platform and a collection of smartphones. The platform residing
on the cloud accepts sensing service requests from system
users, and allocates sensing tasks to the member smartphones.
After being assigned a sensing task, a smartphone performs
the required sensing service and returns the sensing data to the
platform which forwards the data to the querying user. The
smartphones in the participatory sensing system are assumed
cooperative (not strategic), which belong to or affiliated to
the system, willing to take sensing tasks and provide sensing
services to the system. We call such smartphones member
smartphones. Such participatory sensing systems are practical
and realistic in enterprise or agreement-based cooperation
scenarios. \textbf{The issue of participation incentive [10] [11] of
rational or even strategic smartphone user is out of the scope
of the paper.}

\ct{
[1] A. Thiagarajan, J. Biagioni, T. Gerlich, and J. Eriksson, ``Cooperative
transit tracking using smart-phones,'' in Proc. ACM SenSys, 2010.

[2] N. Pham, R. K. Ganti, Y. S. Uddin, S. Nath, and T. Abdelzaher, ``Privacypreserving
reconstruction of multidimensional data maps in vehicular
participatory sensing,'' in Wireless Sensor Networks. Springer, 2010,
pp. 114-130.

[3] K. Ali, D. Al-Yaseen, A. Ejaz, T. Javed, and H. S.Hassanein, ``Crowdits:
crowdsourcing in intelligent transportation systems,'' in IEEE WCNC,
2012.

[4] A. Rai, K. K. Chintalapudi, V. N.Padmanabhan, and R. Sen, ``Zee:
Zero-effort crowdingsourcing for indoor localization,'' in Proc. ACM
SIGOMM, 2012.

[5] J. Zhu, K. Zeng, K.-H. Kim, and P. Mohapatra, ``Improving crowdsourced
wi-fi localization systems using bluetooth beacons,'' in IEEE
SECON, 2012.

[6] F. Zaid, D. Costantini, P. S.Mogre, A. Reinhardt, J. Schmitt, and
R. Steinmetz, ``Wbroximity:mobile participatory sensing for wlan-and
bluetooth-based positiong,'' in IEEE LCN, 2010.

[7] R. K. Rana, C. T. Chou, S. S. Kanhere, N. Bulusu, and W. Hu, ``Earphone:
an end-to-end participatory urban noise mapping system,'' in
Proc. ACM IPSN, 2010.

[8] J. Ballesteros, M. Rahman, B. Carbunar, and N. Rishe, ``Safe cities.a
participatory sensing approach,'' in IEEE LCN, 2012.

[9] P. G. Kannan, S. P. Venkatagiri, M. C. Chan, A. L. Ananda, and L.-
S. Peh, ``Low cost crowd counting using audio tones,'' in Proc. ACM
SenSys, 2012.

[10] T. Luo and C.-K. Tham, ``Fairness and social welfare in incentivizing
participatory sensing,'' in IEEE SECON, 2012.

[11] Y. Zhang and M. v. d. Schaar, ``Reputation-based incentive protocols in
crowdsourcing applications,'' in Proc. IEEE INFOCOM, 2012.
}


\re

Participatory sensing has recently attracted extensive research
attention from both industry and academic due to its
attractive applications [3] [7] [8] [18]. Much existing work
has been done to address various kinds of participatory sensing
issues, such as the privacy problem [19]-[22] and the incentive
mechanism design [10] [11] [23]. This paper focuses on the
sensing task allocation in participatory sensing systems.

\ct{
[18] H. Weinschrott, J. Weisser, F. Durr, and K. Rothermel, ``Participatory
sensing algorithms for mobile object discovery in urban areas,'' in IEEE
percom, 2011.

[19] K. Xing, Z. Wan, P. Hu, H. Zhu, Y. Wang, X. Chen, Y. Wang, and
L. Huang, ``Mutual privacy-preserving regression modeling in participatory
sensing,'' in Proc. IEEE INFOCOM, 2013.

[20] H. Ahmadi, N. Pham, R. Ganti, T. Abdelzaher, S. Nath, and J. Han,
``Privacy-aware regression modeling of participatory sensing data,'' in
Proc. ACM SenSys, 2010.

[21] K. Vu, R. Zheng, and J. Gao, ``Efficient algorithms for k-anonymous
location privacy in participatory sensing,'' in Proc. IEEE INFOCOM,
2012.

[22] F. Zhang, L. He, W. He, and X. Liu, ``Data perturbation with statedependent
noise for participatory sensing,'' in Proc. IEEE INFOCOM,
2012.

[23] J.-S. Lee and B. Hoh, ``Sell your experiences: A market mechanism
based incentive for participatory sensing,'' in IEEE percom, 2009.
}


\ctra{
[R3.x]
Zhenni Feng, Yanmin Zhu, \emph{et al.},
``TRAC: Truthful Auction for Location-Aware
Collaborative Sensing in Mobile Crowdsourcing,'' IEEE INFOCOM 2014.}

\ab

In this paper, we tackle the problem of stimulating
smartphone users to join mobile crowdsourcing applications with
smartphones. Different from existing work of mechanism design,
we uniquely take into consideration the crucial dimension of
location information when assigning sensing tasks to smartphones.
However, the location awareness largely increases the theoretical
and computational complexity. In this paper, we introduce a
reverse auction framework to model the interactions between
the platform and the smartphones. We rigorously prove that
optimally determining the winning bids is NP hard. In this
paper we design a mechanism called TRAC which consists of
two main components. The first component is a near-optimal
approximate algorithm for determining the winning bids with
polynomial-time computation complexity, which approximates
the optimal solution within a factor of 1 + ln(n), where n
is the maximum number of sensing tasks that a smartphone
can accommodate. The second component is a critical payment
scheme which, despite the approximation of determining winning
bids, guarantees that submitted bids of smartphones reflect
their real costs of performing sensing tasks. Through both rigid
theoretical analysis and extensive simulations, we demonstrate
that the proposed mechanism achieves truthfulness, individual
rationality and high computation efficiency.

\bg

With the rapid advance in mobile devices and their embedded
sensors, mobile crowdsourcing with smartphones has
been a compelling paradigm for collecting distributed sensory
data to share with the general public [1]. Being carried by
human users who locate in different places, smartphones can
easily collect ubiquitous data and share such data with a large
number of potential users [2] [3].

A mobile crowdsourcing system typically consists of a
platform residing on the cloud and mobile smartphones. An
example is illustrated in Fig. 1. The platform selects the set of
smartphones to jointly provide sensing services. Once receiving
the notification of the platform, a smartphone collects the
required data. It then returns the collected sensing data to the
platform which then forwards the data to the platform user.
This demonstrates that a mobile crowdsourcing system with
geographically distributed smartphones can support a wide
range of large-scale monitoring applications [4].

Stimulating smartphone users to join collaborative sensing
is greatly important to the success of mobile crowdsourcing
with smartphones. As we know, it incurs some cost (e.g.,
power consumption for driving sensors and the CPU) when
a smartphone performs sensing for others. In addition, smartphone
users may suffer privacy breach as they share sensed
data (e.g., location data) with others. Thus, smartphone users
may not be willing to join a mobile crowdsourcing system
unless they receive enough compensation for their resource
consumption. Without the participation of a large number of
smartphones, one is not able to collect the desired data through
the mobile crowdsourcing application. As a result, no real
mobile crowdsourcing applications would be widely adopted.
Although a number of mobile crowdsourcing applications [5]
[6] [7] [8] have been proposed, most of them have assumed
that smartphones voluntarily contribute to the mobile crowdsourcing
system, which is not true in the real world.

\ct{
[1] ``Sensorly'', http://www.sensorly.com/.

[2] Dejun Yang, Guoliang Xue, Xi Fang, and Jian Tang, ``Crowdsourcing
to smartphones:incentive mechanism design for mobile phone sensing'',
in ACM MOBICOM, 2012. 

[3] Mohammad Nozari Zarmehri and Ana Aguiar, ``Supporting sensing
application in vehicular networks'', in ACM CHANTS, 2012.

[4] Raghu K Ganti, Fan Ye, and Hui Lei, ``Mobile crowdsensing: Current
state and future challenges'', IEEE Communications Magazine, vol. 49,
no. 11, pp. 32-39, 2011.

[5] Min Mun, Sasank Reddy, Katie Shilton, Nathan Yau, Jeff Burke, Deborah
Estrin, Mark Hansen, Eric Howard, Ruth West, and Pter Boda, ``Peir:
the personal environmental impact report, as a platform for participatory
sensing systems research'', in ACM MobiSys, 2009.

[6] Rajib Kumar Rana, Chun Tung Chou, Salil S. Kanhere, Nirupama
Bulusu, and Wen Hu, ``Ear-phone: an end-to-end participatory urban
noise mapping system'', in ACM/IEEE IPSN, 2010.

[7] Arvind Thiagarajan, Lenin Ravindranath, Katrina LaCurts, Samuel Madden,
Hari Balakrishnan, Sivan Toledo, and Jakob Eriksson, ``Vtrack: accurate,
energy-aware road traffic delay estimation using mobile phones'',
in ACM SenSys, 2009.

[8] Anshul Rai, Krishna Kant Chintalapudi, Venkata N.Padmanabhan, and
Rijurekha Sen, ``Zee: Zero-effort crowdingsourcing for indoor localization'',
in ACM SIGCOMM, 2012.
}

\textbf{Incentive:}
The problem of stimulating smartphone users to join mobile
crowdsourcing applications is highly complicated because
strategic behaviors of smartphone users can seriously hinder
the potential collaboration of smartphone users. Merely providing
fixed monetary rewards to participating smartphones,
however, is not adequate for guaranteeing smartphones to
perform collaborative sensing. Strategic smartphones would
take actions solely to maximize their own payoffs. In addition,
the cost information of each smartphone is private and no
smartphones would release such information. As a result,
the platform has no access to the cost information of each
smartphone. To maximize its own payoff, a smartphone may
deliberately claim a cost higher than the real one. Thus, mobile
crowdsourcing applications should be resilient to strategic
behaviors of smartphones.

There have been several research efforts on developing
incentive mechanisms for mobile crowdsourcing applications,
which can generally be divided into two categories. One
category of existing work tries to exploit auctions for inducing
cooperation from smartphones. In [2], Yang et al. consider
two types of incentive mechanisms for maximizing the utility
of the platform. It first proposes one incentive mechanism
using the Stackelberg game. This mechanism assumes that
the utility model of each user is known to the platform,
which is not always true. It then proposes an auction-based
mechanism. In this mechanism, a smartphone can only bid
for a specific subset of sensing tasks, which is not realistic
in the real world. The second category of existing work [9]
[10] adopts a different approach to stimulating cooperative
behaviors of selfish smartphone users. They try to build trust
among smartphones. Trust is useful but may not be sufficient
to fighting against strategic behaviors of smartphone users.

We also have an important observation that location awareness
is central to most mobile crowdsourcing applications. A
sensing task typically specifies the location where the sensing
task should be performed. This is because that the desired
sensing data are closely related to the specific location. A
sensing data collected at an irrelevant location is meaningless
or even invalid. This practical consideration on location awareness
caters to more meaning and accurate matching between
demands and supplies of sensing services. Unfortunately, most
of existing designs of incentive mechanism [11] [12] have
neglected this important dimension of location information in
their designs.

In this paper, we introduce a practical reverse auction framework,
in which the platform announces sensing tasks each of
which has a location attribute, and smartphones can submit
bids for a set of tasks within their service coverage. Each bid
has a private cost for performing the set of tasks. The platform
then decides the set of winning bids by which the sensing tasks
are allocated to the corresponding smartphones. The platform
will pay an amount of rewards to each contributing smartphone
for their sensing services.


To make this reverse auction framework actually work for
location-aware collaborative sensing in mobile crowdsourcing,
we aim at designing a truthful mechanism by which each
smartphone would truthfully declare its cost. To solve the
combinatorial auction problem, we have to address two critical
problems: 1) we have to design an efficient algorithm to
determine the winning bids and allocate the sensing tasks to smartphones
with a high efficiency (minimal social cost), and 2)
we have to design a payment policy to guarantee truthfulness,
fighting against the strategic behavior of smartphones. However,
we find that, after rigorous proof, the optimal winning bids
determination problem is NP hard. In this paper we design a
truthful mechanism called TRAC which consists of two main
components. Exploiting an efficient approximate algorithm,
the first component determines the winning bids. The second
component determines the critical payment to each winning
bid. The approximation algorithm can approximate the optimal
solution within a factor of 1 + ln(n), with polynomial-time
computation complexity, where n is the maximum number of
sensing tasks that a smartphone can accommodate. We also
theoretically prove that despite the approximate assignment
algorithm, TRAC guarantees truthfulness.

\ct{
[9] Xielei(Oscar) Wang, Wei Cheng, Prasant Mohapatra, and Tarek Abdelzaher,
``Artsense: Anonymous reputation and trust in participatory
sensing'', in IEEE INFOCOM, 2013.

[10] Alfred C.Weaver, Joseph P.Boyle, and Liliya I.Besaleva, ``Application
and trust issues when crowdsourcing a crisis'', in IEEE ICCCN, 2012.

[11] Iordanis Koutsopoulos, ``Optimal incentive-driven design of participatory
sensing systems'', in IEEE INFOCOM, 2013.

[12] Yu Zhang and Mihacla van der Schaar, ``Reputation-based incentive
protocols in crowdsourcing applications'', in IEEE INFOCOM, 2012.
}


\re

We review related work from three aspects, including incentive
schemes with strategic users, incentive schemes with
cooperative users, and privacy preservation.

\textbf{Incentives mechanism with strategic behaviors:} In [2], two
incentive mechanisms are designed for a user-centric model
and a platform centric model, respectively. In the platformcentric
model, the platform first announces the total amount
of money that the platform is willing to pay, and then each
smartphone decides the time it would like to provide the
sensing service. In the user-centric model, the objective is
system-wide. If a sensing task is finished, it would receive
some benefit. The goal is to select a subset of smartphones,
maximizing the overall gain. However, they only consider
single preference of a user, which means a user only submits
a single bid and it would win for performing all sensing tasks
in the bid or not at all. Such an assumption is not realistic
for location-aware collaborative sensing, failing to make the
best use of the sensing capabilities of all smartphones. In
[11], the author designs an optimal incentive mechanism for
participatory sensing and aim to maximize the revenue of
the service provider. The participating level of each user is
characterized by units and the user has a cost for each unit
of participation. The algorithm fails to take the location into
consideration and could not be applied to our problem because
of the NP-hardness of winning bids determination problem.

\textbf{Incentives schemes with cooperative users:} Some related
work proposing to provide monetary rewards to generally
cooperative users, such as [16] [17] [18]. Users are supposed
to be well motivated because they receive some monetary
rewards. In [16], a subset of users are greedily selected
according to their locations and the total budget. The algorithm
aims to cover the largest area. In [17], the users sell sensed data
to a service provider and a dynamic pricing scheme is designed
to stimulate more participants, thus achieving better quality of
service. In [18], it considers that a selfish user has the demand
of consuming data, and how much service it could consume
depends on how much she or he contributes to the participatory
sensing system. Thus, they have to consider how to satisfy all
users fairly and how to achieve a desirable result (maximized
social welfare) for the whole system. These existing studies
do not consider that cost information is private, and that users
may misreport their real costs in order to maximize their own
payoffs. As a result, these incentive schemes are not truthful.


\textbf{Privacy preserving schemes:} Privacy preserving is crucial
to mobile crowdsourcing with smartphones. It has attracted
many research efforts, such as [9] [10] [19] [20]. One smartphone
is supposed to report its sensed data, but it is
reluctant to disclose its private information, such as location,
and identity. In [21] and [22], the authors design regression
models for data which allow accurate model construction while
keeping individual information private. Some other studies
[23] [24] add noise or perturbation to original sensory data
for the purpose of anonymity. These papers usually utilize kanonymity
or entropy to measure the leakage of privacy. Our
work, which has focused on designing incentive mechanisms
for location-aware collaborative sensing, can benefit from
these existing schemes for protecting location privacy.


\ct{
[16] Luis G.Jaimes, Idalides Vergara-Laurens, and Miguel A.Labrador, ``A
location-based incentive mechanism for participatory sensing systems
with budget constraints'', in IEEE percom, 2012.

[17] Juong-Sik Lee and Baik Hoh, ``Sell your experiences:a market mechanism
based incentive for participatory sensing'', in IEEE percom, 2009.

[18] Afra J. Mashhadi, Sonia Ben Mokhtar, and Licia Capra, ``Fair content
dissemination in participatory dtns'', Ad Hoc Networks, vol. 10, no. 8,
pp. 1633-1645, 2012.


[19] Michael M.Groat, Benjamin Edwards, James Horey, Wenbo He, and
Stephanie Forrest, ``Enhancing privacy in participatory sensing applications
with multidimensional data'', in IEEE percom, 2012.

[20] Harald Weinschrott, Julian Weisser, Frank Durr, and Kurt Rothermel,
``Participatory sensing algorithms for mobile object discovery in urban
areas'', in IEEE percom, 2011.

[21] Hossein Ahmadi, Nam Pham, Raghu Ganti, Tarek Abdelzaher, Suman
Nath, and Jiawei Han, ``Privacy-aware regression modeling of participatory
sensing data'', in ACM Sensys, 2010.

[22] Kai Xing, Zhiguo Wan, Pengfei Hu, Haojin Zhu, Yuepeng Wang,
Xi Chen, Yang Wang, and Liusheng Huang, ``Mutual privacy-preserving
regression modeling in participatory sensing'', in IEEE INFOCOM,
2013.

[23] Fan Zhang, Li He, Wenbo He, and Xue Liu, ``Data perturbation with
state-dependent noise for participatory sensing'', in IEEE INFOCOM,
2012.

[24] Khuong Vu, Rong Zheng, and Jie Gao, ``Efficient algorithms for
k-anonymous location privacy in participatory sensing'', in IEEE
INFOCOM, 2012.
}


\newpage

\subsection{Yang, Dejun (2012) -- \comm{MobiCom}}


\ctra{
[R1.9]
Yang, Dejun, Guoliang Xue, Xi Fang, and Jian Tang. "Crowdsourcing to smartphones: incentive mechanism design for mobile phone sensing." In Proceedings of the 18th annual international conference on Mobile computing and networking, pp. 173-184. ACM, 2012.
}

\ab

Mobile phone sensing is a new paradigm which takes advantage
of the pervasive smartphones to collect and analyze
data beyond the scale of what was previously possible.
In a mobile phone sensing system, the platform recruits
smartphone users to provide sensing service. Existing
mobile phone sensing applications and systems lack good
incentive mechanisms that can attract more user participation.
To address this issue, we design incentive mechanisms
for mobile phone sensing. We consider two system models:
the platform-centric model where the platform provides a
reward shared by participating users, and the user-centric
model where users have more control over the payment they
will receive. For the platform-centric model, we design an
incentive mechanism using a Stackelberg game, where the
platform is the leader while the users are the followers. We
show how to compute the unique Stackelberg Equilibrium,
at which the utility of the platform is maximized, and none
of the users can improve its utility by unilaterally deviating
from its current strategy. For the user-centric model, we
design an auction-based incentive mechanism, which is computationally
efficient, individually rational, profitable, and
truthful. Through extensive simulations, we evaluate the
performance and validate the theoretical properties of our
incentive mechanisms.

\bg

The past few years have witnessed the proliferation of
smartphones in people?s daily lives. With the advent of
4G networks and more powerful processors, the needs for
laptops in particular have begun to fade. Smartphone sales
passed PCs for the first time in the final quarter of 2010
[3]. This inflection point occurred much quicker than predicted,
which was supposed to be 2012 [15]. According to
the International Data Corporation (IDC) Worldwide Quarterly
Mobile Phone Tracker, it is estimated that 982 million
smartphones will be shipped worldwide in 2015 [11].

Nowadays, smartphones are programmable and equipped
with a set of cheap but powerful embedded sensors, such
as accelerometer, digital compass, gyroscope, GPS, microphone,
and camera. These sensors can collectively monitor a
diverse range of human activities and surrounding environment.
Smartphones are undoubtedly revolutionizing many
sectors of our life, including social networks, environmental
monitoring, business, healthcare, and transportation [13].
If all the smartphones on the planet together constitute
a mobile phone sensing network, it would be the largest
sensing network in the history. One can leverage millions of
personal smartphones and a near-pervasive wireless network
infrastructure to collect and analyze sensed data far beyond
the scale of what was possible before, without the need to
deploy thousands of static sensors.
Realizing the great potential of the mobile phone sensing,
many researchers have developed numerous applications and
systems, such as Sensorly [23] for making cellular/WiFi network
coverage maps, Nericell [16] and VTrack [25] for providing
traffic information, PIER [17] for calculating personalized
environmental impact and exposure, and Ear-Phone
[20] for creating noise maps. For more details on mobile
phone sensing, we refer interested readers to the survey paper
[13].


As shown in Figure 1, a mobile phone sensing system consists
of a mobile phone sensing platform, which resides in
the cloud and consists of multiple sensing servers, and many
smartphone users, which are connected with the platform
via the cloud. These smartphone users can act as sensing
service providers. The platform recruits smartphone users
to provide sensing services.

Although there are many applications and systems on mobile
phone sensing [16, 17, 20, 23, 25], most of them are based
on voluntary participation. While participating in a mobile
phone sensing task, smartphone users consume their own resources
such as battery and computing power. In addition,
users also expose themselves to potential privacy threats by
sharing their sensed data with location tags. Therefore a
user would not be interested in participating in mobile phone
sensing, unless it receives a satisfying reward to compensate
its resource consumption and potential privacy breach.
Without adequate user participation, it is impossible for the
mobile phone sensing applications to achieve good service
quality, since sensing services are truly dependent on users?
sensed data. While many researchers have developed different
mobile phone sensing applications [5, 14], they either
do not consider the design of incentive mechanisms or have
neglected some critical properties of incentive mechanisms.
To fill this void, we will design several incentive mechanisms
to motivate users to participate in mobile phone sensing applications.


We consider two types of incentive mechanisms for a mobile
phone sensing system: platform-centric incentive mechanisms
and user-centric incentive mechanisms. In a platformcentric
incentive mechanism, the platform has the absolute
control over the total payment to users, and users can only
tailor their actions to cater for the platform. Whereas in a
user-centric incentive mechanism, the roles of the platform
and users are reversed. To assure itself of the bottom-line
benefit, each user announces a reserve price, the lowest price
at which it is willing to sell a service. The platform then selects
a subset of users and pay each of them an amount that
is no lower than the user?s reserve price.


\re

In [21], Reddy et al. developed recruitment frameworks
to enable the platform to identify well-suited participants
for sensing services. However, they focused only on the user
selection, not the incentive mechanism design. To the best
of our knowledge, there are few research studies on the incentive
mechanism design for mobile phone sensing [5, 14].
In [5], Danezis et al. developed a sealed-bid second-price
auction to motivate user participation. However, the utility
of the platform was neglected in the design of the auction.
In [14], Lee and Hoh designed and evaluated a reverse auction
based dynamic price incentive mechanism, where users
can sell their sensed data to the service provider with users?
claimed bid prices. However, the authors failed to consider
the truthfulness in the design of the mechanism.

The design of the incentive mechanism was also studied
for other networking problems, such as spectrum trading
[10, 26, 28] and routing [27]. However none of them can
be directly applied to mobile phone sensing applications,
as they all considered properties specifically pertain to the
studied problems.


\ct{
[1] S. Boyd and L. Vandenberghe. Convex Optimization.
Cambridge University Press, 2004.

[2] N. Chen, N. Gravin, and P. Lu. On the
approximability of budget feasible mechanisms. In
Proceedings of ACM-SIAM SODA, pages 685-699,
2011.

[3] CNN Fortune. Industry first: Smartphones pass PCs
in sales.
http://tech.fortune.cnn.com/2011/02/07/idc-
smartphone-shipment-numbers-passed-pc-in-q4-
2010/.

[4] E. Cuervo, A. Balasubramanian, D.-k. Cho,
A. Wolman, S. Saroiu, R. Chandra, and P. Bahl.
MAUI: making smartphones last longer with code
offload. In Proceedings of MobiSys, pages 49-62, 2010.

[5] G. Danezis, S. Lewis, and R. Anderson. How much is
location privacy worth? In Proceedings of WEIS, 2005.

[6] T. Das, P. Mohan, V. N. Padmanabhan, R. Ramjee,
and A. Sharma. PRISM: platform for remote sensing
using smartphones. In Proceedings of ACM MobiSys,
pages 63-76, 2010.

[7] E. De Cristofaro and C. Soriente. Short paper:
Pepsi?privacy-enhanced participatory sensing
infrastructure. In Proceedings of WiSec, pages 23-28,
2011.

[8] U. Feige, V. S. Mirrokni, and J. Vondrak. Maximizing
non-monotone submodular functions. SIAM J. on
Computing, 40(4):1133-1153, 2011.

[9] D. Fudenberg and J. Tirole. Game theory. MIT Press,
1991.

[10] L. Gao, Y. Xu, and X. Wang. Map: Multiauctioneer
progressive auction for dynamic spectrum access.
IEEE Transactions on Mobile Computing, 10(8):1144
-1161, August 2011.

[11] IDC. Worldwide smartphone market expected to grow
55\% in 2011 and approach shipments of one billion in
2015, according to IDC. http://www.idc.com/
getdoc.jsp?containerId=prUS22871611.

[12] V. Krishna. Auction Theory. Academic Press, 2009.

[13] N. Lane, E. Miluzzo, H. Lu, D. Peebles, T. Choudhury,
and A. Campbell. A survey of mobile phone sensing.
IEEE Communications Magazine, 48:140-150, 2010.

[14] J. Lee and B. Hoh. Sell your experiences: A market
mechanism based incentive for participatory sensing.
In Proceedings of IEEE PerCom, pages 60-68, 2010.

[15] M. Meeker. Mary Meeker: Smartphones will surpass
PC shipments in two years.
http://techcrunch.com/2010/11/16/meeker-
smartphones-pcs/.

[16] P. Mohan, V. N. Padmanabhan, and R. Ramjee.
Nericell: rich monitoring of road and traffic conditions
using mobile smartphones. In Proceedings of SenSys,
pages 323-336, 2008.

[17] M. Mun, S. Reddy, K. Shilton, N. Yau, J. Burke,
D. Estrin, M. Hansen, E. Howard, R. West, and
P. Boda. PIER, the personal environmental impact
report, as a platform for participatory sensing systems
research. In Proceedings of ACM MobiSys, pages
55-68, 2009.

[18] R. Myerson. Optimal auction design. Math. of
Operations Research, 6:58-73, 1981.

[19] G. Nemhauser, L. Wolsey, and M. Fisher. An analysis
of the approximations for maximizing submodular set
functions. Mathematical Programming, 14:265-294,
1978.

[20] R. Rana, C. Chou, S. Kanhere, N. Bulusu, and
W. Hu. Earphone: An end-to-end participatory urban
noise mapping. In Proceedings of ACM/IEEE IPSN,
pages 105-116, 2010.

[21] S. Reddy, D. Estrin, and M. B. Srivastava.
Recruitment framework for participatory sensing data
collections. In Proceedings of Pervasive, pages
138-155, 2010.

[22] C. Riederer, V. Erramilli, A. Chaintreau,
B. Krishnamurthy, and P. Rodriguez. For sale: your
data by: you. In Proceedings of ACM HotNets, pages
13:1-13:6, 2011.

[23] Sensorly. Sensorly. http://www.sensorly.com.

[24] Y. Singer. Budget feasible mechanisms. In Proceedings
of IEEE FOCS, pages 765-774, 2010.

[25] A. Thiagarajan, L. Ravindranath, K. LaCurts,
S. Madden, H. Balakrishnan, S. Toledo, and
J. Eriksson. Vtrack: accurate, energy-aware road
traffic delay estimation using mobile phones. In
Proceedings of ACM SenSys, pages 85-98, 2009.

[26] W. Wang, B. Li, and B. Liang. District: Embracing
local markets in truthful spectrum double auctions. In
Proceedings of IEEE SECON, pages 521-529, 2011.

[27] S. Zhong, L. Li, Y. G. Liu, and Y. Yang. On designing
incentive-compatible routing and forwarding protocols
in wireless ad-hoc networks: an integrated approach
using game theoretical and cryptographic techniques.
In Proceedings of ACM Mobicom, pages 117-131, 2005.

[28] X. Zhou, S. Gandhi, S. Suri, and H. Zheng. eBay in
the sky: strategy-proof wireless spectrum auctions. In
Proceedings of ACM Mobicom, pages 2-13, 2008.
}



\newpage


\subsection{Jiajun Sun (2014) -- \comm{Survey}}

\ctra{
Sun, Jiajun. "Incentive Mechanisms for Mobile Crowd Sensing: Current States and Challenges of Work." arXiv preprint arXiv:1310.8364 (2013).}

\ab

Crowd sensing is a new paradigm that leverages
pervasive sensor-equipped mobile devices like smartphones to
provide sensing services like forensic analysis, documenting
public spaces, or collaboratively constructing statistical models
in mobile social networks (MSNs). To achieve good quality
for crowd sensing, extensive user participating is indispensable
for crowd sensing in MSNs. Nowadays, most of existing
mechanisms focus on guaranteeing good service quality based
on instantaneous extensive user participating for crowd sensing
applications. Little attention has been dedicated to maximizing
long-term service quality for crowd sensing applications due to
their asymmetric interests, preferences, selfish behaviors, etc. To
fill these gaps, in this paper, we derive the closed expression of
the marginal content quality based on the monopoly aggregation
in economics. Furthermore, we design marginal-quality based
incentive mechanisms for long-term crowd sensing in MSNs, not
only to enhance extensive user participating by maximizing the
expected total profits of mobile users, but also to stimulate mobile
users to produce high-quality contents by applying the marginal
quality. Finally, simulation results indicate that our mechanisms
outperform the best existing solution.

\bg

With the increasing ubiquity of sensor-embedded mobile
devices (e.g., smartphones), mobile social networks (MSNs),
which integrate sensor data collection techniques and services
into many kinds of social networks [1], have received considerable
research efforts in recent years due to two changes
as follows. First, the terminal devices for social network
applications change from PCs to mobile phones. Second, the
interactive mode extends from the virtual space to the real
physical world. MSNs provide a new opportunity for crowd
sensing, which takes advantage of the pervasive mobile devices
to solve complex sensing tasks. A typical example of crowd
sensing applications involves sensing and reporting timely data
quality measurements about traffic flows in some region to
evaluate the traffic congestion situation to provide the support
of green traffic.

On the other hand, the potential of mixing both the crowd
sensing and MSNs makes it possible for the following application
to offer physical world free sensing data for online usergenerated
content platforms by roadside infrastructure units
(RIU) (e.g. cellular base stations or WLAN access points) in
MSNs. Such crowd sensing applications in MSNs expect that
crowd sensing would lead to both high quality contents from
endogenous entries and the long-term maximal expected profit
by voluntary high participation intelligently. Thus, the high
content quality submission, the long-term maximal expected
profit and the extensive user participation are three critical
issues for crowd sensing applications in MSNs.

However, many recent research works about these key issues
tend to separately study them in crowd sensing applications.
For instance, the authors in [2] proposed eliminating or hiding
low-quality content to provide content producers with incentives
to generate high-quality content. However, they fail to
account for the long-term maximal expected profit and the
extensive user participation. Only a handful of works [3]-[6]
focus on incentive mechanism for crowd sensing applications.
it is often assumed that these pricing schemes are impractical
since they need an accounting infrastructure [7], [8]. Besides,
they also neglect the high-quality content submission problem.
Therefore, how to simultaneously tackle the high content quality
submission, the maximal long-term expected profit and the
extensive user participation becomes particularly challenging
for crowd sensing applications in MSNs.

To this end, we first analyze the main stages of two-sided
marketsÑsensing data providers as providers, platforms, and
sensing data requirers as viewersÑon the basis of a typical
virtual currency supported by MSNs (see Fig. 1). Providers
expect to participate in sensing data so as to maximize their
profits for the high quality contents under the condition of
satisfying the number of desirable coverage users. At the
same time, viewers optimally allocate their content views to
maximize their utilities in terms of preferences. To do so, we
propose that platforms offer providers their advertising revenue
as economic incentives (i.e. subsidizing) to provide more high
quality contents under the condition of satisfying the predefined
number of users sensing data, which correspondingly
attract more content views (see Fig. 2).


\re

Incentives are a powerful and common mechanism for
crowd sensing applications such as task-driven applications,
citizen science applications, and urban sensing applications
[9] in MSNs. Recently, an entirely different approach to the
design of incentive mechanisms is pertinent in identifying the
social psychological motives that better reward those motives
to incentive participation [10], [11]. On the one hand, except
for [2], [8], there are a much smaller literatures addressing
the issue of high-quality contents for crowd sensing. However,
they do not consider the impact of the number of providers
on the content quality and derive the closed expression of
the marginal content quality. On the other hand, the authors
in [12]-[14] found that the quality of the work performed
by participants was affected by the number of the incentive,
compensation rate and work length. But they do not consider
the impact of viewer preferences on the content quality. The
authors of [3], [15] identified well-suited participants for sensing
services. But, they focused only on the user selection, not
novel interaction mechanisms design to incentive. In [3], [16],
participants are provided much stronger incentive mechanisms.
One of their proposed motivations is to better exploit the
available channels. But their network-wide throughput is not
optimal. Even if the mechanism in principle are proper to
attain social optimum by some setting, it is often assumed that
pricing schemes are impractical since they need an accounting
infrastructure [7].

Compared with the above mentioned pricing schemes, virtual
currency based incentive schemes have been extensively
popular since users provides the content collected without
the actual currency payments. For instance, in a reputationbased
mechanism, where profits and punishments are identified
based on differentiated services policy, the authors of [17]-
[19] explore incentives to address the social dilemma between
the ex-post payment and ex-ante payment. However, they do
not take into account the impact of the content quality on
the platform profits and the maximum profits over the infinite
horizon [20] [21]. Although the authors in [2], [8] explore
the content quality issues about maximizing the profits, they
neglect the maximum profits over the infinite horizon.


\ct{
[1] C. C. Aggarwal and T. Abdelzaher, ÒIntegrating sensors and social
networks,Ó in Social Network Data Analytics. Springer, 2011, pp. 379-
412.

[2] A. Ghosh and P. McAfee, ÒIncentivizing high-quality user-generated
content,Ó in Proceedings of the 20th international conference on World
wide web. ACM, 2011, pp. 137-146.

[3] D. Yang, G. Xue, X. Fang, and J. Tang, ÒCrowdsourcing to smartphones:
incentive mechanism design for mobile phone sensing,Ó MobiCom2012,
2012.

[4] J.-S. Lee and B. Hoh, ÒSell your experiences: a market mechanism
based incentive for participatory sensing,Ó in Pervasive Computing and
Communications (PerCom), 2010 IEEE International Conference on.
IEEE, 2010, pp. 60-68.

[5] L. Duan, T. Kubo, K. Sugiyama, J. Huang, T. Hasegawa, and J. Walrand,
ÒIncentive mechanisms for smartphone collaboration in data acquisition
and distributed computing,Ó in INFOCOM, 2012 Proceedings IEEE.
IEEE, 2012, pp. 1701-1709.

[6] L. G. Jaimes, I. Vergara-Laurens, and M. A. Labrador, ÒA location-based
incentive mechanism for participatory sensing systems with budget
constraints,Ó in Pervasive Computing and Communications (PerCom),
2012 IEEE International Conference on. IEEE, 2012, pp. 103-108.

[7] C. Buragohain, D. Agrawal, and S. Suri, ÒA game theoretic framework
for incentives in p2p systems,Ó in Peer-to-Peer Computing, 2003.(P2P
2003). Proceedings. Third International Conference on. IEEE, 2003,
pp. 48-56.

[8] S. Ren, J. Park, and M. van der Schaar, ÒMaximizing profit on usergenerated
content platforms with heterogeneous participants,Ó in INFOCOM,
2012 Proceedings IEEE. IEEE, 2012, pp. 612-620.

[9] J. Thebault-Spieker, ÒCrowdsourced participatory sensing: applications
and motivation of work,Ó 2012.

[10] K. Ling, G. Beenen, P. Ludford, X. Wang, K. Chang, X. Li, D. Cosley,
D. Frankowski, L. Terveen, A. Rashid, et al., ÒUsing social psychology
to motivate contributions to online communities,Ó Journal of Computer-
Mediated Communication, vol. 10, no. 4, 2005.

[11] M. Burke, C. Marlow, and T. Lento, ÒFeed me: motivating newcomer
contribution in social network sites,Ó in Proceedings of the 27th international
conference on Human factors in computing systems. ACM,
2009, pp. 945-954.

[12] M. Musthag, A. Raij, D. Ganesan, S. Kumar, and S. Shiffman, ÒExploring
micro-incentive strategies for participant compensation in highburden
studies,Ó in Proceedings of the 13th international conference on
Ubiquitous computing. ACM, 2011, pp. 435-444.

[13] W. Mason and D. Watts, ÒFinancial incentives and the performance
of crowds,Ó in Proceedings of the ACM SIGKDD workshop on human
computation. ACM, 2009, pp. 77-85.

[14] M. Buhrmester, T. Kwang, and S. Gosling, ÒAmazonÕs mechanical turk
a new source of inexpensive, yet high-quality, data?Ó Perspectives on
Psychological Science, vol. 6, no. 1, pp. 3-5, 2011.

[15] S. Reddy, D. Estrin, and M. Srivastava, ÒRecruitment framework for
participatory sensing data collections,Ó Pervasive Computing, pp. 138-
155, 2010.

[16] F. Wu, N. Singh, N. Vaidya, and G. Chen, ÒOn adaptive-width channel
allocation in non-cooperative, multi-radio wireless networks,Ó in INFOCOM,
2011 Proceedings IEEE. IEEE, 2011, pp. 2804-2812.

[17] C. Ho, Y. Zhang, J. Vaughan, and M. van der Schaar, ÒTowards social
norm design for crowdsourcing markets,Ó in Workshops at the Twenty-
Sixth AAAI Conference on Artificial Intelligence, 2012.

[18] Y. Zhang, J. Park, and M. van der Schaar, ÒDesigning social norm based
incentive schemes to sustain cooperation in a large community,Ó in Proc.
2nd International ICST Conf. on Game Theory for Networks, 2011.

[19] Y. Zhang and M. van der Schaar, ÒReputation-based incentive protocols
in crowdsourcing applications,Ó in INFOCOM, 2012 Proceedings IEEE.
IEEE, 2012, pp. 2140-2148.

[20] M. T. Spaan and N. Vlassis, ÒPerseus: Randomized point-based value
iteration for pomdps,Ó Journal of artificial intelligence research, vol. 24,
no. 1, pp. 195-220, 2005.

[21] M. L. Littman, ÒAlgorithms for sequential decision making,Ó Ph.D.
dissertation, Brown University, 1996.

[22] J. Sun, ÒMaximizing infinite-horizon based profits for crowd sensing in
mobile social networks,Ó http://arxiv.org/abs/1309.7735v1, 2013.

[23] A. Gudipati, S. Pereira, and S. Katti, ÒAutomac: rateless wireless concurrent
medium access,Ó in Proceedings of the 18th annual international
conference on Mobile computing and networking (MobiComÕ2012).
ACM, 2012, pp. 5-16.

[24] P. Whittle, ÒRestless bandits: Activity allocation in a changing world,Ó
Journal of applied probability, pp. 287-298, 1988.

[25] K. Liu and Q. Zhao, ÒIndexability of restless bandit problems and optimality
of whittle index for dynamic multichannel access,Ó Information
Theory, IEEE Transactions on, vol. 56, no. 11, pp. 5547-5567, 2010.

[26] A. E. Wenzhuo Ouyang and N. B. Shroff, ÒAsymptotically optimal
downlink scheduling over markovian fading channels,Ó in INFOCOM,
2012 Proceedings IEEE.

[27] W. Ouyang, A. Eryilmaz, and N. Shroff, ÒLow-complexity optimal
scheduling over correlated fading channels with arq feedback,Ó in
Modeling and Optimization in Mobile, Ad Hoc and Wireless Networks
(WiOpt), 2012 10th International Symposium on. IEEE, 2012, pp. 270-
277.

[28] P.-U. Tournoux, J. Leguay, F. Benbadis, J. Whitbeck, V. Conan, and
M. D. de Amorim, ÒDensity-aware routing in highly dynamic dtns:
The rollernet case,Ó Mobile Computing, IEEE Transactions on, vol. 10,
no. 12, pp. 1755-1768, 2011.
}




\newpage


\subsection{Niwat Thepvilojanapong (2013) -- \comm{utility-based incentive, demand/supply}}

\ctra{
[R5]
Thepvilojanapong, Niwat, Tomoya Tsujimori, Hao Wang, Yoshikatsu Ohta, Yunlong Zhao, and Yoshito Tobe. "Impact of Incentive Mechanism in Participatory Sensing Environment." In SMART 2013, The Second International Conference on Smart Systems, Devices and Technologies, pp. 87-92. 2013.}

\ab

Nowadays, the number of smartphone users is
growing rapidly. Recent smartphones equipped with several
sensors are convenient apps for collecting information in participatory
sensing environment. However, contributing sensing
data requires time and monetary cost, which hinder many
people from participation. To realize active and efficient sensing
activities, incentive mechanism is indispensable. This paper
proposes SenseUtil, utility-based incentive for participatory
sensing. SenseUtil applies the concept of micro economics,
where demand and supply decide the value of sensed data.
The incentive dynamically changes along the time according
to several factors such as sensing frequency, nearby sensing
points and users? preference. To study the impact of incentive
mechanism, we conducted simulation study. The results show
that people actively participate in sensing tasks while keeping
additional cost fewer than three percent in comparison with
non-incentive scenarios.


\bg

The number of smartphone users is growing rapidly [1]-
[3]. It has been reported that the smartphone penetration
in five leading European markets (France, Germany, Italy,
Spain and the United Kingdom) is 54.6% of mobile phone
users by the end of October 2012 [3]. In addition to
cellular communication standards (2G/3G/4G), smartphones
support several communication technologies including Wi-
Fi 802.11 a/b/g/n, Bluetooth and near field communication
(NFC). It also comes with high-performance processor and
various kinds of sensors such as accelerometer, gyroscope,
magnetometer, compass, GPS, barometer, microphone, ambient
light, camera and so on. These features of current
smartphones are useful for many apps which attract new
users
have been proposed in the literature [5]-[9]. However, many
smartphone users are not likely to participate in sensing
activities because it takes time and monetary cost for data
communication. Therefore, incentive mechanism is indispensable
to realize active participatory sensing by urging
people to report sensed data [10], [11].

This paper proposes SenseUtil, a utility-based incentive
framework for participatory sensing. In this model, consumers
who need data pay reward to producers who carry
out sensing tasks and report the data. SenseUtil applies the
concept of micro economics, where demand and supply
decide the value of sensed data. The demand and supply
depend on many factors including location, data types and
users? preference, and they also change along the time
dynamically. In particular, SenseUtil determines the value of
sensing activities by defining utility functions which are used
to calculate economical reward. SenseUtil aims to maximize
sensing activities while maintaining reasonable sensing cost.
To study the impact of SenseUtil, we conducted simulation
study. The results show that people actively participate in
sensing tasks while keeping additional cost fewer than three
percent in comparison with non-incentive scenarios.



\re

Participatory sensing using mobile phones is an active
and growing research area with a number of open issues
and challenges [4]. The Internet of Things (IoT), several
smartphone sensing platforms, information dissemination
algorithms, energy-efficient techniques and context-aware
apps, which are the complement of SenseUtil framework,
have been proposed in the literature [5]-[9], [13]-[15]. Guo
et al. present hybrid social networking, which highlights the
interweaving and cooperation of heterogeneous communities
[13]. Guo et al. extract the embedded intelligence about individual,
environment, and society by exploring the various
interactions between humans and the IoT [14]. Askus [15]
is a mobile social platform which allows users to send a
request to a group of potential people in a remote area to do
a task. Similar to Askus, other existing sensing platforms are
voluntary systems, i.e., sensing data are contribution from
cooperative users. SenseUtil can be applied directly to such
previous works.


To realize active and efficient sensing activities, incentive
mechanism has been introduced recently. Most of previous
works adopt auction algorithms to decide the value
of sensing data [10], [11], [16], [17]. Unlike previous
works, SenseUtil?s consumers indirectly determine their bids
through some factors such as minimum price, maximum
price, changing rate of price. In addition, the bid price of
SenseUtil dynamically changes according to nearby POIs
and sensing frequency without any further intervention of
consumers.

\ct{
[1] R. T. Llamas and W. Stofega, ?Worldwide smartphone 2012-
2016 forecast and analysis,? IDC Corporate USA, Tech.
Rep., Mar. 2012, http://www.idc.com/getdoc.jsp?containerId=
233553 (Accessed: January 29, 2013).

[2] M. Meeker and L.Wu, ?2012 Internet trends,? Kleiner Perkins
Caufield \& Byers, May 2012, http://www.kpcb.com/insights/
2012-internet-trends (Accessed: January 29, 2013).

[3] A. Mohamud, ?EU5 smartphone penetration reaches
55 percent in October 2012,? comScore Press Release,
Dec. 2012, http://www.comscore.com /Insights/Press
Releases/2012/12/EU5 Smartphone Penetration Reaches
55 Percent in October 2012 (Accessed: January 29, 2013).

[4] N. D. Lane et al., ?A survey of mobile phone sensing,? IEEE
Communications Magazine, vol. 48, no. 9, Sep. 2010, pp.
140-150.

[5] E. Miluzzo et al., ?Sensing meets mobile social networks:
the design, implementation and evaluation of the CenceMe
application,? in Proceedings of the 6th International Conference
on Embedded Networked Sensor Systems (SenSys
2008), Raleigh, North Carolina, USA, Nov. 2008, pp. 337-
350.

[6] S. Reddy, D. Estrin, and M. Srivastava, ?Recruitment framework
for participatory sensing data collections,? in Proceedings
of the 8th International Conference on Pervasive
Computing (Pervasive 2010), Helsinki, Finland, May 2010,
pp. 138-155.

[7] M. Musolesi, M. Piraccini, K. Fodor, A. Corradi, and A. T.
Campbell, ?Supporting energy-efficient uploading strategies
for continuous sensing applications on mobile phones,? in
Proceedings of the 8th International Conference on Pervasive
Computing (Pervasive 2010), Helsinki, Finland, May 2010,
pp. 355-372.

[8] T. Choudhury et al., ?The mobile sensing platform: An
embedded activity recognition system,? IEEE Pervasive Computing,
vol. 7, no. 2, April-June 2008, pp. 32-41.

[9] S. Consolvo et al., ?Activity sensing in the wild: a field trial
of ubifit garden,? in Proceedings of the SIGCHI Conference
on Human Factors in Computing Systems (CHI 2008), 2008,
pp. 1797-1806.

[10] D. Yang, G. Xue, X. Fang, and J. Tang, ?Crowdsourcing to
smartphones: incentive mechanism design for mobile phone
sensing,? in Proceedings of the 18th annual international
conference on Mobile computing and networking (Mobicom
2012), Aug. 2012, pp. 173-184.

[11] L. Jaimes, I. Vergara-Laurens, and M. A. Labrador, ?A
location-based incentive mechanism for participatory sensing
systems with budget constraints,? in Proceedings of the IEEE
International Conference on Pervasive Computing and Communications
(PerCom 2012), Mar. 2012, pp. 103-108.

[12] D. B. Johnson and D. A. Maltz, ?Dynamic source routing in
ad hoc wireless networks,? in Mobile Computing, T. Imielinski
and H. Korth, Eds.Kluwer Academic Publishers, 1996,
ch. 5, pp. 153-181.

[13] B. Guo, Z. Yu, X. Zhou, and D. Zhang, ?Hybrid
SN: Interlinking opportunistic and online communities to
augment information dissemination,? in Proceedings of the
9th International Conference on Ubiquitous Intelligence and
Computing and 9th International Conference on Autonomic
and Trusted Computing (UIC-ATC 2012), Washington, DC,
USA, Sep., 2012, pp. 188-195.

[14] B. Guo et al., ?From the internet of things to embedded
intelligence,? World Wide Web Journal, Sep. 2012, pp. 1-22.

[15] S. Konomi et al., ?Askus: Amplifying mobile actions,? in
Proceedings of the 7th International Conference on Pervasive
Computing (Pervasive 2009), Nara Japan, May 2009, pp.
202-219.

[16] J.-S. Lee and B. Hoh, ?Dynamic pricing incentive for
participatory sensing,? Pervasive and Mobile Computing,
vol. 6, no. 6, Dec. 2010, pp. 693-708.

[17] ??, ?Sell your experiences: a market mechanism based
incentive for participatory sensing,? in Proceedings of the
IEEE International Conference on Pervasive Computing and
Communications (PerCom 2010), Mar. 2010, pp. 60-68.
}




\subsection{Akshay Dua (2009) -- \comm{Trustworthy}}


\ctra{
Dua, Akshay, Nirupama Bulusu, Wu-Chang Feng, and Wen Hu. "Towards trustworthy participatory sensing." In HotSec 09: Proceedings of the Usenix Workshop on Hot Topics in Security. 2009.
}

\ab

Grassroots Participatory Sensing empowers people to
collect and share sensor data using mobile devices across
many applications, spanning intelligent transportation,
air quality monitoring and social networking. In this paper,
we argue that the very openness of such a system
makes it vulnerable to abuse by malicious users who may
poison the information, collude to fabricate information,
or launch Sybils to distort that information. We propose
and implement a novel trusted platform module (TPM),
or angel based system that addresses the problem of providing
sensor data integrity. The key idea is to provide
a trusted platform within each sensor device to attest the
integrity of sensor readings. We argue that this localizes
integrity checking to the device, rather than relying on
corroboration, making the system not only simpler, but
also resistant to collusion and data poisoning. A ?burnedin?
private key in the TPM prevents users from launching
Sybils. We also make the case for content protection and
access control mechanisms that enable users to publish
sensor data streams to selected groups of people and address
it using broadcast encryption techniques.

\bg

Participatory Sensing is a revolutionary new paradigm
that allows people to voluntarily sense their environment
using readily available sensor devices such as smart
phones, and share this information using existing cellular
and Internet communication infrastructure. It has
tremendous potential because it harnesses the power of
ordinary citizens to collect sensor data for applications
spanning environmental monitoring, intelligent transportation,
and public health, that are often not cost-viable
using dedicated sensing infrastructure.



Participatory sensing differs from traditional sensor
networks in that there is typically no single data producer
(sensor data owner). As in any participatory system, such
as Wikipedia, and online recommendation systems, participatory
sensing is vulnerable to gaming. Moreover,
data producers and consumers (sensor data users) are different
autonomous entities. So, producers may want to
restrict whom they share their data with.



This paper proposes a novel approach to addressing
the above problems with a trusted hardware platform,
which besides the main processor, consists of a trusted
platform module(such as the TPM [4]), or an angel. The
key idea is that the angel is present in each user device
and is used to (i) check the integrity of contributed sensor
measurements, and (ii) implement state-of-the-art cryptographic
algorithms for content protection. With an angel,
sensor data integrity verification is local to the data
producer, and hence, this model is not only scalable, it
is also inherently resilient to collusion among producers.
The contributions of the paper are:


\subsection{Jaimes, Luis G (2012) -- \comm{location-based incentive} -- A long report}

\ctra{
[R4] 
Jaimes, Luis G., Idalides Vergara-Laurens, and Miguel A. Labrador. "A location-based incentive mechanism for participatory sensing systems with budget constraints." In Pervasive Computing and Communications (PerCom), 2012 IEEE International Conference on, pp. 103-108. IEEE, 2012.}


\ab

Participatory Sensing (PS) systems rely on the willingness of mobile users to participate in the
collection and reporting of data using a variety of sensors either embedded or integrated in their
cellular phones. Users agree to use their cellular phone resources to sense and transmit the data
of interest because these data will be used to address a collective problem that otherwise would
be very difficult to assess and solve. However, this new data collection paradigm has not been
very successful yet mainly because of the lack of incentives for participation and privacy concerns.
Without adequate incentive and privacy guaranteeing mechanisms most users will not be willing to
participate. This thesis concentrates on incentive mechanisms for user participation in PS system.
Although several schemes have been proposed thus far, none has used location information and
imposed budget and coverage constraints, which will make the scheme more realistic and efficient.
A recurrent reverse auction incentive mechanism with a greedy algorithm that selects a representative
subset of the users according to their location given a fixed budget is proposed. Compared to
existing mechanisms, GIA (i.e., Greedy Incentive Algorithm) improves the area covered by more
than 60 percent acquiring a more representative set of samples after every round, i.e., reduces the
collection of unnecessary (redundant) data, while maintaining the same number of active users in
the system and spending the same budget.


\subsection{Sasank Reddy (2010) -- \comm{Micropayment}}

\ctra{
[R2.20] S. Reddy, D. Estrin, M. Hansen, and M. Srivastava, ``Examining micropayments
for participatory sensing data collections,'' in UbiComp, 2010.
}

\ab

The rapid adoption of mobile devices that are able to capture
and transmit a wide variety of sensing modalities (media
and location) has enabled a new data collection paradigm
- participatory sensing. Participatory sensing initiatives organize
individuals to gather sensed information using mobile
devices through cooperative data collection. A major
factor in the success of these data collection projects is sustained,
high quality participation. However, since data capture
requires a time and energy commitment from individuals,
incentives are often introduced to motivate participants.
In this work, we investigate the use of micro-payments as
an incentive model. We define a set of metrics that can be
used to evaluate the effectiveness of incentives and report
on findings from a pilot study using various micro-payment
schemes in a university campus sustainability initiative.

\bg

Mobile phones are increasingly able to sense a variety of
modalities. These familiar devices already record text, images,
and location information. When users are involved in
deciding what data to collect, it is referred to as participatory
sensing [5, 6, 13]. Many interesting technical and user interface
challenges exist in participatory sensing [2, 14]. One of
these is the design of mechanisms that encourage individuals
to contribute information towards the sensing task. Recent
participatory sensing projects have explored different methods
to motivate individuals to participate. Techniques have
included highlighting the altruistic nature of data collections
(gathering information for ecological efforts in EpiCollect),
providing beneficial personal analytics (bicycle ride details
in Biketastic), enabling data bartering to obtain additional
information (bargain hunting through price queries in Live-
Compare), and involving individuals in challenges (traffic
monitoring with treasure quests in Waze) [1, 16, 8, 18].


In this work, we explore incentives based on micro-payments,
i.e., transactions in which small tasks are matched with small
payments. We consider various micro-payment models including
different set amounts per sample and a dynamic payment
in which competition determines the per sample payment
rate. These micro-payment schemes are compared to
the base case of a lump sum macro-payment for the data
collection as a whole. We define a set of standard participation
and performance metrics that can be used to evaluate
the effectiveness of incentive models in data collections and
report on findings from a pilot study. The results from the
study lead to design guidelines in how to create and organize
payment based incentives for participatory sensing projects.

We build on this related
work but concentrate on using micro-payments for mobile
sensing tasks and analyze the effects of different payment
schemes on participation frequency, quality, and coverage.





==> section2-literature.tex <==
%!TEX root = main_participarory_sensing.tex
%SourceDoc main_participarory_sensing.tex


\section{Literature Review}\label{sec:literature}

%Participatory sensing systems greatly rely on the  voluntary participation of users.  
%Hence, 
\revv{
Motivating user participation is one of the most important issues in participatory sensing. 
Several recent works have devoted to the incentive mechanism design in participatory sensing, mainly using pricing 
and auction.
In \cite{yang-mobicom12}, Yang \emph{et al.} considered two system models: the platform-centric model and the user-centric model. 
For the platform-centric model, an incentive mechanism based on Stackelberg game is designed to maximize the utility of the platform. 
For the user-centric model, an auction-based incentive mechanism is designed, under individuals rational assumption. 
In \cite{Jaimes-2012}, Jaimes \emph{et al.} proposed a greedy algorithm based on the recurrent reverse auction incentive mechanism, which aims to
maximize the covered area under a budget constraint.
In \cite{zhuym-infocom14-b}, Zhu \emph{et al.} considered the crucial dimension of location information when assigning sensing tasks to smartphones, and propose a truthful reverse auction incentive framework for the location-aware participatory sensing system. 
In \cite{zhuym-book2013}, Zhu \emph{et al.} proposed a novel price-based decomposition incentive framework for optimizing the system wide performance. 
In \cite{Koutsopoulos-infocom13}, Koutsopoulos \emph{et al.} proposed 
an optimal reverse auction incentive mechanism to to minimize the total costs of users. This work illustrates the significance of the assumptions that the costs of users are their privacy, and users are strategic to maximize their own utilities. 
In \cite{Luo-infocom2014}, Luo \emph{et al.} design an incentive mechanism based on all-pay auctions for the participatory sensing system. 
However, all of the above incentive mechanisms focused on the  {short-term sensing incentive}, without considering the  {long-term participation incentive}. 

In \cite{Lee-2010} and \cite{Lee-2010-b}, Lee \emph{et al.} considered the 
long-term participation incentive  in participatory sensing. 
They assumed that users will drop out of the participatory sensing system unless the achieved Return on Investment (ROI) is greater than their expectations. 
They introduced a \emph{virtual credit} for lowering the bids of users who lost in the previous round of auction, hence increasing their winning probabilities in future auction rounds. 
However, their proposed mechsnisms considered neither the truthfulness, nor the optimality of the proposed auction. 
In this work, we will study both the  {short-term sensing incentive} and the  {long-term participatory incentive} in participatory sensing, with rigorous analysis on the truthfulness and the optimality.
}


%
% 
%Several recent works have focused on designing incentive mechanisms to motivate smartphone users for participatory sensing.
%Most of these works apply auction algorithms \cite{yang-mobicom12, zhuym-infocom14-b, Lee-2010, Lee-2010-b, Jaimes-2012, Koutsopoulos-infocom13, zhuym-infocom14-b, Luo-infocom2014}. 
%A novel reverse auction based on dynamic price is proposed in \cite{Lee-2010, Lee-2010-b}, where
%users sell their sensed data to the platform by claiming bid prices, and the platform selects a subset of these users and purchases
%at their bid prices. Their work shows that using dynamic price can reduce the incentive cost compared with fixed price. Luis
%G. Jaimes et al. \cite{Jaimes-2012} propose a greedy algorithm based on the recurrent reverse auction incentive mechanism, which aims to
%maximize the covered area under a budget constraint. 
%Two system models are considered in \cite{yang-mobicom12}: the platform-centric model
%and the user-centric model. For the platform-centric model, an incentive mechanism based on Stackelberg game is designed
%to maximize the utility of the platform. For the user-centric model, an auction-based incentive mechanism is designed, under
%individuals rational assumption. 
%Koutsopoulos et al. \cite{Koutsopoulos-infocom13} aim to minimize the total costs of compensating users via proposing
%an optimal reverse auction mechanism. This work illustrates the significance of the assumptions that the costs of users are
%their privacy, and users are strategic to maximize their own utilities.
%Y. Zhu et al. \cite{zhuym-infocom14-b} take into consideration the crucial dimension of location information when assigning sensing tasks to smartphones, and propose a truthful reverse auction framework for the location-aware participatory sensing system. 
%In \cite{Luo-infocom2014}, Luo et al. design an incentive mechanism based on all-pay auctions for participatory sensing.
%In [14], Lee and Hoh designed and evaluated a reverse auction based dynamic price incentive
%mechanism, where users can sell their sensed data to the service provider with users? claimed bid prices. However, the authors
%failed to consider the truthfulness in the design of the mechanism.
%
%The second category of
%existing work \cite{Wang-infocom2013, Weaver-icccn2012} adopts a different approach to stimulating cooperative behaviors of selfish smartphone users. They try to
%build trust among smartphones. Trust is useful but may not be sufficient to fighting against strategic behaviors of smartphone
%users.
%
%
%
%In this work, we explore incentives based on micro-payments, i.e., transactions in which small tasks are matched with small
%payments \cite{Reddy-ubicomp2012}.
%
%
%Participation incentives are intrinsic to the application \cite{Zhang-infocom2012, Luo-secon2012}: for example in LiveCompare, users obtain the service, namely
%product prices in nearby stores, only if they participate by submitting prices themselves. If participants do not obtain a direct
%benefit from participation, appropriate incentive mechanisms need to be designed. In the CrowdPark system, compensation
%comes through subsequent gains from re-selling the parking spot, which exceed the refund received if they deny the spot on
%purpose. The work in [x] guides credit allocation to participants by using the feedback of quality of provisioned information
%(QoI) and credit satisfaction from information requesters and participants respectively. In \cite{Luo-secon2012}, the authors consider users as
%data contributors and requesters at the same time, and they formulate convex optimization problems that allocate credit quota
%to users to maximize utility functions that denote social welfare or fairness. User utility is a concave function of normalized
%allocated credit, normalized over user demand and contribution cost. In \cite{Zhang-infocom2012}, the authors consider a reputation-based scheme in
%the context of a crowdsourcing website. The scheme builds upon a reputation metric that rewards or penalizes users, depending
%on whether their strategy is aligned to or deviates from a social norm. The scheme is then incorporated into a repeated game
%model that captures interactions of users who contribute to and request information from the website.
% 
%
%
%
%








==> section5a-noinform-dis.tex <==
%!TEX root = main_participarory_sensing.tex
%SourceDoc main_participarory_sensing.tex

\subsection{Discussion}

Now we compare the above two on-line sensor selection policies. 
Obviously, both policies rely only on the current network information and the allocation history (captured by the dual variables $\blb$ or the virtual queues $\bque$), while not on any complete or stochastic future information.

\subsubsection{Allocation Rule}

From Policies \ref{algo:1} and \ref{algo:2}, we can easily see that both policies use the same allocation rule in each time slot. Namely, both policies aims at  
$$
\max_{ \bxt } \ \Vt - \sumN  \xnt \cdot \wcnt, 
$$
where 
\begin{equation*}
\wcnt \eq \left\{
\begin{aligned}
& \cnt - \lbn^{t} & \mbox{in Policy \ref{algo:1},}
\\
& \textstyle \cnt - \frac{1}{\lypV} \cdot \quen^{t} & \mbox{in Policy \ref{algo:2}.}
\end{aligned}
\right.
\end{equation*}
We refer to the dual variable $\lbn^{t} $ and the virtual queue $\quen^{t} $ as \emph{regulation factors}. 
Accordingly, we refer to $\wcnt$ as the \emph{regulated} sensing cost of user $n$ in slot $t$. 
Obviously, increasing $\lbn^t$ or $\quen^t$ will decrease the  (regulated) sensing cost of user $n$, and thus increase the probability of being selected as sensor in slot $t$. 
Intuitively, the dual variables $\blb$ in Policy \ref{algo:1} or the queue backlogs $\bque$ in Policy \ref{algo:2} are used for lowering the sensing costs of users, such that the users with a low allocation probability will more likely be selected as sensors in the future.

\subsubsection{Updating Rule}
It is easy to see that the updating rules for dual variables in Policie \ref{algo:1} and for queue backlogs in Policy \ref{algo:2} are very different. 
Specifically, in Policy \ref{algo:1}, we have:\footnote{We omit the operation $[.]^+$ for analytical convenience.} 
$$
\lbn^{\tau}= \lbn^{0} - \sum_{t=0}^{\tau-1} \step^{t} \cdot \left( \dn[t] - \D_n\right),
$$
where $\dn[t] = \frac{1}{t}\sum_{k=1}^t \xndo[k] $ is the average allocation probability from the beginning till slot $t$.  
Hence, the dual variable $\lbn^{\tau}$ in slot $\tau$ is a weighted sum  of $(\dn[t] - \D_n), t=0,...,\tau-1$, i.e., the gap between the actual allocation probability and the required allocation probability threshold.

In Policy \ref{algo:2}, we have:
$$
\quen^{\tau}= \quen^0 - \sum_{t=0}^{\tau-1} \xnlo[t] + \tau \cdot D_n. 
$$
That is, the queue backlog $\quen^{\tau}$ in slot $\tau$ is the difference between the required allocation slots and the actual allocation slots till slot $\tau$. 
Hence, $\frac{\quen^{\tau}}{\tau}$ reflects the gap between the required allocation probability and the actual allocation probability till slot $\tau$. 
By Theorem \ref{theorem:2}, the total queue backlog is bounded; thus, the allocation probability gap goes to zero as $\tau \rightarrow \infty$.


%\com{Have not emphasized the difference between these two rules enough. 
%In fact, given the page limit, maybe we can just state one algorithm in this paper (and leave another one in the journal). }
%
%\com{Lin: Agree. We can focus on one policy, and list the key result of another policy. Or in other case, we focus on one policy only, and keep the other policy entirely in the technical report.}




==> section5a-noinform-dual.tex <==
%!TEX root = main_participarory_sensing.tex
%SourceDoc main_participarory_sensing.tex


\subsection{Dual-Decomposition Based On-line Allocation Policy}


\subsubsection{\textbf{Dual Decomposition Technique}}

By dual decomposition, we define Lagrange dual multipliers $\lbn \geq 0$, $n=1,...,N$, for the user participatory constraint (b) in (\ref{problem:stochastic}$\mathrm{x}$).
Then, \revv{the Lagrangian for the relaxation of (\ref{problem:stochastic}$\mathrm{x}$) is} 
%%
\begin{equation}\label{eq:lagrangian}
\begin{aligned}
\txsty
\lag(\bX, \blb) \eq & \txsty
\intTH  \big( \V(\th) - \C(\th) \big) \cdot f(\th) \dd \th
\\
& \txsty + \sumN  \lbn \cdot 
\left( \intTH \xn(\th)   f(\th) \dd \th - \D_n  \right),
%\\
% = & \txsty  \intTH  \lag(\th, \blb) \dd \th
\end{aligned}
\end{equation}
%%
where 
%$\bX \eq \{\bx(\th)\}_{\th\in\TH} = \{\xn(\th)\}_{n=1,...,N,\th\in\TH}$, and 
$\blb \eq \{\lbn\}_{n=1,...,N}$. 
The dual objective function is
%%
\begin{equation}\label{eq:dual-objective}
\dual(\blb) \eq \max_{ \bX } \lag(\bX,\blb).
\end{equation}
%%
With constraint qualifications, it is easy to check that the strong duality holds in the relaxation of problem (\ref{problem:stochastic}$\mathrm{x}$). 
%\comm{x is an integer, hence problem  (10) is not convex? Hence the strong duality does NOT hold?}
Hence, 
%%
\begin{equation}\label{eq:dual-problem}
\VCso  =  \dual(\blb^*) \eq \min_{\blb\succeq 0} \dual(\blb),
\end{equation}
%%
where $\VCso$ is the maximum expected social welfare  with the stochastic information given by (\ref{problem:stochastic}$\mathrm{x}$) (studied in Section \ref{sec:stochastic}).
This implies that maximizing the primal problem (\ref{problem:stochastic}$\mathrm{x}$) is equivalent to minimizing the dual problem (\ref{eq:dual-problem}). 

We first show how to derive the dual objective $D(\blb)$ in (\ref{eq:dual-objective}). 
It is easy to see that the Lagrangian (\ref{eq:lagrangian}) can be rewritten as~~
%%
\begin{equation}\label{eq:lagrangian-new}
\txsty
\lag(\bX, \blb)= \intTH  \lag_{\th}(\bx(\th), \blb) f(\th) \dd \th, 
\end{equation}
%%
where 
$$
\lag_{\th}(\bx(\th), \blb) \eq 
\V(\th) - \C(\th) + \sumN \lbn \cdot (\xn(\th) - \D_n)
$$ 
is related to $\th$ and the associated allocation vector $\bx(\th)$ under $\th$ only. 
This implies that the dual objective $\dual(\blb)$  in (\ref{eq:dual-objective}) can be obtained by 
maximizing $ \lag_{\th}(\bx(\th), \blb)$ under each $\th \in \TH$ independently. Formally, we have
%%
\begin{lemma}\label{lemma:dual}
\begin{equation}\label{eq:dual-objective-new}
\txsty
\dual(\blb)
= \lag(\bXdo, \blb) 
% = \intTH  \lag_{\th}(\bxdo(\th), \blb)f(\th) \dd \th,
\end{equation}
%%
where $\bXdo \eq \{\bxdo(\th)\}_{\th\in\TH}$, and $\bxdo(\th)   $ is given by
%%
\begin{equation}\label{eq:dual-problem-new}
\begin{aligned}
\bxdo(\th) 
%& = \arg \max_{ \bx(\th) } \ \txsty \lag_{\th}(\bx(\th),\blb)
%\\
& = \arg \max_{ \bx(\th) } \ \txsty \V(\th) - \C(\th) + \sumN \lbn \cdot  \xn(\th).
\end{aligned}
\end{equation}
\end{lemma}

Lemma \ref{lemma:dual} implies that solving the dual objective $\dual(\blb)$ via (\ref{eq:dual-problem-new}) does not need the stochastic distribution of $\th$ (although the value of $\dual(\blb)$ depends on the distribution of $\th$). 
Moreover, we can easily find that (\ref{eq:dual-problem-new}) is also a set cover problem (hence is NP-hard), with the same form as (\ref{problem:stochastic-solution}); 
% when ignoring the irrelevant term $\sumN \lbn\cdot \D_n$; 
hence, it can be solved with the same method for (\ref{problem:stochastic-solution}), e.g., the branch-and-bound algorithm or the greedy algorithm in \cite{report}.

We then show how to solve the dual problem (\ref{eq:dual-problem}).
Notice that the dual objective $ \dual(\blb) $ is always convex in $\blb$ (even when the primal problem  (\ref{problem:stochastic}$\mathrm{x}$) is not convex), 
as it is the pointwise supremum of a family of affine functions of $\lbn$, $n\in\N$. Hence, the minimizer of $ \dual(\blb) $ is given by 
$$
\nabla_{\dual}(\blb) = \boldsymbol{0}, 
$$
where $\nabla_{\dual} (\blb) \eq \{ \frac{\partial \dual(\blb)}{\partial \lbn} \}_{n=1,...,N}$ is the gradient of $\dual(\blb)$.
However, without stochastic information, we cannot derive the analytical forms of $\dual(\blb)$ and its gradient $\nabla \dual(\blb)$. 
Hence, we will solve the dual problem (\ref{eq:dual-problem}) by the \emph{sub-gradient} based iterative computational method \cite{Boyd-convex},  which is widely used for solving convex optimization problems.


\subsubsection{\textbf{Sub-Gradient Method}}
 
The key idea of the sub-gradient method is to iteratively search a sequence of feasible dual variables $\{\blb^{1}, \blb^{2}, ..., \blb^{k}  \}$ along a \emph{sub-gradient} direction of $\dual(\blb)$, such that $\dual(\blb^{k}) < \dual(\blb^{k-1})$ and $ \lim_{k\rightarrow \infty}\dual(\blb^{k}) = \dual(\blb^*)$.
Obviously, in such a sub-gradient based method, one  important problem is to find a proper sub-gradient for  $\dual(\blb)$.

We construct a sub-gradient of $\dual(\blb)$ in the following way. 
Given any $\blb$, we denote $\dndo \eq \dn(\bxndo) = \intTH \xndo(\th)   f(\th) \dd \th $ as the allocation probability of user $n$ under the optimal allocation $\bxndo $ given in (\ref{eq:dual-problem-new}). Notice that $\dndo$ is a function of $\blb$ (as $\bxndo$ depends on $\blb$); hence we can write $\dndo$ as $\dndo(\blb)$. 
We further denote $\subg_n(\blb) \eq \dndo(\blb) - \D_n$ as the gap between the actual allocation probability $\dndo(\blb)$ and the required allocation probability (threshold) $\D_n$. 
Then, we have the following sub-gradient for $\dual(\blb)$.
%%
\begin{lemma}\label{lemma:subgradient}
Let $\subG (\blb) \eq \{ \subg_n(\blb) \}_{n=1,...,N}$, where $\subg_n(\blb) =\dndo(\blb) - \D_n$. Then, $\subG (\blb)$ is a sub-gradient of $\dual(\blb)$ at $\blb$.\footnote{Here, the sub-gradient $\subg_n (\blb)$ still depends on the stochastic information. Later we will show how to compute $\subg_n (\blb)$ with the history information only.}~~~~~~~~~~
\end{lemma}

%\begin{proof}
%For any $\blb^{0} \neq \blb$, we have: 
%$$
%\dual(\blb^{0}) = 
%%\lag(\bX^{\ddag}, \blb^{0}) \eq  
%\max_{ \bX } \lag(\bX,\blb^{0}) \geq  \lag(\bXdo, \blb^{0}), 
%$$
%where $\bXdo \eq \arg  \max_{\bX} \lag(\bX,\blb)$  is the optimal scheduling under dual variables $\blb$, i.e., that defined in (\ref{eq:dual-problem-new}). 
%Notice that~~~~
%\begin{equation*}
%\begin{aligned}
%\txsty
%\lag(\bXdo, \blb^{0})
%& \txsty  = 
%\lag(\bXdo, \blb) + \sumN (\lbn^0 - \lbn) \cdot ( \dndo(\blb) -\D_n)
%\\
%& \txsty = \dual(\blb) + 
%	(\blb^{0} - \blb)^{\textsc{T}} \odot \subG (\blb).
%\end{aligned}
%\end{equation*}
%Combining the above two equations, we have: 
%\begin{equation}\label{eq:subg}
%\dual(\blb^{0}) \geq \dual(\blb) + 	(\blb^{0} - \blb)^{\textsc{T}} \odot \subG (\blb).
%\end{equation}
%That is, $\subG (\blb)$ is a sub-gradient of $\dual(\blb)$ at $\blb$. 
%\end{proof}

The lemma can be proved as follows. For any $\blb^{0} \neq \blb$,  
%%
\begin{equation}\label{eq:subg}
\begin{aligned}
 \dual(\blb^{0})
& = \max_{ \bX } \lag(\bX,\blb^{0}) \geq  \lag(\bXdo, \blb^{0})
\\
& \txsty  = 
\lag(\bXdo, \blb) + \sumN (\lbn^0 - \lbn) \cdot ( \dndo(\blb) -\D_n)
\\
&\txsty = \dual(\blb) + 	(\blb^{0} - \blb)^{\textsc{T}} \odot \subG (\blb), 
\end{aligned}
\end{equation}
%%
where $\odot$ is the dot-product operation. 
Hence, $\subG (\blb)$ is a sub-gradient of $\dual(\blb)$ at $\blb$. 
The above equation further implies that if $\subg_n (\blb) > 0$ (or $\subg_n (\blb) < 0$), then we can potentially obtain a smaller dual objective $\dual(\blb)$ by  slightly decreasing $\lbn$ to $\lbn^0 < \lbn$ (or increasing $\lbn$ to $\lbn^0 > \lbn$). Hence, to iteratively reduce $\dual(\blb)$, we can update the dual variables $\blb$ along the (negative) sub-gradient direction, i.e.,~~~~~~
%%
\begin{equation}\label{eq:submethod}
\txsty
\lbn^{k+1}= \left[\lbn^{k} - \step^{k} \cdot \subg_n (\blb^{k}) \right]^+, \quad \forall n=1,...,N,
\end{equation}
%%
where $[\lb]^+ = \max\{0, \lb\}$, and $\step^{k} \geq 0$ is the step-size. This sub-gradient  based iteration of $\blb$   is usually called the \emph{sub-gradient method}. 
It is important to note that the sub-gradient method (\ref{eq:submethod}) still requires the stochastic information, as the sub-gradient $\subG (\blb)$ depends on the stochastic information.~~~~~~~~~~

Next we show how to compute $\subG (\blb)$ without the stochastic information. 
Let $\th[t]$ denote the information realized in slot $t$, and 
$\xndo[t] \eq \xndo(\th[t]) $ denote whether a user $n$ is selected in slot $t$ under the optimal allocation $\xndo(.)$ given in (\ref{eq:dual-problem-new}). Then, by the law of large numbers, we have: 
$$
\txsty
\lim_{T\rightarrow\infty} \frac{1}{T}\sumT \xndo[t] = 
 \intTH \xndo(\th)   f(\th) \dd \th = \dndo (\blb).
$$
That is, as long as the sensing period $T$ is large enough, we can use the statistical allocation probability $\frac{1}{T}\sumT \xndo[t]$ of user $n$ to approximate its theoretical allocation probability $\dndo (\blb) = \intTH \xndo(\th)   f(\th) \dd \th$.  
\revv{Note that when $T$ is finite, there is certain error in the above approximation. 
In this case, the sub-gradient method is actually using a noisy sub-gradient, and is essentially a \emph{stochastic sub-gradient method} in \cite{Boyd-subgradient}.}~~~~~~~~~~~~~~
 

\subsubsection{\textbf{On-line Allocation Policy}}

Based on the above discussion, we propose the following \emph{dual-decomposition} based on-line sensor selection (allocation) policy, which consists of two steps in each time slot: the \emph{allocation rule} and the \emph{updating rule}. 
Specifically, the allocation rule determines the allocation vector $\bxdo[t]$ in each slot $t$  according to (\ref{eq:dual-problem-new}), based on the current information $\th[t]$ and dual multipliers $\blb^t$.  
The updating rule updates the dual variables $\blb$ according to (\ref{eq:submethod}), along the negative (noisy) sub-gradient direction $\frac{1}{t}\sum_{k=1}^t \xndo[k] - \D_n$.   
Formally, we present the detailed policy in Policy \ref{algo:1}.
  
\begin{algorithm}[t]
\label{algo:1}
\small
\caption{Dual-decomposition based policy}
\DontPrintSemicolon
%\BlankLine
%\emph{The economic interaction of master $m$ with the database and the end-users}\;
%\vspace{-3mm}
\textbf{Initialization:} $\blb = \blb^1$;\;
\For{each time slot $t=1,...,T$}
{
%Denote the realized information in slot $t$ as $\th[t] = \th$;\;
\emph{Allocation Rule:}
\begin{equation*}
\begin{aligned}
\bxdo[t]
%& = \arg \max_{ \bx(\th[t]) } \lag_{\th[t]} (\bx(\th[t]),\blb^{t}) 
%\\
& = \arg \max_{ \bxt } \left( 
\Vt - \Ct + \txsty \sumN \lbn^{t} \cdot \xnt \right)
\end{aligned}
\end{equation*}
\emph{Updating Rule:}
$$
\txsty
\lbn^{t+1}= \left[\lbn^{t} - \step^{t} \cdot \left(\frac{1}{t}\sum_{k=1}^t \xndo[k] - \D_n\right) \right]^+, \quad \forall n\in\N
$$
}
\end{algorithm}


It is easy to see that the dual-decomposition based Policy \ref{algo:1} selects users in each time slot $t$ only based on the current network information $\th[t]$ and the past allocation history (captured by the dual variables $\blb^t$), while not on any complete or stochastic future information. 
In the following, we further show that with a proper step-size $\step^{t}$, it asymptotically converges to the same maximum expected social welfare as that using the stochastic information. 
Let $\VCdo[t]\eq (\Vt - \Ct)|_{\bxdo[t]}$ denote the social welfare achieved in a particular slot $t$  by using the proposed dual-decomposition policy. Then, 
%$\VCdo \eq \frac{1}{T} \sumT \VCdo[t]$ denote the expected social welfare achieved in the entire sensing period. 
%Then,
 

\begin{theorem}\label{theorem:1}
If $\step^{t}$ satisfies the diminishing nonsummable condition:
$\lim_{t\rightarrow\infty} \step^{t} = 0$ and 
$\sum_{t=1}^{\infty} \step^{t} = \infty$, then
$$
 \lim_{t\rightarrow \infty} \blb^{t} = \blb^*,
 \mbox{~~and~~}
 \lim_{T\rightarrow \infty} \frac{1}{T} \sumT \VCdo[t] = \VCso.
$$
\end{theorem}


\revv{Theory \ref{theorem:1} and Policy \ref{algo:1} imply that we do not need to go through another round of iteration to obtain the precise sub-gradient for the updating of dual variables in each step. The reason is that the error in the approximate sub-gradient is stochastic and unbiased (i.e., with a zero mean), and hence can be gradually ``average out'' in the iteration.}
A typical example of $\step^{t}$ that satisfies the diminishing nonsummable condition is $\step^{t} = \frac{1}{t}$. 
It is notable that we can also choose other step-sizes, e.g., a constant step-size $\step^t = \step$. 
However, as shown in \cite{Boyd-subgradient}, a constant step-size may lead to certain approximation error in the achieved social welfare.
%
%\comm{Proof sketch? 
%the index should be ÒkÓ instead of ÒtÓ?
%In other words, we require a separation of time scales? In each time slot t, we need to go through another round of iteration indexed by k, such that we get the right subgradient with a larger enough iterations in a single time slot? 
%Even when this happens, we will have exact the optimal $\lambda^*$ eventually, or the time average (expected) value of lambda will converge to the optimal?}
%



%
%\\
%& \geq  \lag(\bxdo, \blb^{0}) 
%\\
%& = \lag(\bxdo, \blb) + (\blb^{0} - \blb) \otimes \subG (\blb)
%\\
%& = \dual(\blb) + (\blb^{0} - \blb) \otimes \subG (\blb)
%\end{aligned}
%\end{equation}


%\emph{Scheduling Rule.} 
%In a particular time slot $t$ (with an information realization $\th$), the SP schedules mobile users, aiming at maximizing the following objective function:
%$$
%\txsty
%\lag(\th) = \V(\th) - \C(\th) + \sumN \lbn \cdot (\D_n - \d_n^{(t)})
%$$
%where $\lbn$ is the Lagrange multiplier of user $n$, and $\d_n^{(t)}$ is the actual scheduling probability of user $n$ until slot $t$. 
%
%\emph{Updating Rule.}
%In each time slot $t$, the SP updates the Lagrange multiplier of each user $n$ in the following way: 
%$$
%\lbn = [\lbn - \step^{(t)} \cdot (\d_n^{(t)} - \D_n)]^+, \quad \forall n\in \N,
%$$
%where $\step^{(t)} $ is the stepsize in slot $t$. 
%
%\com{It is important to note that if the stepsize $\step^{(t)} $ satisfies: (i) $\lim_{T\rightarrow \infty} \sumT \step^{(t)}  = \infty $, and (ii) $\lim_{T\rightarrow \infty} \step^{(t)} = 0$. Then, the above $\lbn $ converges to that with stochastic information. 
%In our previous report, we choose a constant stepsize, which does not satisfy the above conditions, hence does not converge.}
%
%\begin{lemma}
%The above dual-decomposition based on-line scheduling policy converges to the optimal (in expectation) social welfare. 
%\end{lemma}
%
%\begin{lemma}
%The above dual-decomposition based on-line scheduling policy guarantees the user participatory constraint. 
%\end{lemma}



